Exoplanet Atmosphere Measurements from Direct Imaging

In the last decade, about a dozen giant exoplanets have been directly imaged in the IR as companions to young stars. With photometry and spectroscopy of these planets in hand from new extreme coronagraphic instruments such as SPHERE at VLT and GPI at Gemini, we are beginning to characterize and classify the atmospheres of these objects. Initially, it was assumed that young planets would be similar to field brown dwarfs, more massive objects that nonetheless share similar effective temperatures and compositions. Surprisingly, young planets appear considerably redder than field brown dwarfs, likely a result of their low surface gravities and indicating much different atmospheric structures. Preliminarily, young free-floating planets appear to be as or more variable than field brown dwarfs, due to rotational modulation of inhomogeneous surface features. Eventually, such inhomogeneity will allow the top of atmosphere structure of these objects to be mapped via Doppler imaging on extremely large telescopes. Direct imaging spectroscopy of giant exoplanets now is a prelude for the study of habitable zone planets. Eventual direct imaging spectroscopy of a large sample of habitable zone planets with future telescopes such as LUVOIR will be necessary to identify multiple biosignatures and establish habitability for Earth-mass exoplanets in the habitable zones of nearby stars.

==> HBexoTemplateBib <==
@STRING{\apjl = "Astrophys. J. Lett."}
@STRING{\apj = "Astrophys. J"}
@STRING{\mnras = "Mon. Not. R. Astron. Soc."}
@STRING{\aap = "Astron. \& Astrophys."}
@STRING{\nat = "Nature"}
@STRING{\sci = "Science"} 
@STRING{\araa = "Ann. Rev. of Astron. \& Astrophys."}
@STRING{\aj = "Astron. J."}
@STRING{\procspie = "Proc. SPIE"}
@STRING{\apjs = "Astrophys. J. Supplement"}

@ARTICLE{Gel02,
   author = {{Gelino}, C.~R. and {Marley}, M.~S. and {Holtzman}, J.~A. and 
	{Ackerman}, A.~S. and {Lodders}, K.},
    title = "{L Dwarf Variability: I-Band Observations}",
  journal = \apj,
   eprint = {astro-ph/0205305},
 keywords = {Stars: Atmospheres, Stars: Low-Mass, Brown Dwarfs},
     year = 2002,
    month = sep,
   volume = 577,
    pages = {433-446},
      doi = {10.1086/342150},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...577..433G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sam17,
       author = {{Samland}, M. and {Molli{\`e}re}, P. and {Bonnefoy}, M. and {Maire}, A.
        -L. and {Cantalloube}, F. and {Cheetham}, A.~C. and {Mesa}, D.
        and {Gratton}, R. and {Biller}, B.~A. and {Wahhaj}, Z. and
        {Bouwman}, J. and {Brandner}, W. and {Melnick}, D. and {Carson},
        J. and {Janson}, M. and {Henning}, T. and {Homeier}, D. and
        {Mordasini}, C. and {Langlois}, M. and {Quanz}, S.~P. and {van
        Boekel}, R. and {Zurlo}, A. and {Schlieder}, J.~E. and
        {Avenhaus}, H. and {Beuzit}, J. -L. and {Boccaletti}, A. and
        {Bonavita}, M. and {Chauvin}, G. and {Claudi}, R. and {Cudel},
        M. and {Desidera}, S. and {Feldt}, M. and {Fusco}, T. and
        {Galicher}, R. and {Kopytova}, T.~G. and {Lagrange}, A. -M. and
        {Le Coroller}, H. and {Martinez}, P. and {Moeller-Nilsson}, O.
        and {Mouillet}, D. and {Mugnier}, L.~M. and {Perrot}, C. and
        {Sevin}, A. and {Sissa}, E. and {Vigan}, A. and {Weber}, L.},
        title = "{Spectral and atmospheric characterization of 51 Eridani b using
        VLT/SPHERE}",
      journal = {\aap},
     keywords = {stars: individual: 51 Eridani, planets and satellites: atmospheres,
        methods: data analysis, techniques: high angular resolution,
        techniques: image processing, Astrophysics - Earth and Planetary
        Astrophysics},
         year = 2017,
        month = Jul,
       volume = {603},
          eid = {A57},
        pages = {A57},
          doi = {10.1051/0004-6361/201629767},
       adsurl = {https://ui-adsabs-harvard-edu.insu.bib.cnrs.fr/#abs/2017A&A...603A..57S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Ch17,
       author = {{Chauvin}, G. and {Desidera}, S. and {Lagrange}, A. -M. and {Vigan}, A.
        and {Gratton}, R. and {Langlois}, M. and {Bonnefoy}, M. and
        {Beuzit}, J. -L. and {Feldt}, M. and {Mouillet}, D. and {Meyer},
        M. and {Cheetham}, A. and {Biller}, B. and {Boccaletti}, A. and
        {D'Orazi}, V. and {Galicher}, R. and {Hagelberg}, J. and
        {Maire}, A. -L. and {Mesa}, D. and {Olofsson}, J. and {Samland},
        M. and {Schmidt}, T.~O.~B. and {Sissa}, E. and {Bonavita}, M.
        and {Charnay}, B. and {Cudel}, M. and {Daemgen}, S. and
        {Delorme}, P. and {Janin-Potiron}, P. and {Janson}, M. and
        {Keppler}, M. and {Le Coroller}, H. and {Ligi}, R. and
        {Marleau}, G.~D. and {Messina}, S. and {Molli{\`e}re}, P. and
        {Mordasini}, C. and {M{\"u}ller}, A. and {Peretti}, S. and
        {Perrot}, C. and {Rodet}, L. and {Rouan}, D. and {Zurlo}, A. and
        {Dominik}, C. and {Henning}, T. and {Menard}, F. and {Schmid},
        H. -M. and {Turatto}, M. and {Udry}, S. and {Vakili}, F. and
        {Abe}, L. and {Antichi}, J. and {Baruffolo}, A. and {Baudoz}, P.
        and {Baudrand}, J. and {Blanchard}, P. and {Bazzon}, A. and
        {Buey}, T. and {Carbillet}, M. and {Carle}, M. and {Charton}, J.
        and {Cascone}, E. and {Claudi}, R. and {Costille}, A. and
        {Deboulbe}, A. and {De Caprio}, V. and {Dohlen}, K. and
        {Fantinel}, D. and {Feautrier}, P. and {Fusco}, T. and {Gigan},
        P. and {Giro}, E. and {Gisler}, D. and {Gluck}, L. and {Hubin},
        N. and {Hugot}, E. and {Jaquet}, M. and {Kasper}, M. and
        {Madec}, F. and {Magnard}, Y. and {Martinez}, P. and {Maurel},
        D. and {Le Mignant}, D. and {M{\"o}ller-Nilsson}, O. and
        {Llored}, M. and {Moulin}, T. and {Orign{\'e}}, A. and {Pavlov},
        A. and {Perret}, D. and {Petit}, C. and {Pragt}, J. and {Puget},
        P. and {Rabou}, P. and {Ramos}, J. and {Rigal}, R. and {Rochat},
        S. and {Roelfsema}, R. and {Rousset}, G. and {Roux}, A. and
        {Salasnich}, B. and {Sauvage}, J. -F. and {Sevin}, A. and
        {Soenke}, C. and {Stadler}, E. and {Suarez}, M. and {Weber}, L.
        and {Wildi}, F. and {Antoniucci}, S. and {Augereau}, J. -C. and
        {Baudino}, J. -L. and {Brandner}, W. and {Engler}, N. and
        {Girard}, J. and {Gry}, C. and {Kral}, Q. and {Kopytova}, T. and
        {Lagadec}, E. and {Milli}, J. and {Moutou}, C. and {Schlieder},
        J. and {Szul{\'a}gyi}, J. and {Thalmann}, C. and {Wahhaj}, Z.},
        title = "{Discovery of a warm, dusty giant planet around HIP 65426}",
      journal = {\aap},
     keywords = {instrumentation: adaptive optics, instrumentation: high angular
        resolution, methods: observational, planets and satellites:
        atmospheres, planets and satellites: formation, Astrophysics -
        Earth and Planetary Astrophysics},
         year = 2017,
        month = Sep,
       volume = {605},
          eid = {L9},
        pages = {L9},
          doi = {10.1051/0004-6361/201731152},
       adsurl = {https://ui-adsabs-harvard-edu.insu.bib.cnrs.fr/#abs/2017A&A...605L...9C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{All16,
   author = {{Allers}, K.~N. and {Gallimore}, J.~F. and {Liu}, M.~C. and 
	{Dupuy}, T.~J.},
    title = "{The Radial and Rotational Velocities of PSO J318.5338-22.8603, a Newly Confirmed Planetary-mass Member of the {$\beta$} Pictoris Moving Group}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1601.04717},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, infrared: stars, planets and satellites: atmospheres, stars: rotation, techniques: radial velocities, techniques: spectroscopic},
     year = 2016,
    month = mar,
   volume = 819,
      eid = {133},
    pages = {133},
      doi = {10.3847/0004-637X/819/2/133},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...819..133A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{All13,
   author = {{Allers}, K.~N. and {Liu}, M.~C.},
    title = "{A Near-infrared Spectroscopic Study of Young Field Ultracool Dwarfs}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1305.4418},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, infrared: stars, planets and satellites: atmospheres, stars: low-mass },
     year = 2013,
    month = aug,
   volume = 772,
      eid = {79},
    pages = {79},
      doi = {10.1088/0004-637X/772/2/79},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...772...79A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zap06,
   author = {{Zapatero Osorio}, M.~R. and {Mart{\'{\i}}n}, E.~L. and {Bouy}, H. and 
	{Tata}, R. and {Deshpande}, R. and {Wainscoat}, R.~J.},
    title = "{Spectroscopic Rotational Velocities of Brown Dwarfs}",
  journal = \apj,
   eprint = {astro-ph/0603194},
 keywords = {stars: individual (DENIS-P J0255.0-4700), stars: individual (GL 570D), Stars: Individual: Alphanumeric: LP 944-20, stars: individual ([Pleiades] PPl 1), stars: individual (SDSS J053951.99-005902.0), stars: individual (SDSS J134646.45-003150.4), stars: individual (SDSS J162414.37+002915.6), stars: individual (SDSSp J125453.90-012247.4), stars: individual (2MASS J00361617+1821104), stars: individual (2MASS J03341218-4953322), stars: individual (2MASS J04151954-0935066), stars: individual (2MASS J05591914-1404488), stars: individual (2MASS J12171110-0311131), stars: individual (2MASS J15031961+2525196), stars: individual (2MASS J15530228+1532369AB), stars: individual (2MASS J16322911+1904407), stars: individual (2MASS J17281150+3948593AB), stars: individual (2MASS J22244381-0158521), stars: individual (vB 10), Stars: Low-Mass, Brown Dwarfs, Stars: Rotation},
     year = 2006,
    month = aug,
   volume = 647,
    pages = {1405-1412},
      doi = {10.1086/505484},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...647.1405Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bur03,
   author = {{Burrows}, A. and {Sudarsky}, D. and {Lunine}, J.~I.},
    title = "{Beyond the T Dwarfs: Theoretical Spectra, Colors, and Detectability of the Coolest Brown Dwarfs}",
  journal = \apj,
   eprint = {astro-ph/0304226},
 keywords = {Infrared: Stars, Molecular Processes, Radiative Transfer, Stars: Low-Mass, Brown Dwarfs},
     year = 2003,
    month = oct,
   volume = 596,
    pages = {587-596},
      doi = {10.1086/377709},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...596..587B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sne14,
   author = {{Snellen}, I.~A.~G. and {Brandl}, B.~R. and {de Kok}, R.~J. and 
	{Brogi}, M. and {Birkby}, J. and {Schwarz}, H.},
    title = "{Fast spin of the young extrasolar planet {$\beta$} Pictoris b}",
  journal = \nat,
     year = 2014,
    month = may,
   volume = 509,
    pages = {63-65},
      doi = {10.1038/nature13253},
   adsurl = {http://adsabs.harvard.edu/abs/2014Natur.509...63S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lag10,
   author = {{Lagrange}, A.-M. and {Bonnefoy}, M. and {Chauvin}, G. and {Apai}, D. and 
	{Ehrenreich}, D. and {Boccaletti}, A. and {Gratadour}, D. and 
	{Rouan}, D. and {Mouillet}, D. and {Lacour}, S. and {Kasper}, M.
	},
    title = "{A Giant Planet Imaged in the Disk of the Young Star {$\beta$} Pictoris}",
  journal = \sci,
archivePrefix = "arXiv",
   eprint = {1006.3314},
 primaryClass = "astro-ph.EP",
     year = 2010,
    month = jul,
   volume = 329,
    pages = {57},
      doi = {10.1126/science.1187187},
   adsurl = {http://adsabs.harvard.edu/abs/2010Sci...329...57L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sch16,
   author = {{Schwarz}, H. and {Ginski}, C. and {de Kok}, R.~J. and {Snellen}, I.~A.~G. and 
	{Brogi}, M. and {Birkby}, J.~L.},
    title = "{The slow spin of the young sub-stellar companion GQ Lupi b and its orbital configuration}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1607.00012},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics},
     year = 2016,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160700012S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bil15,
   author = {{Biller}, B.~A. and {Vos}, J. and {Bonavita}, M. and {Buenzli}, E. and 
	{Baxter}, C. and {Crossfield}, I.~J.~M. and {Allers}, K. and 
	{Liu}, M.~C. and {Bonnefoy}, M. and {Deacon}, N. and {Brandner}, W. and 
	{Schlieder}, J.~E. and {Dupuy}, T. and {Kopytova}, T. and {Manjavacas}, E. and 
	{Allard}, F. and {Homeier}, D. and {Henning}, T.},
    title = "{Variability in a Young, L/T Transition Planetary-mass Object}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1510.07625},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, planets and satellites: atmospheres, planets and satellites: gaseous planets},
     year = 2015,
    month = nov,
   volume = 813,
      eid = {L23},
    pages = {L23},
      doi = {10.1088/2041-8205/813/2/L23},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...813L..23B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bil13,
   author = {{Biller}, B.~A. and {Crossfield}, I.~J.~M. and {Mancini}, L. and 
	{Ciceri}, S. and {Southworth}, J. and {Kopytova}, T.~G. and 
	{Bonnefoy}, M. and {Deacon}, N.~R. and {Schlieder}, J.~E. and 
	{Buenzli}, E. and {Brandner}, W. and {Allard}, F. and {Homeier}, D. and 
	{Freytag}, B. and {Bailer-Jones}, C.~A.~L. and {Greiner}, J. and 
	{Henning}, T. and {Goldman}, B.},
    title = "{Weather on the Nearest Brown Dwarfs: Resolved Simultaneous Multi-wavelength Variability Monitoring of WISE J104915.57-531906.1AB}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1310.5144},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: low-mass},
     year = 2013,
    month = nov,
   volume = 778,
      eid = {L10},
    pages = {L10},
      doi = {10.1088/2041-8205/778/1/L10},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...778L..10B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zho16,
   author = {{Zhou}, Y. and {Apai}, D. and {Schneider}, G.~H. and {Marley}, M.~S. and 
	{Showman}, A.~P.},
    title = "{Discovery of Rotational Modulations in the Planetary-mass Companion 2M1207b: Intermediate Rotation Period and Heterogeneous Clouds in a Low Gravity Atmosphere}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1512.02706},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, planets and satellites: atmospheres, planets and satellites: individual: 2M1207b, techniques: photometric},
     year = 2016,
    month = feb,
   volume = 818,
      eid = {176},
    pages = {176},
      doi = {10.3847/0004-637X/818/2/176},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...818..176Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mar10,
   author = {{Marley}, M.~S. and {Saumon}, D. and {Goldblatt}, C.},
    title = "{A Patchy Cloud Model for the L to T Dwarf Transition}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1009.6217},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: atmospheres},
     year = 2010,
    month = nov,
   volume = 723,
    pages = {L117-L121},
      doi = {10.1088/2041-8205/723/1/L117},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...723L.117M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ske14,
   author = {{Skemer}, A.~J. and {Marley}, M.~S. and {Hinz}, P.~M. and {Morzinski}, K.~M. and 
	{Skrutskie}, M.~F. and {Leisenring}, J.~M. and {Close}, L.~M. and 
	{Saumon}, D. and {Bailey}, V.~P. and {Briguglio}, R. and {Defrere}, D. and 
	{Esposito}, S. and {Follette}, K.~B. and {Hill}, J.~M. and {Males}, J.~R. and 
	{Puglisi}, A. and {Rodigas}, T.~J. and {Xompero}, M.},
    title = "{Directly Imaged L-T Transition Exoplanets in the Mid-infrared}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1311.2085},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, infrared: planetary systems, instrumentation: adaptive optics, planets and satellites: atmospheres, planets and satellites: gaseous planets, stars: individual: HR 8799 2M1207 b},
     year = 2014,
    month = sep,
   volume = 792,
      eid = {17},
    pages = {17},
      doi = {10.1088/0004-637X/792/1/17},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...792...17S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ske12,
   author = {{Skemer}, A.~J. and {Hinz}, P.~M. and {Esposito}, S. and {Burrows}, A. and 
	{Leisenring}, J. and {Skrutskie}, M. and {Desidera}, S. and 
	{Mesa}, D. and {Arcidiacono}, C. and {Mannucci}, F. and {Rodigas}, T.~J. and 
	{Close}, L. and {McCarthy}, D. and {Kulesa}, C. and {Agapito}, G. and 
	{Apai}, D. and {Argomedo}, J. and {Bailey}, V. and {Boutsia}, K. and 
	{Briguglio}, R. and {Brusa}, G. and {Busoni}, L. and {Claudi}, R. and 
	{Eisner}, J. and {Fini}, L. and {Follette}, K.~B. and {Garnavich}, P. and 
	{Gratton}, R. and {Guerra}, J.~C. and {Hill}, J.~M. and {Hoffmann}, W.~F. and 
	{Jones}, T. and {Krejny}, M. and {Males}, J. and {Masciadri}, E. and 
	{Meyer}, M.~R. and {Miller}, D.~L. and {Morzinski}, K. and {Nelson}, M. and 
	{Pinna}, E. and {Puglisi}, A. and {Quanz}, S.~P. and {Quiros-Pacheco}, F. and 
	{Riccardi}, A. and {Stefanini}, P. and {Vaitheeswaran}, V. and 
	{Wilson}, J.~C. and {Xompero}, M.},
    title = "{First Light LBT AO Images of HR 8799 bcde at 1.6 and 3.3 {$\mu$}m: New Discrepancies between Young Planets and Old Brown Dwarfs}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1203.2615},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, instrumentation: adaptive optics, planetary systems, planets and satellites: atmospheres, stars: individual: HR 8799},
     year = 2012,
    month = jul,
   volume = 753,
      eid = {14},
    pages = {14},
      doi = {10.1088/0004-637X/753/1/14},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...753...14S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Luh13,
   author = {{Luhman}, K.~L.},
    title = "{Discovery of a Binary Brown Dwarf at 2 pc from the Sun}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1303.2401},
 keywords = {brown dwarfs, infrared: stars, proper motions, solar neighborhood, stars: low-mass},
     year = 2013,
    month = apr,
   volume = 767,
      eid = {L1},
    pages = {L1},
      doi = {10.1088/2041-8205/767/1/L1},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...767L...1L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...783L..17Z,
   author = {{Zhou}, Y. and {Herczeg}, G.~J. and {Kraus}, A.~L. and {Metchev}, S. and 
	{Cruz}, K.~L.},
    title = "{Accretion onto Planetary Mass Companions of Low-mass Young Stars}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1401.6545},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, brown dwarfs, protoplanetary disks, stars: low-mass, stars: pre-main sequence},
     year = 2014,
    month = mar,
   volume = 783,
      eid = {L17},
    pages = {L17},
      doi = {10.1088/2041-8205/783/1/L17},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...783L..17Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gil13,
   author = {{Gillon}, M. and {Triaud}, A.~H.~M.~J. and {Jehin}, E. and {Delrez}, L. and 
	{Opitom}, C. and {Magain}, P. and {Lendl}, M. and {Queloz}, D.
	},
    title = "{Fast-evolving weather for the coolest of our two new substellar neighbours}",
  journal = \aap,
archivePrefix = "arXiv",
   eprint = {1304.0481},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: individual: WISE-J104915.57-531906.1, solar neighborhood, techniques: photometric},
     year = 2013,
    month = jul,
   volume = 555,
      eid = {L5},
    pages = {L5},
      doi = {10.1051/0004-6361/201321620},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...555L...5G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bur13,
   author = {{Burgasser}, A.~J. and {Sheppard}, S.~S. and {Luhman}, K.~L.
	},
    title = "{Resolved Near-infrared Spectroscopy of WISE J104915.57-531906.1AB: A Flux-reversal Binary at the L dwarf/T Dwarf Transition}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1303.7283},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: visual, brown dwarfs, stars: individual: WISE J104915.57{\ndash}531906.1, stars: low-mass},
     year = 2013,
    month = aug,
   volume = 772,
      eid = {129},
    pages = {129},
      doi = {10.1088/0004-637X/772/2/129},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...772..129B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Met15,
   author = {{Metchev}, S.~A. and {Heinze}, A. and {Apai}, D. and {Flateau}, D. and 
	{Radigan}, J. and {Burgasser}, A. and {Marley}, M.~S. and {Artigau}, {\'E}. and 
	{Plavchan}, P. and {Goldman}, B.},
    title = "{Weather on Other Worlds. II. Survey Results: Spots are Ubiquitous on L and T Dwarfs}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1411.3051},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: low-mass, stars: rotation, starspots, stars: variables: general, techniques: photometric},
     year = 2015,
    month = feb,
   volume = 799,
      eid = {154},
    pages = {154},
      doi = {10.1088/0004-637X/799/2/154},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...799..154M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bue15b,
   author = {{Buenzli}, E. and {Marley}, M.~S. and {Apai}, D. and {Saumon}, D. and 
	{Biller}, B.~A. and {Crossfield}, I.~J.~M. and {Radigan}, J.
	},
    title = "{Cloud Structure of the Nearest Brown Dwarfs. II. High-amplitude Variability for Luhman 16 A and B in and out of the 0.99 {$\mu$}m FeH feature}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1509.06148},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: visual, brown dwarfs, stars: atmospheres, stars: individual: WISE J104915.57{\ndash}531906.1, Luhman 16AB, stars: variables: general},
     year = 2015,
    month = oct,
   volume = 812,
      eid = {163},
    pages = {163},
      doi = {10.1088/0004-637X/812/2/163},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...812..163B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bue15a,
   author = {{Buenzli}, E. and {Saumon}, D. and {Marley}, M.~S. and {Apai}, D. and 
	{Radigan}, J. and {Bedin}, L.~R. and {Reid}, I.~N. and {Morley}, C.~V.
	},
    title = "{Cloud Structure of the Nearest Brown Dwarfs: Spectroscopic Variability of Luhman 16AB from the Hubble Space Telescope}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1411.0003},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: visual, brown dwarfs, stars: atmospheres, stars: individual: WISE J104915.57-531906.1 Luhman 16AB, stars: variables: general},
     year = 2015,
    month = jan,
   volume = 798,
      eid = {127},
    pages = {127},
      doi = {10.1088/0004-637X/798/2/127},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798..127B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bue14,
   author = {{Buenzli}, E. and {Apai}, D. and {Radigan}, J. and {Reid}, I.~N. and 
	{Flateau}, D.},
    title = "{Brown Dwarf Photospheres are Patchy: A Hubble Space Telescope Near-infrared Spectroscopic Survey Finds Frequent Low-level Variability}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1312.5294},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: atmospheres, stars: low-mass},
     year = 2014,
    month = feb,
   volume = 782,
      eid = {77},
    pages = {77},
      doi = {10.1088/0004-637X/782/2/77},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...782...77B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bue12,
   author = {{Buenzli}, E. and {Apai}, D. and {Morley}, C.~V. and {Flateau}, D. and 
	{Showman}, A.~P. and {Burrows}, A. and {Marley}, M.~S. and {Lewis}, N.~K. and 
	{Reid}, I.~N.},
    title = "{Vertical Atmospheric Structure in a Variable Brown Dwarf: Pressure-dependent Phase Shifts in Simultaneous Hubble Space Telescope-Spitzer Light Curves}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1210.6654},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: atmospheres, stars: individual: 2MASS J22282889{\ndash}4310262, stars: variables: general},
     year = 2012,
    month = dec,
   volume = 760,
      eid = {L31},
    pages = {L31},
      doi = {10.1088/2041-8205/760/2/L31},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...760L..31B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rad14b,
   author = {{Radigan}, J.},
    title = "{An Independent Analysis of the Brown Dwarf Atmosphere Monitoring (BAM) Data: Large-amplitude Variability is Rare Outside the L/T Transition}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1408.5919},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: atmospheres, stars: variables: general},
     year = 2014,
    month = dec,
   volume = 797,
      eid = {120},
    pages = {120},
      doi = {10.1088/0004-637X/797/2/120},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...797..120R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rad14a,
   author = {{Radigan}, J. and {Lafreni{\`e}re}, D. and {Jayawardhana}, R. and 
	{Artigau}, E.},
    title = "{Strong Brightness Variations Signal Cloudy-to-clear Transition of Brown Dwarfs}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1404.3247},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: variables: general},
     year = 2014,
    month = oct,
   volume = 793,
      eid = {75},
    pages = {75},
      doi = {10.1088/0004-637X/793/2/75},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...793...75R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rad12,
   author = {{Radigan}, J. and {Jayawardhana}, R. and {Lafreni{\`e}re}, D. and 
	{Artigau}, {\'E}. and {Marley}, M. and {Saumon}, D.},
    title = "{Large-amplitude Variations of an L/T Transition Brown Dwarf: Multi-wavelength Observations of Patchy, High-contrast Cloud Features}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1201.3403},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: individual: 2MASS J21392676+0220226, stars: variables: general},
     year = 2012,
    month = may,
   volume = 750,
      eid = {105},
    pages = {105},
      doi = {10.1088/0004-637X/750/2/105},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...750..105R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wil14,
   author = {{Wilson}, P.~A. and {Rajan}, A. and {Patience}, J.},
    title = "{The brown dwarf atmosphere monitoring (BAM) project. I. The largest near-IR monitoring survey of L and T dwarfs}",
  journal = \aap,
archivePrefix = "arXiv",
   eprint = {1404.4633},
 primaryClass = "astro-ph.SR",
 keywords = {techniques: photometric, brown dwarfs, stars: low-mass, stars: atmospheres},
     year = 2014,
    month = jun,
   volume = 566,
      eid = {A111},
    pages = {A111},
      doi = {10.1051/0004-6361/201322995},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...566A.111W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bai03,
   author = {{Bailer-Jones}, C.~A.~L. and {Lamm}, M.},
    title = "{Limits on the infrared photometric monitoring of brown dwarfs}",
  journal = \mnras,
   eprint = {astro-ph/0210413},
 keywords = {methods: data analysis, techniques: photometric, stars: individual: 2MASSW J1439284+192915, stars: individual: SDSSp J12035819+001550.33, stars: individual: 2MASSW J1112257+354813, stars: low-mass, brown dwarfs},
     year = 2003,
    month = feb,
   volume = 339,
    pages = {477-485},
      doi = {10.1046/j.1365-8711.2003.06189.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.339..477B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cla03,
   author = {{Clarke}, F.~J. and {Tinney}, C.~G. and {Hodgkin}, S.~T.},
    title = "{Time-resolved spectroscopy of the variable brown dwarf Kelu-1$^{*}$}",
  journal = \mnras,
   eprint = {astro-ph/0301155},
 keywords = {techniques: photometric, techniques: spectroscopic, stars: individual: Kelu-1, stars: low-mass, brown dwarfs},
     year = 2003,
    month = may,
   volume = 341,
    pages = {239-246},
      doi = {10.1046/j.1365-8711.2003.06405.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.341..239C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eno03,
   author = {{Enoch}, M.~L. and {Brown}, M.~E. and {Burgasser}, A.~J.},
    title = "{Photometric Variability at the L/T Dwarf Boundary}",
  journal = \aj,
   eprint = {astro-ph/0305048},
 keywords = {stars: individual (2MASSW J0030300-145033), stars: individual (SDSSp J015141.69+124429.6), Stars: Low-Mass, Brown Dwarfs, Stars: Variables: Other},
     year = 2003,
    month = aug,
   volume = 126,
    pages = {1006-1016},
      doi = {10.1086/376598},
   adsurl = {http://adsabs.harvard.edu/abs/2003AJ....126.1006E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zap03,
   author = {{Zapatero Osorio}, M.~R. and {Caballero}, J.~A. and {B{\'e}jar}, V.~J.~S. and 
	{Rebolo}, R.},
    title = "{Photometric variability of a young, low-mass brown dwarf}",
  journal = \aap,
   eprint = {astro-ph/0306398},
 keywords = {stars: low mass, brown dwarfs, stars: rotation, stars: pre-main sequence, stars: formation},
     year = 2003,
    month = sep,
   volume = 408,
    pages = {663-673},
      doi = {10.1051/0004-6361:20030987},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...408..663Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Joe03,
   author = {{Joergens}, V. and {Fern{\'a}ndez}, M. and {Carpenter}, J.~M. and 
	{Neuh{\"a}user}, R.},
    title = "{Rotational Periods of Very Young Brown Dwarfs and Very Low Mass Stars in Chamaeleon I}",
  journal = \apj,
   eprint = {astro-ph/0305397},
 keywords = {Stars: Activity, Stars: Fundamental Parameters, Stars: Individual: Constellation Name: Chamaeleon H{$\alpha$} 1, Stars: Individual: Constellation Name: Chamaeleon H{$\alpha$} 2, Stars: Individual: Constellation Name: Chamaeleon H{$\alpha$} 3, stars: individual (Chamaeleon H{$\alpha$} 4, Chamaeleon H{$\alpha$} 5), Stars: Individual: Constellation Name: Chamaeleon H{$\alpha$} 6, stars: individual (Chamaeleon H{$\alpha$} 7, Chamaeleon H{$\alpha$} 8), Stars: Individual: Constellation Name: Chamaeleon H{$\alpha$} 9, stars: individual (Chamaeleon H{$\alpha$} 10, Chamaeleon H{$\alpha$} 11), Stars: Individual: Constellation Name: Chamaeleon H{$\alpha$} 12, Stars: Individual: Alphanumeric: B34, stars: individual (CHXR 73), stars: individual (CHXR 78C), Stars: Late-Type, Stars: Low-Mass, Brown Dwarfs, Stars: Rotation},
     year = 2003,
    month = sep,
   volume = 594,
    pages = {971-981},
      doi = {10.1086/377041},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...594..971J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Koe03,
   author = {{Koen}, C.},
    title = "{A search for short time-scale I-band variability in ultracool dwarfs}",
  journal = \mnras,
 keywords = {stars: individual: 2MASS J1155395-372735, stars: low-mass, brown dwarfs, stars: variables: other},
     year = 2003,
    month = dec,
   volume = 346,
    pages = {473-482},
      doi = {10.1046/j.1365-2966.2003.07099.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.346..473K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sch04,
   author = {{Scholz}, A. and {Eisl{\"o}ffel}, J.},
    title = "{Rotation and accretion of very low mass objects in the {$\sigma$} Ori cluster}",
  journal = \aap,
   eprint = {astro-ph/0404014},
 keywords = {techniques: photometric, stars: low-mass, brown dwarfs, stars: rotation, stars: formation, stars: activity, stars: magnetic fields},
     year = 2004,
    month = may,
   volume = 419,
    pages = {249-267},
      doi = {10.1051/0004-6361:20034022},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...419..249S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bai04,
   author = {{Bailer-Jones}, C.~A.~L.},
    title = "{Spectroscopic rotation velocities of L dwarfs from VLT/UVES and their comparison with periods from photometric monitoring}",
  journal = \aap,
   eprint = {astro-ph/0403013},
 keywords = {techniques: spectroscopic, stars: low-mass, brown dwarfs, stars: variables: general, stars: rotation},
     year = 2004,
    month = may,
   volume = 419,
    pages = {703-712},
      doi = {10.1051/0004-6361:20040965},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...419..703B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cab04,
   author = {{Caballero}, J.~A. and {B{\'e}jar}, V.~J.~S. and {Rebolo}, R. and 
	{Zapatero Osorio}, M.~R.},
    title = "{Photometric variability of young brown dwarfs  in the {$\sigma$} Orionis open cluster}",
  journal = \aap,
   eprint = {astro-ph/0406341},
 keywords = {stars: low mass, brown dwarfs, Galaxy: open clusters and associations: individual: {$\sigma$} Orionis, techniques: photometric},
     year = 2004,
    month = sep,
   volume = 424,
    pages = {857-872},
      doi = {10.1051/0004-6361:20047048},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...424..857C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Koe04,
   author = {{Koen}, C. and {Matsunaga}, N. and {Menzies}, J.},
    title = "{A search for short time-scale JHK variability in ultracool dwarfs}",
  journal = \mnras,
 keywords = {stars: low-mass, brown dwarfs, stars: variables: other},
     year = 2004,
    month = oct,
   volume = 354,
    pages = {466-476},
      doi = {10.1111/j.1365-2966.2004.08208.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.354..466K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mai05,
   author = {{Maiti}, M. and {Sengupta}, S. and {Parihar}, P.~S. and {Anupama}, G.~C.
	},
    title = "{Observation of R-Band Variability of L Dwarfs}",
  journal = \apjl,
   eprint = {astro-ph/0412409},
 keywords = {Stars: Atmospheres, Stars: Low-Mass, Brown Dwarfs},
     year = 2005,
    month = feb,
   volume = 619,
    pages = {L183-L186},
      doi = {10.1086/428088},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...619L.183M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Koe05,
   author = {{Koen}, C.},
    title = "{I$_{C}$ and R$_{C}$ band time-series observations of some bright ultracool dwarfs}",
  journal = \mnras,
 keywords = {stars: low mass, brown dwarfs, stars: variables: other},
     year = 2005,
    month = jul,
   volume = 360,
    pages = {1132-1142},
      doi = {10.1111/j.1365-2966.2005.09119.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.360.1132K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Koe05b,
   author = {{Koen}, C. and {Tanab{\'e}}, T. and {Tamura}, M. and {Kusakabe}, N.
	},
    title = "{JHK$_{s}$ time-series observations of a few ultracool dwarfs}",
  journal = \mnras,
 keywords = {techniques: photometric, stars: individual: {$\epsilon$} Indi Bab, stars: individual: SSSPM J0109-5101, stars: low-mass, brown dwarfs, stars: variables: other},
     year = 2005,
    month = sep,
   volume = 362,
    pages = {727-736},
      doi = {10.1111/j.1365-2966.2005.09280.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.362..727K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gol05,
   author = {{Goldman}, B.},
    title = "{Ultra-cool dwarf variability}",
  journal = {Astronomische Nachrichten},
 keywords = {stars: low-mass, brown dwarfs, stars: variables: other},
     year = 2005,
    month = dec,
   volume = 326,
    pages = {1059-1064},
      doi = {10.1002/asna.200510474},
   adsurl = {http://adsabs.harvard.edu/abs/2005AN....326.1059G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Koe06,
   author = {{Koen}, C.},
    title = "{Evidence for rapid evolution of periodic variations in an ultracool dwarf}",
  journal = \mnras,
 keywords = {stars: low mass, brown dwarfs, stars: variables: other},
     year = 2006,
    month = apr,
   volume = 367,
    pages = {1735-1738},
      doi = {10.1111/j.1365-2966.2006.10059.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.367.1735K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lit06,
   author = {{Littlefair}, S.~P. and {Dhillon}, V.~S. and {Marsh}, T.~R. and 
	{Shahbaz}, T. and {Mart{\'{\i}}n}, E.~L.},
    title = "{Observations of ultracool dwarfs with ULTRACAM on the VLT: a search for weather}",
  journal = \mnras,
   eprint = {astro-ph/0605225},
 keywords = {stars: individual: Kelu-1: stars: individual: 2MASS 1300+1912: stars: individual: 2MASS 2057-0252: stars: individual: DENIS 1441-0945: stars: low-mass, brown dwarfs, stars: individual: Kelu-1, stars: individual: 2MASS 1300+1912, stars: individual: 2MASS 2057-0252, stars: individual: DENIS 1441-0945, stars: low-mass},
     year = 2006,
    month = aug,
   volume = 370,
    pages = {1208-1212},
      doi = {10.1111/j.1365-2966.2006.10523.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370.1208L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mor06,
   author = {{Morales-Calder{\'o}n}, M. and {Stauffer}, J.~R. and {Kirkpatrick}, J.~D. and 
	{Carey}, S. and {Gelino}, C.~R. and {Barrado y Navascu{\'e}s}, D. and 
	{Rebull}, L. and {Lowrance}, P. and {Marley}, M.~S. and {Charbonneau}, D. and 
	{Patten}, B.~M. and {Megeath}, S.~T. and {Buzasi}, D.},
    title = "{A Sensitive Search for Variability in Late L Dwarfs: The Quest for Weather}",
  journal = \apj,
   eprint = {astro-ph/0607537},
 keywords = {stars: individual (DENIS-P J0255-4700), stars: individual (2MASS J0908+5032), stars: individual (2MASS J2244+2043), Stars: Low-Mass, Brown Dwarfs, Stars: Variables: Other},
     year = 2006,
    month = dec,
   volume = 653,
    pages = {1454-1463},
      doi = {10.1086/507866},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...653.1454M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mai07,
   author = {{Maiti}, M.},
    title = "{Observational Evidence of Optical Variability in L Dwarfs}",
  journal = \aj,
 keywords = {stars: low-mass, brown dwarfs, stars: rotation, stars: variables: other},
     year = 2007,
    month = apr,
   volume = 133,
    pages = {1633-1644},
      doi = {10.1086/511956},
   adsurl = {http://adsabs.harvard.edu/abs/2007AJ....133.1633M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Art09,
   author = {{Artigau}, {\'E}. and {Bouchard}, S. and {Doyon}, R. and {Lafreni{\`e}re}, D.
	},
    title = "{Photometric Variability of the T2.5 Brown Dwarf SIMP J013656.5+093347: Evidence for Evolving Weather Patterns}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {0906.3514},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: SIMP J013656.5+093347, stars: low-mass, brown dwarfs},
     year = 2009,
    month = aug,
   volume = 701,
    pages = {1534-1539},
      doi = {10.1088/0004-637X/701/2/1534},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...701.1534A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Art06,
   author = {{Artigau}, {\'E}. and {Doyon}, R. and {Lafreni{\`e}re}, D. and 
	{Nadeau}, D. and {Robert}, J. and {Albert}, L.},
    title = "{Discovery of the Brightest T Dwarf in the Northern Hemisphere}",
  journal = \apjl,
   eprint = {astro-ph/0609419},
 keywords = {stars: individual (SIMP J013656.5+093347), Stars: Low-Mass, Brown Dwarfs},
     year = 2006,
    month = nov,
   volume = 651,
    pages = {L57-L60},
      doi = {10.1086/509146},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...651L..57A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Cus16,
   author = {{Cushing}, M.~C. and {Hardegree-Ullman}, K.~K. and {Trucks}, J.~L. and 
	{Morley}, C.~V. and {Gizis}, J.~E. and {Marley}, M.~S. and {Fortney}, J.~J. and 
	{Kirkpatrick}, J.~D. and {Gelino}, C.~R. and {Mace}, G.~N. and 
	{Carey}, S.~J.},
    title = "{The First Detection of Photometric Variability in a Y Dwarf: WISE J140518.39+553421.3}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1602.06321},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, infrared: stars, stars: individual: WISE J140518.39+553421.3, stars: low-mass },
     year = 2016,
    month = jun,
   volume = 823,
      eid = {152},
    pages = {152},
      doi = {10.3847/0004-637X/823/2/152},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...823..152C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hei15,
   author = {{Heinze}, A.~N. and {Metchev}, S. and {Kellogg}, K.},
    title = "{Weather on Other Worlds. III. A Survey for T Dwarfs with High-amplitude Optical Variability}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1412.6733},
 primaryClass = "astro-ph.SR",
 keywords = {atmospheric effects, brown dwarfs, stars: individual: 2MASS J16291840+0335371 2MASS 13243559+6358284, stars: variables: general, techniques: photometric},
     year = 2015,
    month = mar,
   volume = 801,
      eid = {104},
    pages = {104},
      doi = {10.1088/0004-637X/801/2/104},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...801..104H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kha13,
   author = {{Khandrika}, H. and {Burgasser}, A.~J. and {Melis}, C. and {Luk}, C. and 
	{Bowsher}, E. and {Swift}, B.},
    title = "{A Search for Photometric Variability in L- and T-type Brown Dwarf Atmospheres}",
  journal = \aj,
archivePrefix = "arXiv",
   eprint = {1301.0545},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, infrared: stars, stars: low-mass},
     year = 2013,
    month = mar,
   volume = 145,
      eid = {71},
    pages = {71},
      doi = {10.1088/0004-6256/145/3/71},
   adsurl = {http://adsabs.harvard.edu/abs/2013AJ....145...71K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Raj15,
   author = {{Rajan}, A. and {Patience}, J. and {Wilson}, P.~A. and {Bulger}, J. and 
	{De Rosa}, R.~J. and {Ward-Duong}, K. and {Morley}, C. and {Pont}, F. and 
	{Windhorst}, R.},
    title = "{The brown dwarf atmosphere monitoring (BAM) project - II. Multi-epoch monitoring of extremely cool brown dwarfs}",
  journal = \mnras,
archivePrefix = "arXiv",
   eprint = {1502.01346},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: low-mass, stars: variables: general},
     year = 2015,
    month = apr,
   volume = 448,
    pages = {3775-3783},
      doi = {10.1093/mnras/stv181},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.448.3775R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mac14,
   author = {{Macintosh}, B. and {Graham}, J.~R. and {Ingraham}, P. and {Konopacky}, Q. and 
	{Marois}, C. and {Perrin}, M. and {Poyneer}, L. and {Bauman}, B. and 
	{Barman}, T. and {Burrows}, A.~S. and {Cardwell}, A. and {Chilcote}, J. and 
	{De Rosa}, R.~J. and {Dillon}, D. and {Doyon}, R. and {Dunn}, J. and 
	{Erikson}, D. and {Fitzgerald}, M.~P. and {Gavel}, D. and {Goodsell}, S. and 
	{Hartung}, M. and {Hibon}, P. and {Kalas}, P. and {Larkin}, J. and 
	{Maire}, J. and {Marchis}, F. and {Marley}, M.~S. and {McBride}, J. and 
	{Millar-Blanchaer}, M. and {Morzinski}, K. and {Norton}, A. and 
	{Oppenheimer}, B.~R. and {Palmer}, D. and {Patience}, J. and 
	{Pueyo}, L. and {Rantakyro}, F. and {Sadakuni}, N. and {Saddlemyer}, L. and 
	{Savransky}, D. and {Serio}, A. and {Soummer}, R. and {Sivaramakrishnan}, A. and 
	{Song}, I. and {Thomas}, S. and {Wallace}, J.~K. and {Wiktorowicz}, S. and 
	{Wolff}, S.},
    title = "{First light of the Gemini Planet Imager}",
  journal = {Proceedings of the National Academy of Science},
archivePrefix = "arXiv",
   eprint = {1403.7520},
 primaryClass = "astro-ph.EP",
     year = 2014,
    month = sep,
   volume = 111,
    pages = {12661-12666},
      doi = {10.1073/pnas.1304215111},
   adsurl = {http://adsabs.harvard.edu/abs/2014PNAS..11112661M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Beu08,
   author = {{Beuzit}, J.-L. and {Feldt}, M. and {Dohlen}, K. and {Mouillet}, D. and 
	{Puget}, P. and {Wildi}, F. and {Abe}, L. and {Antichi}, J. and 
	{Baruffolo}, A. and {Baudoz}, P. and {Boccaletti}, A. and {Carbillet}, M. and 
	{Charton}, J. and {Claudi}, R. and {Downing}, M. and {Fabron}, C. and 
	{Feautrier}, P. and {Fedrigo}, E. and {Fusco}, T. and {Gach}, J.-L. and 
	{Gratton}, R. and {Henning}, T. and {Hubin}, N. and {Joos}, F. and 
	{Kasper}, M. and {Langlois}, M. and {Lenzen}, R. and {Moutou}, C. and 
	{Pavlov}, A. and {Petit}, C. and {Pragt}, J. and {Rabou}, P. and 
	{Rigal}, F. and {Roelfsema}, R. and {Rousset}, G. and {Saisse}, M. and 
	{Schmid}, H.-M. and {Stadler}, E. and {Thalmann}, C. and {Turatto}, M. and 
	{Udry}, S. and {Vakili}, F. and {Waters}, R.},
    title = "{SPHERE: a 'Planet Finder' instrument for the VLT}",
booktitle = {Ground-based and Airborne Instrumentation for Astronomy II},
     year = 2008,
   series = \procspie,
   volume = 7014,
    month = jul,
      eid = {701418},
    pages = {701418},
      doi = {10.1117/12.790120},
   adsurl = {http://adsabs.harvard.edu/abs/2008SPIE.7014E..18B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gag15b,
   author = {{Gagn{\'e}}, J. and {Faherty}, J.~K. and {Cruz}, K.~L. and {Lafreni{\'e}re}, D. and 
	{Doyon}, R. and {Malo}, L. and {Burgasser}, A.~J. and {Naud}, M.-E. and 
	{Artigau}, {\'E}. and {Bouchard}, S. and {Gizis}, J.~E. and 
	{Albert}, L.},
    title = "{BANYAN. VII. A New Population of Young Substellar Candidate Members of Nearby Moving Groups from the BASS Survey}",
  journal = \apjs,
archivePrefix = "arXiv",
   eprint = {1506.07712},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, methods: data analysis, proper motions, stars: kinematics and dynamics, stars: low-mass},
     year = 2015,
    month = aug,
   volume = 219,
      eid = {33},
    pages = {33},
      doi = {10.1088/0067-0049/219/2/33},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJS..219...33G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gag15a,
   author = {{Gagn{\'e}}, J. and {Lafreni{\`e}re}, D. and {Doyon}, R. and 
	{Malo}, L. and {Artigau}, {\'E}.},
    title = "{BANYAN. V. A Systematic All-sky Survey for New Very Late-type Low-mass Stars and Brown Dwarfs in Nearby Young Moving Groups}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1410.4864},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, methods: data analysis, proper motions, stars: kinematics and dynamics, stars: low-mass},
     year = 2015,
    month = jan,
   volume = 798,
      eid = {73},
    pages = {73},
      doi = {10.1088/0004-637X/798/2/73},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798...73G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gag14,
   author = {{Gagn{\'e}}, J. and {Lafreni{\`e}re}, D. and {Doyon}, R. and 
	{Malo}, L. and {Artigau}, {\'E}.},
    title = "{BANYAN. II. Very Low Mass and Substellar Candidate Members to Nearby, Young Kinematic Groups with Previously Known Signs of Youth}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1312.5864},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, methods: data analysis, open clusters and associations: general, proper motions, stars: kinematics and dynamics, stars: low-mass },
     year = 2014,
    month = mar,
   volume = 783,
      eid = {121},
    pages = {121},
      doi = {10.1088/0004-637X/783/2/121},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...783..121G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fah16,
   author = {{Faherty}, J.~K. and {Riedel}, A.~R. and {Cruz}, K.~L. and {Gagne}, J. and 
	{Filippazzo}, J.~C. and {Lambrides}, E. and {Fica}, H. and {Weinberger}, A. and 
	{Thorstensen}, J.~R. and {Tinney}, C.~G. and {Baldassare}, V. and 
	{Lemonier}, E. and {Rice}, E.~L.},
    title = "{Population Properties of Brown Dwarf Analogs to Exoplanets}",
  journal = \apjs,
archivePrefix = "arXiv",
   eprint = {1605.07927},
 primaryClass = "astro-ph.SR",
 keywords = {astrometry, brown dwarfs, stars: low-mass },
     year = 2016,
    month = jul,
   volume = 225,
      eid = {10},
    pages = {10},
      doi = {10.3847/0067-0049/225/1/10},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJS..225...10F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cro14a,
   author = {{Crossfield}, I.~J.~M. and {Biller}, B. and {Schlieder}, J.~E. and 
	{Deacon}, N.~R. and {Bonnefoy}, M. and {Homeier}, D. and {Allard}, F. and 
	{Buenzli}, E. and {Henning}, T. and {Brandner}, W. and {Goldman}, B. and 
	{Kopytova}, T.},
    title = "{A global cloud map of the nearest known brown dwarf}",
  journal = \nat,
archivePrefix = "arXiv",
   eprint = {1401.8145},
 primaryClass = "astro-ph.EP",
     year = 2014,
    month = jan,
   volume = 505,
    pages = {654-656},
      doi = {10.1038/nature12955},
   adsurl = {http://adsabs.harvard.edu/abs/2014Natur.505..654C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gir13,
   author = {{Girardin}, F. and {Artigau}, {\'E}. and {Doyon}, R.},
    title = "{In Search of Dust Clouds: Photometric Monitoring of a Sample of Late L and T Dwarfs}",
  journal = \apj,
 keywords = {brown dwarfs, stars: individual: SDSS J105213.51+442255.7 SDSSp J125453.90{\ndash}012247.4, stars: low-mass, stars: variables: general, techniques: photometric},
     year = 2013,
    month = apr,
   volume = 767,
      eid = {61},
    pages = {61},
      doi = {10.1088/0004-637X/767/1/61},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...767...61G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Str15,
   author = {{Street}, R.~A. and {Fulton}, B.~J. and {Scholz}, A. and {Horne}, K. and 
	{Helling}, C. and {Juncher}, D. and {Lee}, G. and {Valenti}, S.
	},
    title = "{Extended Baseline Photometry of Rapidly Changing Weather Patterns on the Brown Dwarf Binary Luhman-16}",
  journal = \apj,
 keywords = {brown dwarfs, stars: general, stars: individual: Luhman-16, WISE-J1049-0053, stars: low-mass},
     year = 2015,
    month = oct,
   volume = 812,
      eid = {161},
    pages = {161},
      doi = {10.1088/0004-637X/812/2/161},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...812..161S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Man15,
   author = {{Mancini}, L. and {Giacobbe}, P. and {Littlefair}, S.~P. and 
	{Southworth}, J. and {Bozza}, V. and {Damasso}, M. and {Dominik}, M. and 
	{Hundertmark}, M. and {J{\o}rgensen}, U.~G. and {Juncher}, D. and 
	{Popovas}, A. and {Rabus}, M. and {Rahvar}, S. and {Schmidt}, R.~W. and 
	{Skottfelt}, J. and {Snodgrass}, C. and {Sozzetti}, A. and {Alsubai}, K. and 
	{Bramich}, D.~M. and {Calchi Novati}, S. and {Ciceri}, S. and 
	{D'Ago}, G. and {Figuera Jaimes}, R. and {Galianni}, P. and 
	{Gu}, S.-H. and {Harps{\o}e}, K. and {Haugb{\o}lle}, T. and 
	{Henning}, T. and {Hinse}, T.~C. and {Kains}, N. and {Korhonen}, H. and 
	{Scarpetta}, G. and {Starkey}, D. and {Surdej}, J. and {Wang}, X.-B. and 
	{Wertz}, O.},
    title = "{Rotation periods and astrometric motions of the Luhman 16AB brown dwarfs by high-resolution lucky-imaging monitoring}",
  journal = \aap,
archivePrefix = "arXiv",
   eprint = {1510.08099},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: visual, brown dwarfs, stars: variables: general, techniques: photometric, techniques: image processing},
     year = 2015,
    month = dec,
   volume = 584,
      eid = {A104},
    pages = {A104},
      doi = {10.1051/0004-6361/201526899},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...584A.104M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Bur14,
   author = {{Burgasser}, A.~J.},
    title = "{The SpeX Prism Library: 1000+ low-resolution, near-infrared spectra of ultracool M, L, T and Y dwarfs}",
 keywords = {catalogs, stars: brown dwarfs, stars: low mass},
booktitle = {Astronomical Society of India Conference Series},
     year = 2014,
   series = {Astronomical Society of India Conference Series},
   volume = 11,
archivePrefix = "arXiv",
   eprint = {1406.4887},
 primaryClass = "astro-ph.SR",
   adsurl = {http://adsabs.harvard.edu/abs/2014ASInC..11....7B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bon16,
   author = {{Bonnefoy}, M. and {Zurlo}, A. and {Baudino}, J.~L. and {Lucas}, P. and 
	{Mesa}, D. and {Maire}, A.-L. and {Vigan}, A. and {Galicher}, R. and 
	{Homeier}, D. and {Marocco}, F. and {Gratton}, R. and {Chauvin}, G. and 
	{Allard}, F. and {Desidera}, S. and {Kasper}, M. and {Moutou}, C. and 
	{Lagrange}, A.-M. and {Antichi}, J. and {Baruffolo}, A. and 
	{Baudrand}, J. and {Beuzit}, J.-L. and {Boccaletti}, A. and 
	{Cantalloube}, F. and {Carbillet}, M. and {Charton}, J. and 
	{Claudi}, R.~U. and {Costille}, A. and {Dohlen}, K. and {Dominik}, C. and 
	{Fantinel}, D. and {Feautrier}, P. and {Feldt}, M. and {Fusco}, T. and 
	{Gigan}, P. and {Girard}, J.~H. and {Gluck}, L. and {Gry}, C. and 
	{Henning}, T. and {Janson}, M. and {Langlois}, M. and {Madec}, F. and 
	{Magnard}, Y. and {Maurel}, D. and {Mawet}, D. and {Meyer}, M.~R. and 
	{Milli}, J. and {Moeller-Nilsson}, O. and {Mouillet}, D. and 
	{Pavlov}, A. and {Perret}, D. and {Pujet}, P. and {Quanz}, S.~P. and 
	{Rochat}, S. and {Rousset}, G. and {Roux}, A. and {Salasnich}, B. and 
	{Salter}, G. and {Sauvage}, J.-F. and {Schmid}, H.~M. and {Sevin}, A. and 
	{Soenke}, C. and {Stadler}, E. and {Turatto}, M. and {Udry}, S. and 
	{Vakili}, F. and {Wahhaj}, Z. and {Wildi}, F.},
    title = "{First light of the VLT planet finder SPHERE. IV. Physical and chemical properties of the planets around HR8799}",
  journal = \aap,
archivePrefix = "arXiv",
   eprint = {1511.04082},
 primaryClass = "astro-ph.EP",
 keywords = {instrumentation: high angular resolution, stars: individual: HR8799, planets and satellites: atmospheres, planets and satellites: detection, techniques: imaging spectroscopy, planets and satellites: fundamental parameters},
     year = 2016,
    month = mar,
   volume = 587,
      eid = {A58},
    pages = {A58},
      doi = {10.1051/0004-6361/201526906},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...587A..58B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lee13,
   author = {{Lee}, J.-M. and {Heng}, K. and {Irwin}, P.~G.~J.},
    title = "{Atmospheric Retrieval Analysis of the Directly Imaged Exoplanet HR 8799b}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1307.1404},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: atmospheres},
     year = 2013,
    month = dec,
   volume = 778,
      eid = {97},
    pages = {97},
      doi = {10.1088/0004-637X/778/2/97},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...778...97L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vig08,
   author = {{Vigan}, A. and {Langlois}, M. and {Moutou}, C. and {Dohlen}, K.
	},
    title = "{Exoplanet characterization with long slit spectroscopy}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0808.3817},
 keywords = {techniques: spectroscopic, techniques: image processing, methods: data analysis, stars: planetary systems},
     year = 2008,
    month = oct,
   volume = 489,
    pages = {1345-1354},
      doi = {10.1051/0004-6361:200810090},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...489.1345V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Luh07,
   author = {{Luhman}, K.~L. and {Patten}, B.~M. and {Marengo}, M. and {Schuster}, M.~T. and 
	{Hora}, J.~L. and {Ellis}, R.~G. and {Stauffer}, J.~R. and {Sonnett}, S.~M. and 
	{Winston}, E. and {Gutermuth}, R.~A. and {Megeath}, S.~T. and 
	{Backman}, D.~E. and {Henry}, T.~J. and {Werner}, M.~W. and 
	{Fazio}, G.~G.},
    title = "{Discovery of Two T Dwarf Companions with the Spitzer Space Telescope}",
  journal = {\apj},
   eprint = {astro-ph/0609464},
 keywords = {Stars: Binaries: Visual, Infrared: Stars, Stars: Evolution, Stars: Fundamental Parameters, Stars: Low-Mass, Brown Dwarfs},
     year = 2007,
    month = jan,
   volume = 654,
    pages = {570-579},
      doi = {10.1086/509073},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...654..570L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zur16,
   author = {{Zurlo}, A. and {Vigan}, A. and {Galicher}, R. and {Maire}, A.-L. and 
	{Mesa}, D. and {Gratton}, R. and {Chauvin}, G. and {Kasper}, M. and 
	{Moutou}, C. and {Bonnefoy}, M. and {Desidera}, S. and {Abe}, L. and 
	{Apai}, D. and {Baruffolo}, A. and {Baudoz}, P. and {Baudrand}, J. and 
	{Beuzit}, J.-L. and {Blancard}, P. and {Boccaletti}, A. and 
	{Cantalloube}, F. and {Carle}, M. and {Cascone}, E. and {Charton}, J. and 
	{Claudi}, R.~U. and {Costille}, A. and {de Caprio}, V. and {Dohlen}, K. and 
	{Dominik}, C. and {Fantinel}, D. and {Feautrier}, P. and {Feldt}, M. and 
	{Fusco}, T. and {Gigan}, P. and {Girard}, J.~H. and {Gisler}, D. and 
	{Gluck}, L. and {Gry}, C. and {Henning}, T. and {Hugot}, E. and 
	{Janson}, M. and {Jaquet}, M. and {Lagrange}, A.-M. and {Langlois}, M. and 
	{Llored}, M. and {Madec}, F. and {Magnard}, Y. and {Martinez}, P. and 
	{Maurel}, D. and {Mawet}, D. and {Meyer}, M.~R. and {Milli}, J. and 
	{Moeller-Nilsson}, O. and {Mouillet}, D. and {Orign{\'e}}, A. and 
	{Pavlov}, A. and {Petit}, C. and {Puget}, P. and {Quanz}, S.~P. and 
	{Rabou}, P. and {Ramos}, J. and {Rousset}, G. and {Roux}, A. and 
	{Salasnich}, B. and {Salter}, G. and {Sauvage}, J.-F. and {Schmid}, H.~M. and 
	{Soenke}, C. and {Stadler}, E. and {Suarez}, M. and {Turatto}, M. and 
	{Udry}, S. and {Vakili}, F. and {Wahhaj}, Z. and {Wildi}, F. and 
	{Antichi}, J.},
    title = "{First light of the VLT planet finder SPHERE. III. New spectrophotometry and astrometry of the HR 8799 exoplanetary system}",
  journal = \aap,
archivePrefix = "arXiv",
   eprint = {1511.04083},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: image processing, astrometry, techniques: high angular resolution, techniques: spectroscopic, methods: data analysis},
     year = 2016,
    month = mar,
   volume = 587,
      eid = {A57},
    pages = {A57},
      doi = {10.1051/0004-6361/201526835},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...587A..57Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bon14,
   author = {{Bonnefoy}, M. and {Marleau}, G.-D. and {Galicher}, R. and {Beust}, H. and 
	{Lagrange}, A.-M. and {Baudino}, J.-L. and {Chauvin}, G. and 
	{Borgniet}, S. and {Meunier}, N. and {Rameau}, J. and {Boccaletti}, A. and 
	{Cumming}, A. and {Helling}, C. and {Homeier}, D. and {Allard}, F. and 
	{Delorme}, P.},
    title = "{Physical and orbital properties of {$\beta$} Pictoris b}",
  journal = \aap,
archivePrefix = "arXiv",
   eprint = {1407.4001},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: photometric, techniques: spectroscopic, planetary systems, stars: individual:{$\beta$}Pic},
     year = 2014,
    month = jul,
   volume = 567,
      eid = {L9},
    pages = {L9},
      doi = {10.1051/0004-6361/201424041},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...567L...9B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chi15,
   author = {{Chilcote}, J. and {Barman}, T. and {Fitzgerald}, M.~P. and 
	{Graham}, J.~R. and {Larkin}, J.~E. and {Macintosh}, B. and 
	{Bauman}, B. and {Burrows}, A.~S. and {Cardwell}, A. and {De Rosa}, R.~J. and 
	{Dillon}, D. and {Doyon}, R. and {Dunn}, J. and {Erikson}, D. and 
	{Gavel}, D. and {Goodsell}, S.~J. and {Hartung}, M. and {Hibon}, P. and 
	{Ingraham}, P. and {Kalas}, P. and {Konopacky}, Q. and {Maire}, J. and 
	{Marchis}, F. and {Marley}, M.~S. and {Marois}, C. and {Millar-Blanchaer}, M. and 
	{Morzinski}, K. and {Norton}, A. and {Oppenheimer}, R. and {Palmer}, D. and 
	{Patience}, J. and {Perrin}, M. and {Poyneer}, L. and {Pueyo}, L. and 
	{Rantakyr{\"o}}, F.~T. and {Sadakuni}, N. and {Saddlemyer}, L. and 
	{Savransky}, D. and {Serio}, A. and {Sivaramakrishnan}, A. and 
	{Song}, I. and {Soummer}, R. and {Thomas}, S. and {Wallace}, J.~K. and 
	{Wiktorowicz}, S. and {Wolff}, S.},
    title = "{The First H-band Spectrum of the Giant Planet {$\beta$} Pictoris b}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1407.4469},
 primaryClass = "astro-ph.EP",
 keywords = {infrared: general, instrumentation: adaptive optics, planetary systems, stars: individual: beta Pictoris, techniques: spectroscopic },
     year = 2015,
    month = jan,
   volume = 798,
      eid = {L3},
    pages = {L3},
      doi = {10.1088/2041-8205/798/1/L3},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798L...3C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeR16,
   author = {{De Rosa}, R.~J. and {Rameau}, J. and {Patience}, J. and {Graham}, J.~R. and 
	{Doyon}, R. and {Lafreni{\`e}re}, D. and {Macintosh}, B. and 
	{Pueyo}, L. and {Rajan}, A. and {Wang}, J.~J. and {Ward-Duong}, K. and 
	{Hung}, L.-W. and {Maire}, J. and {Nielsen}, E.~L. and {Ammons}, S.~M. and 
	{Bulger}, J. and {Cardwell}, A. and {Chilcote}, J.~K. and {Galvez}, R.~L. and 
	{Gerard}, B.~L. and {Goodsell}, S. and {Hartung}, M. and {Hibon}, P. and 
	{Ingraham}, P. and {Johnson-Groh}, M. and {Kalas}, P. and {Konopacky}, Q.~M. and 
	{Marchis}, F. and {Marois}, C. and {Metchev}, S. and {Morzinski}, K.~M. and 
	{Oppenheimer}, R. and {Perrin}, M.~D. and {Rantakyr{\"o}}, F.~T. and 
	{Savransky}, D. and {Thomas}, S.},
    title = "{Spectroscopic Characterization of HD 95086 b with the Gemini Planet Imager}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1604.01411},
 primaryClass = "astro-ph.EP",
 keywords = {infrared: planetary systems, instrumentation: adaptive optics, planets and satellites: atmospheres, stars: individual: HD 95086 },
     year = 2016,
    month = jun,
   volume = 824,
      eid = {121},
    pages = {121},
      doi = {10.3847/0004-637X/824/2/121},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...824..121D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ing14,
   author = {{Ingraham}, P. and {Marley}, M.~S. and {Saumon}, D. and {Marois}, C. and 
	{Macintosh}, B. and {Barman}, T. and {Bauman}, B. and {Burrows}, A. and 
	{Chilcote}, J.~K. and {De Rosa}, R.~J. and {Dillon}, D. and 
	{Doyon}, R. and {Dunn}, J. and {Erikson}, D. and {Fitzgerald}, M.~P. and 
	{Gavel}, D. and {Goodsell}, S.~J. and {Graham}, J.~R. and {Hartung}, M. and 
	{Hibon}, P. and {Kalas}, P.~G. and {Konopacky}, Q. and {Larkin}, J.~A. and 
	{Maire}, J. and {Marchis}, F. and {McBride}, J. and {Millar-Blanchaer}, M. and 
	{Morzinski}, K.~M. and {Norton}, A. and {Oppenheimer}, R. and 
	{Palmer}, D.~W. and {Patience}, J. and {Perrin}, M.~D. and {Poyneer}, L.~A. and 
	{Pueyo}, L. and {Rantakyr{\"o}}, F. and {Sadakuni}, N. and {Saddlemyer}, L. and 
	{Savransky}, D. and {Soummer}, R. and {Sivaramakrishnan}, A. and 
	{Song}, I. and {Thomas}, S. and {Wallace}, J.~K. and {Wiktorowicz}, S.~J. and 
	{Wolff}, S.~G.},
    title = "{Gemini Planet Imager Spectroscopy of the HR 8799 Planets c and d}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1409.5456},
 primaryClass = "astro-ph.EP",
 keywords = {infrared: planetary systems, instrumentation: adaptive optics, instrumentation: high angular resolution, planets and satellites: atmospheres, planets and satellites: gaseous planets, techniques: imaging spectroscopy },
     year = 2014,
    month = oct,
   volume = 794,
      eid = {L15},
    pages = {L15},
      doi = {10.1088/2041-8205/794/1/L15},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...794L..15I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wag16,
   author = {{Wagner}, K. and {Apai}, D. and {Kasper}, M. and {Kratter}, K. and 
	{McClure}, M. and {Robberto}, M. and {Beuzit}, J.-L.},
    title = "{Direct imaging discovery of a Jovian exoplanet within a triple-star system}",
  journal = \sci,
archivePrefix = "arXiv",
   eprint = {1607.02525},
 primaryClass = "astro-ph.EP",
     year = 2016,
    month = aug,
   volume = 353,
    pages = {673-678},
      doi = {10.1126/science.aaf9671},
   adsurl = {http://adsabs.harvard.edu/abs/2016Sci...353..673W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mac15,
   author = {{Macintosh}, B. and {Graham}, J.~R. and {Barman}, T. and {De Rosa}, R.~J. and 
	{Konopacky}, Q. and {Marley}, M.~S. and {Marois}, C. and {Nielsen}, E.~L. and 
	{Pueyo}, L. and {Rajan}, A. and {Rameau}, J. and {Saumon}, D. and 
	{Wang}, J.~J. and {Patience}, J. and {Ammons}, M. and {Arriaga}, P. and 
	{Artigau}, E. and {Beckwith}, S. and {Brewster}, J. and {Bruzzone}, S. and 
	{Bulger}, J. and {Burningham}, B. and {Burrows}, A.~S. and {Chen}, C. and 
	{Chiang}, E. and {Chilcote}, J.~K. and {Dawson}, R.~I. and {Dong}, R. and 
	{Doyon}, R. and {Draper}, Z.~H. and {Duch{\^e}ne}, G. and {Esposito}, T.~M. and 
	{Fabrycky}, D. and {Fitzgerald}, M.~P. and {Follette}, K.~B. and 
	{Fortney}, J.~J. and {Gerard}, B. and {Goodsell}, S. and {Greenbaum}, A.~Z. and 
	{Hibon}, P. and {Hinkley}, S. and {Cotten}, T.~H. and {Hung}, L.-W. and 
	{Ingraham}, P. and {Johnson-Groh}, M. and {Kalas}, P. and {Lafreniere}, D. and 
	{Larkin}, J.~E. and {Lee}, J. and {Line}, M. and {Long}, D. and 
	{Maire}, J. and {Marchis}, F. and {Matthews}, B.~C. and {Max}, C.~E. and 
	{Metchev}, S. and {Millar-Blanchaer}, M.~A. and {Mittal}, T. and 
	{Morley}, C.~V. and {Morzinski}, K.~M. and {Murray-Clay}, R. and 
	{Oppenheimer}, R. and {Palmer}, D.~W. and {Patel}, R. and {Perrin}, M.~D. and 
	{Poyneer}, L.~A. and {Rafikov}, R.~R. and {Rantakyr{\"o}}, F.~T. and 
	{Rice}, E.~L. and {Rojo}, P. and {Rudy}, A.~R. and {Ruffio}, J.-B. and 
	{Ruiz}, M.~T. and {Sadakuni}, N. and {Saddlemyer}, L. and {Salama}, M. and 
	{Savransky}, D. and {Schneider}, A.~C. and {Sivaramakrishnan}, A. and 
	{Song}, I. and {Soummer}, R. and {Thomas}, S. and {Vasisht}, G. and 
	{Wallace}, J.~K. and {Ward-Duong}, K. and {Wiktorowicz}, S.~J. and 
	{Wolff}, S.~G. and {Zuckerman}, B.},
    title = "{Discovery and spectroscopy of the young jovian planet 51 Eri b with the Gemini Planet Imager}",
  journal = \sci,
archivePrefix = "arXiv",
   eprint = {1508.03084},
 primaryClass = "astro-ph.EP",
     year = 2015,
    month = oct,
   volume = 350,
    pages = {64-67},
      doi = {10.1126/science.aac5891},
   adsurl = {http://adsabs.harvard.edu/abs/2015Sci...350...64M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tre16,
   author = {{Tremblin}, P. and {Amundsen}, D.~S. and {Chabrier}, G. and 
	{Baraffe}, I. and {Drummond}, B. and {Hinkley}, S. and {Mourier}, P. and 
	{Venot}, O.},
    title = "{Cloudless Atmospheres for L/T Dwarfs and Extrasolar Giant Planets}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1601.03652},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, methods: numerical, methods: observational, planets and satellites: atmospheres},
     year = 2016,
    month = feb,
   volume = 817,
      eid = {L19},
    pages = {L19},
      doi = {10.3847/2041-8205/817/2/L19},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...817L..19T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tre15,
   author = {{Tremblin}, P. and {Amundsen}, D.~S. and {Mourier}, P. and {Baraffe}, I. and 
	{Chabrier}, G. and {Drummond}, B. and {Homeier}, D. and {Venot}, O.
	},
    title = "{Fingering Convection and Cloudless Models for Cool Brown Dwarf Atmospheres}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1504.03334},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, methods: numerical, methods: observational},
     year = 2015,
    month = may,
   volume = 804,
      eid = {L17},
    pages = {L17},
      doi = {10.1088/2041-8205/804/1/L17},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...804L..17T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bar11,
   author = {{Barman}, T.~S. and {Macintosh}, B. and {Konopacky}, Q.~M. and 
	{Marois}, C.},
    title = "{Clouds and Chemistry in the Atmosphere of Extrasolar Planet HR8799b}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1103.3895},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, planetary systems, stars: atmospheres, stars: low-mass},
     year = 2011,
    month = may,
   volume = 733,
      eid = {65},
    pages = {65},
      doi = {10.1088/0004-637X/733/1/65},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...733...65B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kir12,
   author = {{Kirkpatrick}, J.~D. and {Gelino}, C.~R. and {Cushing}, M.~C. and 
	{Mace}, G.~N. and {Griffith}, R.~L. and {Skrutskie}, M.~F. and 
	{Marsh}, K.~A. and {Wright}, E.~L. and {Eisenhardt}, P.~R. and 
	{McLean}, I.~S. and {Mainzer}, A.~K. and {Burgasser}, A.~J. and 
	{Tinney}, C.~G. and {Parker}, S. and {Salter}, G.},
    title = "{Further Defining Spectral Type ''Y'' and Exploring the Low-mass End of the Field Brown Dwarf Mass Function}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1205.2122},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, solar neighborhood, stars: low-mass, stars: luminosity function, mass function, surveys, techniques: spectroscopic},
     year = 2012,
    month = jul,
   volume = 753,
      eid = {156},
    pages = {156},
      doi = {10.1088/0004-637X/753/2/156},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...753..156K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kir05,
   author = {{Kirkpatrick}, J.~D.},
    title = "{New Spectral Types L and T}",
  journal = \araa,
     year = 2005,
    month = sep,
   volume = 43,
    pages = {195-245},
      doi = {10.1146/annurev.astro.42.053102.134017},
   adsurl = {http://adsabs.harvard.edu/abs/2005ARA%26A..43..195K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cus11,
   author = {{Cushing}, M.~C. and {Kirkpatrick}, J.~D. and {Gelino}, C.~R. and 
	{Griffith}, R.~L. and {Skrutskie}, M.~F. and {Mainzer}, A. and 
	{Marsh}, K.~A. and {Beichman}, C.~A. and {Burgasser}, A.~J. and 
	{Prato}, L.~A. and {Simcoe}, R.~A. and {Marley}, M.~S. and {Saumon}, D. and 
	{Freedman}, R.~S. and {Eisenhardt}, P.~R. and {Wright}, E.~L.
	},
    title = "{The Discovery of Y Dwarfs using Data from the Wide-field Infrared Survey Explorer (WISE)}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1108.4678},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, infrared: stars, stars: individual: UGPS J072227.51{\ndash}054031.2 WISEPC J014807.25{\ndash}720258.8 WISEP J041022.71+150248.5 WISEPC J140518.40+553421.5 WISEP J154151.65-225025.2 WISEP J173835.52+273258.9 WISEP J182831.08+265037.8 WISEPC J205628.90+145953.3, stars: low-mass},
     year = 2011,
    month = dec,
   volume = 743,
      eid = {50},
    pages = {50},
      doi = {10.1088/0004-637X/743/1/50},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743...50C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bai99,
   author = {{Bailer-Jones}, C.~A.~L. and {Mundt}, R.},
    title = "{A search for variability in brown dwarfs and L dwarfs}",
  journal = \aap,
   eprint = {astro-ph/9906439},
 keywords = {METHODS: OBSERVATIONAL, STARS: ACTIVITY, STARS: INDIVIDUAL: 2MASSW J1145572+231730, STARS: LOW-MASS, BROWN DWARFS, STARS: ROTATION},
     year = 1999,
    month = aug,
   volume = 348,
    pages = {800-804},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...348..800B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bai01,
   author = {{Bailer-Jones}, C.~A.~L. and {Mundt}, R.},
    title = "{Variability in ultra cool dwarfs: Evidence for the evolution of surface features}",
  journal = \aap,
   eprint = {astro-ph/0012224},
 keywords = {METHODS: DATA ANALYSIS, STARS: ATMOSPHERES, STARS: LOW-MASS, BROWN DWARFS, STARS: ROTATION, STARS: STARSPOTS, STARS: VARIABLES: OTHERS},
     year = 2001,
    month = feb,
   volume = 367,
    pages = {218-235},
      doi = {10.1051/0004-6361:20000416},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...367..218B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gol08,
   author = {{Goldman}, B. and {Cushing}, M.~C. and {Marley}, M.~S. and {Artigau}, {\'E}. and 
	{Baliyan}, K.~S. and {B{\'e}jar}, V.~J.~S. and {Caballero}, J.~A. and 
	{Chanover}, N. and {Connelley}, M. and {Doyon}, R. and {Forveille}, T. and 
	{Ganesh}, S. and {Gelino}, C.~R. and {Hammel}, H.~B. and {Holtzman}, J. and 
	{Joshi}, S. and {Joshi}, U.~C. and {Leggett}, S.~K. and {Liu}, M.~C. and 
	{Mart{\'{\i}}n}, E.~L. and {Mohan}, V. and {Nadeau}, D. and 
	{Sagar}, R. and {Stephens}, D.},
    title = "{CLOUDS search for variability in brown dwarf atmospheres. Infrared spectroscopic time series of L/T transition brown dwarfs}",
  journal = \aap,
archivePrefix = "arXiv",
   eprint = {0801.2371},
 keywords = {stars: low-mass, brown dwarfs, stars: atmospheres, techniques: spectroscopic, stars: general},
     year = 2008,
    month = aug,
   volume = 487,
    pages = {277-292},
      doi = {10.1051/0004-6361:20065075},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...487..277G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Giz13,
   author = {{Gizis}, J.~E. and {Burgasser}, A.~J. and {Berger}, E. and {Williams}, P.~K.~G. and 
	{Vrba}, F.~J. and {Cruz}, K.~L. and {Metchev}, S.},
    title = "{Kepler Monitoring of an L Dwarf I. The Photometric Period and White Light Flares}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1310.5940},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: activity, stars: flare, stars: individual: WISEP J190648.47+401106.8, starspots},
     year = 2013,
    month = dec,
   volume = 779,
      eid = {172},
    pages = {172},
      doi = {10.1088/0004-637X/779/2/172},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...779..172G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Giz15,
   author = {{Gizis}, J.~E. and {Dettman}, K.~G. and {Burgasser}, A.~J. and 
	{Camnasio}, S. and {Alam}, M. and {Filippazzo}, J.~C. and {Cruz}, K.~L. and 
	{Metchev}, S. and {Berger}, E. and {Williams}, P.~K.~G.},
    title = "{Kepler Monitoring of an L Dwarf. II. Clouds with Multi-year Lifetimes}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1509.07186},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: activity, stars: atmospheres, stars: individual: WISEP J190648.47+401106.8, starspots},
     year = 2015,
    month = nov,
   volume = 813,
      eid = {104},
    pages = {104},
      doi = {10.1088/0004-637X/813/2/104},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...813..104G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Liu13,
   author = {{Liu}, M.~C. and {Magnier}, E.~A. and {Deacon}, N.~R. and {Allers}, K.~N. and 
	{Dupuy}, T.~J. and {Kotson}, M.~C. and {Aller}, K.~M. and {Burgett}, W.~S. and 
	{Chambers}, K.~C. and {Draper}, P.~W. and {Hodapp}, K.~W. and 
	{Jedicke}, R. and {Kaiser}, N. and {Kudritzki}, R.-P. and {Metcalfe}, N. and 
	{Morgan}, J.~S. and {Price}, P.~A. and {Tonry}, J.~L. and {Wainscoat}, R.~J.
	},
    title = "{The Extremely Red, Young L Dwarf PSO J318.5338-22.8603: A Free-floating Planetary-mass Analog to Directly Imaged Young Gas-giant Planets}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1310.0457},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, parallaxes, planets and satellites: atmospheres, proper motions, solar neighborhood, surveys},
     year = 2013,
    month = nov,
   volume = 777,
      eid = {L20},
    pages = {L20},
      doi = {10.1088/2041-8205/777/2/L20},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...777L..20L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cha04,
   author = {{Chauvin}, G. and {Lagrange}, A.-M. and {Dumas}, C. and {Zuckerman}, B. and 
	{Mouillet}, D. and {Song}, I. and {Beuzit}, J.-L. and {Lowrance}, P.
	},
    title = "{A giant planet candidate near a young brown dwarf. Direct VLT/NACO observations using IR wavefront sensing}",
  journal = \aap,
   eprint = {astro-ph/0409323},
 keywords = {2MASSWJ 1207334-393254, brown dwarf, giant planet, adaptive optics imaging and spectroscopy},
     year = 2004,
    month = oct,
   volume = 425,
    pages = {L29-L32},
      doi = {10.1051/0004-6361:200400056},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...425L..29C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cha05,
   author = {{Chauvin}, G. and {Lagrange}, A.-M. and {Dumas}, C. and {Zuckerman}, B. and 
	{Mouillet}, D. and {Song}, I. and {Beuzit}, J.-L. and {Lowrance}, P.
	},
    title = "{Giant planet companion to 2MASSW J1207334-393254}",
  journal = \aap,
   eprint = {astro-ph/0504659},
     year = 2005,
    month = aug,
   volume = 438,
    pages = {L25-L28},
      doi = {10.1051/0004-6361:200500116},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...438L..25C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Apa16,
   author = {{Apai}, D. and {Kasper}, M. and {Skemer}, A. and {Hanson}, J.~R. and 
	{Lagrange}, A.-M. and {Biller}, B.~A. and {Bonnefoy}, M. and 
	{Buenzli}, E. and {Vigan}, A.},
    title = "{High-cadence, High-contrast Imaging for Exoplanet Mapping: Observations of the HR 8799 Planets with VLT/SPHERE Satellite-spot-corrected Relative Photometry}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1602.02856},
 primaryClass = "astro-ph.EP",
 keywords = {methods: observational, planetary systems, planets and satellites: atmospheres, planets and satellites: gaseous planets, planets and satellites: individual: HR 8799, techniques: photometric},
     year = 2016,
    month = mar,
   volume = 820,
      eid = {40},
    pages = {40},
      doi = {10.3847/0004-637X/820/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...820...40A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kar16,
   author = {{Karalidi}, T. and {Apai}, D. and {Marley}, M.~S. and {Buenzli}, E.
	},
    title = "{Maps of Evolving Cloud Structures in Luhman 16AB from HST Time-resolved Spectroscopy}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1605.01682},
 primaryClass = "astro-ph.EP",
 keywords = {methods: statistical, stars: individual: WISE J104915.57-531906.1, techniques: photometric},
     year = 2016,
    month = jul,
   volume = 825,
      eid = {90},
    pages = {90},
      doi = {10.3847/0004-637X/825/2/90},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...825...90K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kar15,
   author = {{Karalidi}, T. and {Apai}, D. and {Schneider}, G. and {Hanson}, J.~R. and 
	{Pasachoff}, J.~M.},
    title = "{Aeolus: A Markov Chain Monte Carlo Code for Mapping Ultracool Atmospheres. An Application on Jupiter and Brown Dwarf HST Light Curves}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1510.04251},
 primaryClass = "astro-ph.EP",
 keywords = {methods: statistical, planets and satellites: individual: Jupiter, stars: individual: 2MASS J21392676+0220226, 2MASS J0136565+093347, techniques: photometric},
     year = 2015,
    month = nov,
   volume = 814,
      eid = {65},
    pages = {65},
      doi = {10.1088/0004-637X/814/1/65},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...814...65K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Apa13,
   author = {{Apai}, D. and {Radigan}, J. and {Buenzli}, E. and {Burrows}, A. and 
	{Reid}, I.~N. and {Jayawardhana}, R.},
    title = "{HST Spectral Mapping of L/T Transition Brown Dwarfs Reveals Cloud Thickness Variations}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1303.4151},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, planetary systems, planets and satellites: individual: Jupiter, stars: atmospheres, stars: low-mass, starspots },
     year = 2013,
    month = may,
   volume = 768,
      eid = {121},
    pages = {121},
      doi = {10.1088/0004-637X/768/2/121},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...768..121A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kos13,
   author = {{Kostov}, V. and {Apai}, D.},
    title = "{Mapping Directly Imaged Giant Exoplanets}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1210.6915},
 primaryClass = "astro-ph.EP",
 keywords = {methods: analytical, planetary systems, planets and satellites: atmospheres, planets and satellites: composition, techniques: photometric, techniques: spectroscopic },
     year = 2013,
    month = jan,
   volume = 762,
      eid = {47},
    pages = {47},
      doi = {10.1088/0004-637X/762/1/47},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...762...47K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cro14b,
   author = {{Crossfield}, I.~J.~M.},
    title = "{Doppler imaging of exoplanets and brown dwarfs}",
  journal = \aap,
archivePrefix = "arXiv",
   eprint = {1404.7853},
 primaryClass = "astro-ph.SR",
 keywords = {instrumentation: spectrographs, techniques: spectroscopic, catalogs, planets and satellites: atmospheres, brown dwarfs, stars: imaging},
     year = 2014,
    month = jun,
   volume = 566,
      eid = {A130},
    pages = {A130},
      doi = {10.1051/0004-6361/201423750},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...566A.130C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vog87,
   author = {{Vogt}, S.~S. and {Penrod}, G.~D. and {Hatzes}, A.~P.},
    title = "{Doppler images of rotating stars using maximum entropy image reconstruction}",
  journal = \apj,
 keywords = {Doppler Effect, Image Reconstruction, Maximum Entropy Method, Peculiar Stars, Stellar Rotation, Stellar Spectra, Computational Grids, Iterative Solution, Line Spectra, Signal To Noise Ratios, Spatial Resolution, Spectral Resolution, Starspots},
     year = 1987,
    month = oct,
   volume = 321,
    pages = {496-515},
      doi = {10.1086/165647},
   adsurl = {http://adsabs.harvard.edu/abs/1987ApJ...321..496V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ric89,
   author = {{Rice}, J.~B. and {Wehlau}, W.~H. and {Khokhlova}, V.~L.},
    title = "{Mapping stellar surfaces by Doppler imaging - Technique and application}",
  journal = \aap,
 keywords = {A Stars, Doppler Effect, Mapping, Peculiar Stars, Image Reconstruction, Iron, Line Spectra, Red Shift, Spectral Line Width, Stellar Magnetic Fields, Stellar Rotation},
     year = 1989,
    month = jan,
   volume = 208,
    pages = {179-188},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...208..179R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Unr95,
   author = {{Unruh}, Y.~C. and {Collier Cameron}, A.},
    title = "{The sensitivity of Doppler imaging to line profile models}",
  journal = \mnras,
 keywords = {TECHNIQUES: IMAGE PROCESSING, STARS: ACTIVITY, STARS: IMAGING},
     year = 1995,
    month = mar,
   volume = 273,
    pages = {1-16},
      doi = {10.1093/mnras/273.1.1},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.273....1U},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yan16,
   author = {{Yang}, H. and {Apai}, D. and {Marley}, M.~S. and {Karalidi}, T. and 
	{Flateau}, D. and {Showman}, A.~P. and {Metchev}, S. and {Buenzli}, E. and 
	{Radigan}, J. and {Artigau}, {\'E}. and {Lowrance}, P.~J. and 
	{Burgasser}, A.~J.},
    title = "{Extrasolar Storms: Pressure-dependent Changes in Light-curve Phase in Brown Dwarfs from Simultaneous HST and Spitzer Observations}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1605.02708},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, infrared: stars, stars: atmospheres, stars: low-mass},
     year = 2016,
    month = jul,
   volume = 826,
      eid = {8},
    pages = {8},
      doi = {10.3847/0004-637X/826/1/8},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...826....8Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yan15,
   author = {{Yang}, H. and {Apai}, D. and {Marley}, M.~S. and {Saumon}, D. and 
	{Morley}, C.~V. and {Buenzli}, E. and {Artigau}, {\'E}. and 
	{Radigan}, J. and {Metchev}, S. and {Burgasser}, A.~J. and {Mohanty}, S. and 
	{Lowrance}, P.~J. and {Showman}, A.~P. and {Karalidi}, T. and 
	{Flateau}, D. and {Heinze}, A.~N.},
    title = "{HST Rotational Spectral Mapping of Two L-type Brown Dwarfs: Variability in and out of Water Bands indicates High-altitude Haze Layers}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1411.2911},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, stars: atmospheres, stars: individual: 2MASS J18212815+1414010 2MASS J15074769-1627386 2MASS J01365662+0933473, stars: low-mass},
     year = 2015,
    month = jan,
   volume = 798,
      eid = {L13},
    pages = {L13},
      doi = {10.1088/2041-8205/798/1/L13},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798L..13Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bur02,
   author = {{Burgasser}, A.~J. and {Marley}, M.~S. and {Ackerman}, A.~S. and 
	{Saumon}, D. and {Lodders}, K. and {Dahn}, C.~C. and {Harris}, H.~C. and 
	{Kirkpatrick}, J.~D.},
    title = "{Evidence of Cloud Disruption in the L/T Dwarf Transition}",
  journal = \apjl,
   eprint = {astro-ph/0205051},
 keywords = {Infrared: Stars, Stars: Atmospheres, Stars: Fundamental Parameters, Stars: Individual: Alphanumeric: SDSS J1254-0122, Stars: Individual: Alphanumeric: 2MASS J0559-1404, Stars: Low-Mass, Brown Dwarfs},
     year = 2002,
    month = jun,
   volume = 571,
    pages = {L151-L154},
      doi = {10.1086/341343},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...571L.151B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bur03,
   author = {{Burgasser}, A.~J. and {Kirkpatrick}, J.~D. and {Liebert}, J. and 
	{Burrows}, A.},
    title = "{The Spectra of T Dwarfs. II. Red Optical Data}",
  journal = \apj,
   eprint = {astro-ph/0305139},
 keywords = {Stars: Activity, Stars: Fundamental Parameters, Stars: Individual: Alphanumeric: 2MASS J09373487+2931409, Stars: Low-Mass, Brown Dwarfs},
     year = 2003,
    month = sep,
   volume = 594,
    pages = {510-524},
      doi = {10.1086/376756},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...594..510B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cus08,
   author = {{Cushing}, M.~C. and {Marley}, M.~S. and {Saumon}, D. and {Kelly}, B.~C. and 
	{Vacca}, W.~D. and {Rayner}, J.~T. and {Freedman}, R.~S. and 
	{Lodders}, K. and {Roellig}, T.~L.},
    title = "{Atmospheric Parameters of Field L and T Dwarfs}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {0711.0801},
 keywords = {infrared: stars, radiative transfer, stars: fundamental parameters, stars: low-mass, brown dwarfs},
     year = 2008,
    month = may,
   volume = 678,
      eid = {1372-1395},
    pages = {1372-1395},
      doi = {10.1086/526489},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...678.1372C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Esp16,
   author = {{Esplin}, T. and {Luhman}, K. and {Cushing}, M. and {Hardegree-Ullman}, K. and 
	{Trucks}, J. and {Burgasser}, A. and {Schneider}, A.},
    title = "{Photometric Monitoring of the Coldest Known Brown Dwarf with the Spitzer Space Telescope}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1609.05850},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
     year = 2016,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160905850E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leg16,
   author = {{Leggett}, S.~K. and {Cushing}, M.~C. and {Hardegree-Ullman}, K.~K. and 
	{Trucks}, J.~L. and {Marley}, M.~S. and {Morley}, C.~V. and 
	{Saumon}, D. and {Carey}, S.~J. and {Fortney}, J.~J. and {Gelino}, C.~R. and 
	{Gizis}, J.~E. and {Kirkpatrick}, J.~D. and {Mace}, G.~N.},
    title = "{Observed Variability at 1um and 4um in the Y0 Brown Dwarf WISEP J173835.52+273258.9}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1607.07888},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics},
     year = 2016,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160707888L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Luh14,
   author = {{Luhman}, K.~L.},
    title = "{Discovery of a \~{}250 K Brown Dwarf at 2 pc from the Sun}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1404.6501},
 keywords = {brown dwarfs, infrared: stars, proper motions, solar neighborhood, stars: low-mass},
     year = 2014,
    month = may,
   volume = 786,
      eid = {L18},
    pages = {L18},
      doi = {10.1088/2041-8205/786/2/L18},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...786L..18L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bar03,
   author = {{Baraffe}, I. and {Chabrier}, G. and {Barman}, T.~S. and {Allard}, F. and 
	{Hauschildt}, P.~H.},
    title = "{Evolutionary models for cool brown dwarfs and extrasolar giant planets. The case of HD 209458}",
  journal = \aap,
   eprint = {astro-ph/0302293},
 keywords = {planetary systems, stars: brown dwarfs, stars: evolution, stars: individual (HD 209458)},
     year = 2003,
    month = may,
   volume = 402,
    pages = {701-712},
      doi = {10.1051/0004-6361:20030252},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...402..701B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mor14b,
   author = {{Morley}, C.~V. and {Marley}, M.~S. and {Fortney}, J.~J. and 
	{Lupu}, R.},
    title = "{Spectral Variability from the Patchy Atmospheres of T and Y Dwarfs}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1406.0863},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, planets and satellites: atmospheres, stars: atmospheres},
     year = 2014,
    month = jul,
   volume = 789,
      eid = {L14},
    pages = {L14},
      doi = {10.1088/2041-8205/789/1/L14},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...789L..14M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mor14a,
   author = {{Morley}, C.~V. and {Marley}, M.~S. and {Fortney}, J.~J. and 
	{Lupu}, R. and {Saumon}, D. and {Greene}, T. and {Lodders}, K.
	},
    title = "{Water Clouds in Y Dwarfs and Exoplanets}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1404.0005},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, planets and satellites: atmospheres, planets and satellites: detection, stars: atmospheres},
     year = 2014,
    month = may,
   volume = 787,
      eid = {78},
    pages = {78},
      doi = {10.1088/0004-637X/787/1/78},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...787...78M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hal15,
   author = {{Hallinan}, G. and {Littlefair}, S.~P. and {Cotter}, G. and 
	{Bourke}, S. and {Harding}, L.~K. and {Pineda}, J.~S. and {Butler}, R.~P. and 
	{Golden}, A. and {Basri}, G. and {Doyle}, J.~G. and {Kao}, M.~M. and 
	{Berdyugina}, S.~V. and {Kuznetsov}, A. and {Rupen}, M.~P. and 
	{Antonova}, A.},
    title = "{Magnetospherically driven optical and radio aurorae at the end of the stellar main sequence}",
  journal = \nat,
archivePrefix = "arXiv",
   eprint = {1507.08739},
 primaryClass = "astro-ph.SR",
     year = 2015,
    month = jul,
   volume = 523,
    pages = {568-571},
      doi = {10.1038/nature14619},
   adsurl = {http://adsabs.harvard.edu/abs/2015Natur.523..568H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Giz15,
   author = {{Gizis}, J.~E. and {Allers}, K.~N. and {Liu}, M.~C. and {Harris}, H.~C. and 
	{Faherty}, J.~K. and {Burgasser}, A.~J. and {Kirkpatrick}, J.~D.
	},
    title = "{WISEP J004701.06+680352.1: An Intermediate Surface Gravity, Dusty Brown Dwarf in the AB Dor Moving Group}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1412.1856},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, infrared: stars, stars: individual: WISEP J004701.06+680352.1 2MASS J21481628+4003593},
     year = 2015,
    month = feb,
   volume = 799,
      eid = {203},
    pages = {203},
      doi = {10.1088/0004-637X/799/2/203},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...799..203G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Giz12,
   author = {{Gizis}, J.~E. and {Faherty}, J.~K. and {Liu}, M.~C. and {Castro}, P.~J. and 
	{Shaw}, J.~D. and {Vrba}, F.~J. and {Harris}, H.~C. and {Aller}, K.~M. and 
	{Deacon}, N.~R.},
    title = "{Discovery of an Unusually Red L-type Brown Dwarf}",
  journal = \aj,
archivePrefix = "arXiv",
   eprint = {1207.4012},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, infrared: stars, proper motions, stars: individual: WISEP J004701.06+680352.1},
     year = 2012,
    month = oct,
   volume = 144,
      eid = {94},
    pages = {94},
      doi = {10.1088/0004-6256/144/4/94},
   adsurl = {http://adsabs.harvard.edu/abs/2012AJ....144...94G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Zha14,
   author = {{Zhang}, X. and {Showman}, A.~P.},
    title = "{Atmospheric Circulation of Brown Dwarfs: Jets, Vortices, and Time Variability}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1403.2143},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, methods: numerical, stars: atmospheres, stars: low-mass},
     year = 2014,
    month = jun,
   volume = 788,
      eid = {L6},
    pages = {L6},
      doi = {10.1088/2041-8205/788/1/L6},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...788L...6Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Sho13,
   author = {{Showman}, A.~P. and {Kaspi}, Y.},
    title = "{Atmospheric Dynamics of Brown Dwarfs and Directly Imaged Giant Planets}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1210.7573},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, convection, methods: numerical, stars: low-mass, turbulence, waves},
     year = 2013,
    month = oct,
   volume = 776,
      eid = {85},
    pages = {85},
      doi = {10.1088/0004-637X/776/2/85},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...776...85S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rob14,
   author = {{Robinson}, T.~D. and {Marley}, M.~S.},
    title = "{Temperature Fluctuations as a Source of Brown Dwarf Variability}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1403.2438},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, convection, radiation mechanisms: thermal, stars: atmospheres},
     year = 2014,
    month = apr,
   volume = 785,
      eid = {158},
    pages = {158},
      doi = {10.1088/0004-637X/785/2/158},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...785..158R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sta15,
   author = {{Stark}, C.~R. and {Helling}, C. and {Diver}, D.~A.},
    title = "{Inhomogeneous cloud coverage through the Coulomb explosion of dust in substellar atmospheres}",
  journal = \aap,
archivePrefix = "arXiv",
   eprint = {1505.04592},
 primaryClass = "astro-ph.SR",
 keywords = {stars: atmospheres, brown dwarfs, stars: low-mass, plasmas},
     year = 2015,
    month = jul,
   volume = 579,
      eid = {A41},
    pages = {A41},
      doi = {10.1051/0004-6361/201526045},
   adsurl = {http://adsabs.harvard.edu/abs/2015A\%26A...579A..41S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fre10,
   author = {{Freytag}, B. and {Allard}, F. and {Ludwig}, H.-G. and {Homeier}, D. and 
	{Steffen}, M.},
    title = "{The role of convection, overshoot, and gravity waves for the transport of dust in M dwarf and brown dwarf atmospheres}",
  journal = \aap,
archivePrefix = "arXiv",
   eprint = {1002.3437},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, hydrodynamics, convection, waves, stars: atmospheres, stars: low-mass},
     year = 2010,
    month = apr,
   volume = 513,
      eid = {A19},
    pages = {A19},
      doi = {10.1051/0004-6361/200913354},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...513A..19F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mar12,
   author = {{Marley}, M.~S. and {Saumon}, D. and {Cushing}, M. and {Ackerman}, A.~S. and 
	{Fortney}, J.~J. and {Freedman}, R.},
    title = "{Masses, Radii, and Cloud Properties of the HR 8799 Planets}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1205.6488},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, planetary systems, stars: atmospheres, stars: individual: HR 8799, stars: low-mass},
     year = 2012,
    month = aug,
   volume = 754,
      eid = {135},
    pages = {135},
      doi = {10.1088/0004-637X/754/2/135},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754..135M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mor12,
   author = {{Morley}, C.~V. and {Fortney}, J.~J. and {Marley}, M.~S. and 
	{Visscher}, C. and {Saumon}, D. and {Leggett}, S.~K.},
    title = "{Neglected Clouds in T and Y Dwarf Atmospheres}",
  journal = \apj,
archivePrefix = "arXiv",
   eprint = {1206.4313},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: atmospheres},
     year = 2012,
    month = sep,
   volume = 756,
      eid = {172},
    pages = {172},
      doi = {10.1088/0004-637X/756/2/172},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...756..172M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mar15,
   author = {{Marley}, M.~S. and {Robinson}, T.~D.},
    title = "{On the Cool Side: Modeling the Atmospheres of Brown Dwarfs and Giant Planets}",
  journal = \araa,
archivePrefix = "arXiv",
   eprint = {1410.6512},
 primaryClass = "astro-ph.EP",
     year = 2015,
    month = aug,
   volume = 53,
    pages = {279-323},
      doi = {10.1146/annurev-astro-082214-122522},
   adsurl = {http://adsabs.harvard.edu/abs/2015ARA%26A..53..279M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{May14,
   author = {{Mayne}, N.~J. and {Baraffe}, I. and {Acreman}, D.~M. and {Smith}, C. and 
	{Browning}, M.~K. and {Sk{\aa}lid Amundsen}, D. and {Wood}, N. and 
	{Thuburn}, J. and {Jackson}, D.~R.},
    title = "{The unified model, a fully-compressible, non-hydrostatic, deep atmosphere global circulation model, applied to hot Jupiters. ENDGame for a HD 209458b test case}",
  journal = \aap,
 keywords = {methods: numerical, hydrodynamics, planets and satellites: atmospheres},
     year = 2014,
    month = jan,
   volume = 561,
      eid = {A1},
    pages = {A1},
      doi = {10.1051/0004-6361/201322174},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...561A...1M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bai04,
   author = {{Bailer-Jones}, C.~A.~L.},
    title = "{Spectroscopic rotation velocities of L dwarfs from VLT/UVES and their comparison with periods from photometric monitoring}",
  journal = \aap,
   eprint = {astro-ph/0403013},
 keywords = {techniques: spectroscopic, stars: low-mass, brown dwarfs, stars: variables: general, stars: rotation},
     year = 2004,
    month = may,
   volume = 419,
    pages = {703-712},
      doi = {10.1051/0004-6361:20040965},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...419..703B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bai03,
   author = {{Bailer-Jones}, C.~A.~L. and {Lamm}, M.},
    title = "{Limits on the infrared photometric monitoring of brown dwarfs}",
  journal = \mnras,
   eprint = {astro-ph/0210413},
 keywords = {methods: data analysis, techniques: photometric, stars: individual: 2MASSW J1439284+192915, stars: individual: SDSSp J12035819+001550.33, stars: individual: 2MASSW J1112257+354813, stars: low-mass, brown dwarfs},
     year = 2003,
    month = feb,
   volume = 339,
    pages = {477-485},
      doi = {10.1046/j.1365-8711.2003.06189.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.339..477B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lew16,
   author = {{Lew}, B.~W.~P. and {Apai}, D. and {Zhou}, Y. and {Schneider}, G. and 
	{Burgasser}, A.~J. and {Karalidi}, T. and {Yang}, H. and {Marley}, M.~S. and 
	{Cowan}, N.~B. and {Bedin}, L.~R. and {Metchev}, S.~A. and {Radigan}, J. and 
	{Lowrance}, P.~J.},
    title = "{Cloud Atlas: Discovery of Patchy Clouds and High-amplitude Rotational Modulations in a Young, Extremely Red L-type Brown Dwarf}",
  journal = \apjl,
archivePrefix = "arXiv",
   eprint = {1609.04804},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: atmospheres, stars: individual: WISEP J004701.06+680352.1, stars: low-mass },
     year = 2016,
    month = oct,
   volume = 829,
      eid = {L32},
    pages = {L32},
      doi = {10.3847/2041-8205/829/2/L32},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...829L..32L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mar08,
   author = {{Marois}, C. and {Macintosh}, B. and {Barman}, T. and {Zuckerman}, B. and 
	{Song}, I. and {Patience}, J. and {Lafreni{\`e}re}, D. and {Doyon}, R.
	},
    title = "{Direct Imaging of Multiple Planets Orbiting the Star HR 8799}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {0811.2606},
     year = 2008,
    month = nov,
   volume = 322,
    pages = {1348},
      doi = {10.1126/science.1166585},
   adsurl = {http://adsabs.harvard.edu/abs/2008Sci...322.1348M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maro10,
   author = {{Marois}, C. and {Zuckerman}, B. and {Konopacky}, Q.~M. and 
	{Macintosh}, B. and {Barman}, T.},
    title = "{Images of a fourth planet orbiting HR 8799}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1011.4918},
 primaryClass = "astro-ph.EP",
     year = 2010,
    month = dec,
   volume = 468,
    pages = {1080-1083},
      doi = {10.1038/nature09684},
   adsurl = {http://adsabs.harvard.edu/abs/2010Natur.468.1080M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jen15,
   author = {{Jenkins}, J.~M. and {Twicken}, J.~D. and {Batalha}, N.~M. and 
	{Caldwell}, D.~A. and {Cochran}, W.~D. and {Endl}, M. and {Latham}, D.~W. and 
	{Esquerdo}, G.~A. and {Seader}, S. and {Bieryla}, A. and {Petigura}, E. and 
	{Ciardi}, D.~R. and {Marcy}, G.~W. and {Isaacson}, H. and {Huber}, D. and 
	{Rowe}, J.~F. and {Torres}, G. and {Bryson}, S.~T. and {Buchhave}, L. and 
	{Ramirez}, I. and {Wolfgang}, A. and {Li}, J. and {Campbell}, J.~R. and 
	{Tenenbaum}, P. and {Sanderfer}, D. and {Henze}, C.~E. and {Catanzarite}, J.~H. and 
	{Gilliland}, R.~L. and {Borucki}, W.~J.},
    title = "{Discovery and Validation of Kepler-452b: A 1.6 R$_{⨁}$ Super Earth Exoplanet in the Habitable Zone of a G2 Star}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1507.06723},
 primaryClass = "astro-ph.EP",
 keywords = {methods: statistical, planets and satellites: detection, stars: fundamental parameters, stars: individual: Kepler-452b, KIC 8311864, KOI7016.01},
     year = 2015,
    month = aug,
   volume = 150,
      eid = {56},
    pages = {56},
      doi = {10.1088/0004-6256/150/2/56},
   adsurl = {http://adsabs.harvard.edu/abs/2015AJ....150...56J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ang16,
   author = {{Anglada-Escud{\'e}}, G. and {Amado}, P.~J. and {Barnes}, J. and 
	{Berdi{\~n}as}, Z.~M. and {Butler}, R.~P. and {Coleman}, G.~A.~L. and 
	{de La Cueva}, I. and {Dreizler}, S. and {Endl}, M. and {Giesers}, B. and 
	{Jeffers}, S.~V. and {Jenkins}, J.~S. and {Jones}, H.~R.~A. and 
	{Kiraga}, M. and {K{\"u}rster}, M. and {L{\'o}pez-Gonz{\'a}lez}, M.~J. and 
	{Marvin}, C.~J. and {Morales}, N. and {Morin}, J. and {Nelson}, R.~P. and 
	{Ortiz}, J.~L. and {Ofir}, A. and {Paardekooper}, S.-J. and 
	{Reiners}, A. and {Rodr{\'{\i}}guez}, E. and {Rodr{\'{\i}}guez-L{\'o}pez}, C. and 
	{Sarmiento}, L.~F. and {Strachan}, J.~P. and {Tsapras}, Y. and 
	{Tuomi}, M. and {Zechmeister}, M.},
    title = "{A terrestrial planet candidate in a temperate orbit around Proxima Centauri}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1609.03449},
 primaryClass = "astro-ph.EP",
     year = 2016,
    month = aug,
   volume = 536,
    pages = {437-440},
      doi = {10.1038/nature19106},
   adsurl = {http://adsabs.harvard.edu/abs/2016Natur.536..437A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bil07,
   author = {{Biller}, B.~A. and {Close}, L.~M. and {Masciadri}, E. and {Nielsen}, E. and 
	{Lenzen}, R. and {Brandner}, W. and {McCarthy}, D. and {Hartung}, M. and 
	{Kellner}, S. and {Mamajek}, E. and {Henning}, T. and {Miller}, D. and 
	{Kenworthy}, M. and {Kulesa}, C.},
    title = "{An Imaging Survey for Extrasolar Planets around 45 Close, Young Stars with the Simultaneous Differential Imager at the Very Large Telescope and MMT}",
  journal = {\apjs},
 keywords = {Instrumentation: Adaptive Optics, Stars: Planetary Systems},
     year = 2007,
    month = nov,
   volume = 173,
    pages = {143-165},
      doi = {10.1086/519925},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..173..143B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tra07,
   author = {{Trauger}, J.~T. and {Traub}, W.~A.},
    title = "{A laboratory demonstration of the capability to image an Earth-like extrasolar planet}",
  journal = {\nat},
     year = 2007,
    month = apr,
   volume = 446,
    pages = {771-773},
      doi = {10.1038/nature05729},
   adsurl = {http://adsabs.harvard.edu/abs/2007Natur.446..771T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bil13b,
   author = {{Biller}, B.~A. and {Liu}, M.~C. and {Wahhaj}, Z. and {Nielsen}, E.~L. and 
	{Hayward}, T.~L. and {Males}, J.~R. and {Skemer}, A. and {Close}, L.~M. and 
	{Chun}, M. and {Ftaclas}, C. and {Clarke}, F. and {Thatte}, N. and 
	{Shkolnik}, E.~L. and {Reid}, I.~N. and {Hartung}, M. and {Boss}, A. and 
	{Lin}, D. and {Alencar}, S.~H.~P. and {de Gouveia Dal Pino}, E. and 
	{Gregorio-Hetem}, J. and {Toomey}, D.},
    title = "{The Gemini/NICI Planet-Finding Campaign: The Frequency of Planets around Young Moving Group Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1309.1462},
 primaryClass = "astro-ph.EP",
 keywords = {binaries: close, brown dwarfs, planetary systems, planets and satellites: detection, stars: late-type},
     year = 2013,
    month = nov,
   volume = 777,
      eid = {160},
    pages = {160},
      doi = {10.1088/0004-637X/777/2/160},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...777..160B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bra14,
   author = {{Brandt}, T.~D. and {McElwain}, M.~W. and {Turner}, E.~L. and 
	{Mede}, K. and {Spiegel}, D.~S. and {Kuzuhara}, M. and {Schlieder}, J.~E. and 
	{Wisniewski}, J.~P. and {Abe}, L. and {Biller}, B. and {Brandner}, W. and 
	{Carson}, J. and {Currie}, T. and {Egner}, S. and {Feldt}, M. and 
	{Golota}, T. and {Goto}, M. and {Grady}, C.~A. and {Guyon}, O. and 
	{Hashimoto}, J. and {Hayano}, Y. and {Hayashi}, M. and {Hayashi}, S. and 
	{Henning}, T. and {Hodapp}, K.~W. and {Inutsuka}, S. and {Ishii}, M. and 
	{Iye}, M. and {Janson}, M. and {Kandori}, R. and {Knapp}, G.~R. and 
	{Kudo}, T. and {Kusakabe}, N. and {Kwon}, J. and {Matsuo}, T. and 
	{Miyama}, S. and {Morino}, J.-I. and {Moro-Mart{\'{\i}}n}, A. and 
	{Nishimura}, T. and {Pyo}, T.-S. and {Serabyn}, E. and {Suto}, H. and 
	{Suzuki}, R. and {Takami}, M. and {Takato}, N. and {Terada}, H. and 
	{Thalmann}, C. and {Tomono}, D. and {Watanabe}, M. and {Yamada}, T. and 
	{Takami}, H. and {Usuda}, T. and {Tamura}, M.},
    title = "{A Statistical Analysis of SEEDS and Other High-contrast Exoplanet Surveys: Massive Planets or Low-mass Brown Dwarfs?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1404.5335},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, methods: statistical, open clusters and associations: general, planetary systems, stars: activity, stars: imaging},
     year = 2014,
    month = oct,
   volume = 794,
      eid = {159},
    pages = {159},
      doi = {10.1088/0004-637X/794/2/159},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...794..159B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nau14,
   author = {{Naud}, M.-E. and {Artigau}, {\'E}. and {Malo}, L. and {Albert}, L. and 
	{Doyon}, R. and {Lafreni{\`e}re}, D. and {Gagn{\'e}}, J. and 
	{Saumon}, D. and {Morley}, C.~V. and {Allard}, F. and {Homeier}, D. and 
	{Beichman}, C.~A. and {Gelino}, C.~R. and {Boucher}, A.},
    title = "{Discovery of a Wide Planetary-mass Companion to the Young M3 Star GU Psc}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1405.2932},
 primaryClass = "astro-ph.EP",
 keywords = {infrared: planetary systems, planetary systems, planets and satellites: detection, stars: imaging, stars: individual: GU Psc, stars: low-mass},
     year = 2014,
    month = may,
   volume = 787,
      eid = {5},
    pages = {5},
      doi = {10.1088/0004-637X/787/1/5},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...787....5N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ram13,
   author = {{Rameau}, J. and {Chauvin}, G. and {Lagrange}, A.-M. and {Boccaletti}, A. and 
	{Quanz}, S.~P. and {Bonnefoy}, M. and {Girard}, J.~H. and {Delorme}, P. and 
	{Desidera}, S. and {Klahr}, H. and {Mordasini}, C. and {Dumas}, C. and 
	{Bonavita}, M.},
    title = "{Discovery of a Probable 4-5 Jupiter-mass Exoplanet to HD 95086 by Direct Imaging}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1305.7428},
 primaryClass = "astro-ph.EP",
 keywords = {instrumentation: adaptive optics, planets and satellites: detection, stars: individual: HD 95086, stars: massive},
     year = 2013,
    month = aug,
   volume = 772,
      eid = {L15},
    pages = {L15},
      doi = {10.1088/2041-8205/772/2/L15},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...772L..15R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kuz13,
   author = {{Kuzuhara}, M. and {Tamura}, M. and {Kudo}, T. and {Janson}, M. and 
	{Kandori}, R. and {Brandt}, T.~D. and {Thalmann}, C. and {Spiegel}, D. and 
	{Biller}, B. and {Carson}, J. and {Hori}, Y. and {Suzuki}, R. and 
	{Burrows}, A. and {Henning}, T. and {Turner}, E.~L. and {McElwain}, M.~W. and 
	{Moro-Mart{\'{\i}}n}, A. and {Suenaga}, T. and {Takahashi}, Y.~H. and 
	{Kwon}, J. and {Lucas}, P. and {Abe}, L. and {Brandner}, W. and 
	{Egner}, S. and {Feldt}, M. and {Fujiwara}, H. and {Goto}, M. and 
	{Grady}, C.~A. and {Guyon}, O. and {Hashimoto}, J. and {Hayano}, Y. and 
	{Hayashi}, M. and {Hayashi}, S.~S. and {Hodapp}, K.~W. and {Ishii}, M. and 
	{Iye}, M. and {Knapp}, G.~R. and {Matsuo}, T. and {Mayama}, S. and 
	{Miyama}, S. and {Morino}, J.-I. and {Nishikawa}, J. and {Nishimura}, T. and 
	{Kotani}, T. and {Kusakabe}, N. and {Pyo}, T.-S. and {Serabyn}, E. and 
	{Suto}, H. and {Takami}, M. and {Takato}, N. and {Terada}, H. and 
	{Tomono}, D. and {Watanabe}, M. and {Wisniewski}, J.~P. and 
	{Yamada}, T. and {Takami}, H. and {Usuda}, T.},
    title = "{Direct Imaging of a Cold Jovian Exoplanet in Orbit around the Sun-like Star GJ 504}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1307.2886},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems, stars: formation, stars: individual: GJ 504},
     year = 2013,
    month = sep,
   volume = 774,
      eid = {11},
    pages = {11},
      doi = {10.1088/0004-637X/774/1/11},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...774...11K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sch12,
   author = {{Schlieder}, J.~E. and {L{\'e}pine}, S. and {Simon}, M.},
    title = "{Likely Members of the {$\beta$} Pictoris and AB Doradus Moving Groups in the North}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1208.0679},
 primaryClass = "astro-ph.SR",
 keywords = {open clusters and associations: individual: {$\beta$} Pic AB Dor, stars: pre-main sequence},
     year = 2012,
    month = oct,
   volume = 144,
      eid = {109},
    pages = {109},
      doi = {10.1088/0004-6256/144/4/109},
   adsurl = {http://adsabs.harvard.edu/abs/2012AJ....144..109S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mad11,
   author = {{Madhusudhan}, N. and {Burrows}, A. and {Currie}, T.},
    title = "{Model Atmospheres for Massive Gas Giants with Thick Clouds: Application to the HR 8799 Planets and Predictions for Future Detections}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1102.5089},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems, planets and satellites: general, planets and satellites: individual: HR 8799b HR 8799c HR 8799d},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {34},
    pages = {34},
      doi = {10.1088/0004-637X/737/1/34},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737...34M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mar06,
   author = {{Marois}, C. and {Lafreni{\`e}re}, D. and {Doyon}, R. and {Macintosh}, B. and 
	{Nadeau}, D.},
    title = "{Angular Differential Imaging: A Powerful High-Contrast Imaging Technique}",
  journal = {\apj},
   eprint = {astro-ph/0512335},
 keywords = {Instrumentation: Adaptive Optics, Stars: Planetary Systems, Stars: Imaging},
     year = 2006,
    month = apr,
   volume = 641,
    pages = {556-564},
      doi = {10.1086/500401},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...641..556M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rac99,
   author = {{Racine}, R. and {Walker}, G.~A.~H. and {Nadeau}, D. and {Doyon}, R. and 
	{Marois}, C.},
    title = "{Speckle Noise and the Detection of Faint Companions}",
  journal = {\pasp},
 keywords = {TECHNIQUES: IMAGE PROCESSING},
     year = 1999,
    month = may,
   volume = 111,
    pages = {587-594},
      doi = {10.1086/316367},
   adsurl = {http://adsabs.harvard.edu/abs/1999PASP..111..587R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Laf07,
   author = {{Lafreni{\`e}re}, D. and {Marois}, C. and {Doyon}, R. and {Nadeau}, D. and 
	{Artigau}, {\'E}.},
    title = "{A New Algorithm for Point-Spread Function Subtraction in High-Contrast Imaging: A Demonstration with Angular Differential Imaging}",
  journal = {\apj},
   eprint = {astro-ph/0702697},
 keywords = {Instrumentation: Adaptive Optics, Stars: Planetary Systems, Stars: Imaging, Techniques: High Angular Resolution, Techniques: Image Processing},
     year = 2007,
    month = may,
   volume = 660,
    pages = {770-780},
      doi = {10.1086/513180},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...660..770L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sou12,
   author = {{Soummer}, R. and {Pueyo}, L. and {Larkin}, J.},
    title = "{Detection and Characterization of Exoplanets and Disks Using Projections on Karhunen-Lo{\`e}ve Eigenimages}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1207.4197},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, techniques: image processing},
     year = 2012,
    month = aug,
   volume = 755,
      eid = {L28},
    pages = {L28},
      doi = {10.1088/2041-8205/755/2/L28},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...755L..28S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ama12,
   author = {{Amara}, A. and {Quanz}, S.~P.},
    title = "{PYNPOINT: an image processing package for finding exoplanets}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1207.6637},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, techniques: image processing, planets and satellites: detection},
     year = 2012,
    month = dec,
   volume = 427,
    pages = {948-955},
      doi = {10.1111/j.1365-2966.2012.21918.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427..948A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Can15,
   author = {{Cantalloube}, F. and {Mouillet}, D. and {Mugnier}, L.~M. and 
	{Milli}, J. and {Absil}, O. and {Gomez Gonzalez}, C.~A. and 
	{Chauvin}, G. and {Beuzit}, J.-L. and {Cornia}, A.},
    title = "{Direct exoplanet detection and characterization using the ANDROMEDA method: Performance on VLT/NaCo data}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1508.06406},
 primaryClass = "astro-ph.IM",
 keywords = {techniques: image processing, techniques: high angular resolution, instrumentation: adaptive optics, methods: data analysis, planets and satellites: detection},
     year = 2015,
    month = oct,
   volume = 582,
      eid = {A89},
    pages = {A89},
      doi = {10.1051/0004-6361/201425571},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...582A..89C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kuc02,
   author = {{Kuchner}, M.~J. and {Traub}, W.~A.},
    title = "{A Coronagraph with a Band-limited Mask for Finding Terrestrial Planets}",
  journal = {\apj},
   eprint = {astro-ph/0203455},
 keywords = {Astrobiology, Stars: Circumstellar Matter, Instrumentation: Adaptive Optics, Stars: Planetary Systems, Techniques: Interferometric},
     year = 2002,
    month = may,
   volume = 570,
    pages = {900-908},
      doi = {10.1086/339625},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...570..900K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sch16,
   author = {{Schwarz}, H. and {Ginski}, C. and {de Kok}, R.~J. and {Snellen}, I.~A.~G. and 
	{Brogi}, M. and {Birkby}, J.~L.},
    title = "{The slow spin of the young substellar companion GQ Lupi b and its orbital configuration}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1607.00012},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: individual: GQ Lupi b, techniques: imaging spectroscopy, infrared: planetary systems, planets and satellites: atmospheres, brown dwarfs},
     year = 2016,
    month = sep,
   volume = 593,
      eid = {A74},
    pages = {A74},
      doi = {10.1051/0004-6361/201628908},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...593A..74S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ske16,
   author = {{Skemer}, A.~J. and {Morley}, C.~V. and {Allers}, K.~N. and 
	{Geballe}, T.~R. and {Marley}, M.~S. and {Fortney}, J.~J. and 
	{Faherty}, J.~K. and {Bjoraker}, G.~L. and {Lupu}, R.},
    title = "{The First Spectrum of the Coldest Brown Dwarf}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1605.04902},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs},
     year = 2016,
    month = aug,
   volume = 826,
      eid = {L17},
    pages = {L17},
      doi = {10.3847/2041-8205/826/2/L17},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...826L..17S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yat16,
   author = {{Yates}, J.~S. and {Palmer}, P.~I. and {Biller}, B. and {Cockell}, C.~S.
	},
    title = "{Atmospheric Habitable Zones in Cool Y Dwarf Atmospheres}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1611.09074},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics},
     year = 2016,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161109074Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barn16,
   author = {{Barnes}, R. and {Deitrick}, R. and {Luger}, R. and {Driscoll}, P.~E. and 
	{Quinn}, T.~R. and {Fleming}, D.~P. and {Guyer}, B. and {McDonald}, D.~V. and 
	{Meadows}, V.~S. and {Arney}, G. and {Crisp}, D. and {Domagal-Goldman}, S.~D. and 
	{Lincowski}, A. and {Lustig-Yaeger}, J. and {Schwieterman}, E.
	},
    title = "{The Habitability of Proxima Centauri b I: Evolutionary Scenarios}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1608.06919},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics},
     year = 2016,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160806919B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Omal16,
   author = {{O'Malley-James}, J.~T. and {Kaltenegger}, L.},
    title = "{Biofluorescent Worlds: Biological fluorescence as a temporal biosignature for flare star worlds}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1608.06930},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics},
     year = 2016,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160806930O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gold16,
   author = {{Goldblatt}, C.},
    title = "{Tutorial models of the climate and habitability of Proxima Centauri b: a thin atmosphere is sufficient to distribute heat given low stellar flux}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1608.07263},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics, Physics - Atmospheric and Oceanic Physics},
     year = 2016,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160807263G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mead16,
   author = {{Meadows}, V.~S. and {Arney}, G.~N. and {Schwieterman}, E.~W. and 
	{Lustig-Yaeger}, J. and {Lincowski}, A.~P. and {Robinson}, T. and 
	{Domagal-Goldman}, S.~D. and {Barnes}, R.~K. and {Fleming}, D.~P. and 
	{Deitrick}, R. and {Luger}, R. and {Driscoll}, P.~E. and {Quinn}, T.~R. and 
	{Crisp}, D.},
    title = "{The Habitability of Proxima Centauri b: II: Environmental States and Observational Discriminants}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1608.08620},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics},
     year = 2016,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160808620M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lovi16,
   author = {{Lovis}, C. and {Snellen}, I. and {Mouillet}, D. and {Pepe}, F. and 
	{Wildi}, F. and {Astudillo-Defru}, N. and {Beuzit}, J.-L. and 
	{Bonfils}, X. and {Cheetham}, A. and {Conod}, U. and {Delfosse}, X. and 
	{Ehrenreich}, D. and {Figueira}, P. and {Forveille}, T. and 
	{Martins}, J.~H.~C. and {Quanz}, S.~P. and {Santos}, N.~C. and 
	{Schmid}, H.-M. and {S{\'e}gransan}, D. and {Udry}, S.},
    title = "{Atmospheric characterization of Proxima b by coupling the Sphere high-contrast imager to the Espresso spectrograph}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1609.03082},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2016,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160903082L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Luge16,
   author = {{Luger}, R. and {Lustig-Yaeger}, J. and {Fleming}, D.~P. and 
	{Tilley}, M.~A. and {Agol}, E. and {Meadows}, V.~S. and {Deitrick}, R. and 
	{Barnes}, R.},
    title = "{The Pale Green Dot: A Method to Characterize Proxima Centauri b using Exo-Aurorae}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1609.09075},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2016,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160909075L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shie16,
   author = {{Shields}, A.~L. and {Ballard}, S. and {Johnson}, J.~A.},
    title = "{The Habitability of Planets Orbiting M-dwarf Stars}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1610.05765},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
     year = 2016,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161005765S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krie16,
   author = {{Kreidberg}, L. and {Loeb}, A.},
    title = "{Prospects for Characterizing the Atmosphere of Proxima Centauri b}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1608.07345},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: atmospheres, planets and satellites: individual: Proxima Centauri b},
     year = 2016,
    month = nov,
   volume = 832,
      eid = {L12},
    pages = {L12},
      doi = {10.3847/2041-8205/832/1/L12},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...832L..12K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Riba16,
   author = {{Ribas}, I. and {Bolmont}, E. and {Selsis}, F. and {Reiners}, A. and 
	{Leconte}, J. and {Raymond}, S.~N. and {Engle}, S.~G. and {Guinan}, E.~F. and 
	{Morin}, J. and {Turbet}, M. and {Forget}, F. and {Anglada-Escud{\'e}}, G.
	},
    title = "{The habitability of Proxima Centauri b. I. Irradiation, rotation and volatile inventory from formation to the present}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1608.06813},
 primaryClass = "astro-ph.EP",
 keywords = {stars: individual: Proxima Cen, planets and satellites: individual: Proxima b, planets and satellites: atmospheres, X-rays: stars, planet-star interactions},
     year = 2016,
    month = dec,
   volume = 596,
      eid = {A111},
    pages = {A111},
      doi = {10.1051/0004-6361/201629576},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...596A.111R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garr16,
   author = {{Garraffo}, C. and {Drake}, J.~J. and {Cohen}, O.},
    title = "{The Space Weather of Proxima Centauri b}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1609.09076},
 primaryClass = "astro-ph.SR",
 keywords = {planets and satellites: terrestrial planets, stars: activity, stars: individual: Proxima Centauri, stars: late-type, stars: winds, outflows},
     year = 2016,
    month = dec,
   volume = 833,
      eid = {L4},
    pages = {L4},
      doi = {10.3847/2041-8205/833/1/L4},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...833L...4G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kane17,
   author = {{Kane}, S.~R. and {Gelino}, D.~M. and {Turnbull}, M.~C.},
    title = "{On the Orbital Inclination of Proxima Centauri b}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1612.02872},
 primaryClass = "astro-ph.EP",
 keywords = {astrobiology, planetary systems, stars: individual: Proxima Centauri, techniques: high angular resolution},
     year = 2017,
    month = feb,
   volume = 153,
      eid = {52},
    pages = {52},
      doi = {10.3847/1538-3881/153/2/52},
   adsurl = {http://adsabs.harvard.edu/abs/2017AJ....153...52K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kipp17,
   author = {{Kipping}, D.~M. and {Cameron}, C. and {Hartman}, J.~D. and 
	{Davenport}, J.~R.~A. and {Matthews}, J.~M. and {Sasselov}, D. and 
	{Rowe}, J. and {Siverd}, R.~J. and {Chen}, J. and {Sandford}, E. and 
	{Bakos}, G.~{\'A}. and {Jord{\'a}n}, A. and {Bayliss}, D. and 
	{Henning}, T. and {Mancini}, L. and {Penev}, K. and {Csubry}, Z. and 
	{Bhatti}, W. and {Da Silva Bento}, J. and {Guenther}, D.~B. and 
	{Kuschnig}, R. and {Moffat}, A.~F.~J. and {Rucinski}, S.~M. and 
	{Weiss}, W.~W.},
    title = "{No Conclusive Evidence for Transits of Proxima b in MOST Photometry}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1609.08718},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems, stars: individual: Proxima Centauri, techniques: photometric },
     year = 2017,
    month = mar,
   volume = 153,
      eid = {93},
    pages = {93},
      doi = {10.3847/1538-3881/153/3/93},
   adsurl = {http://adsabs.harvard.edu/abs/2017AJ....153...93K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mesa17,
   author = {{Mesa}, D. and {Zurlo}, A. and {Milli}, J. and {Gratton}, R. and 
	{Desidera}, S. and {Langlois}, M. and {Vigan}, A. and {Bonavita}, M. and 
	{Antichi}, J. and {Avenhaus}, H. and {Baruffolo}, A. and {Biller}, B. and 
	{Boccaletti}, A. and {Bruno}, P. and {Cascone}, E. and {Chauvin}, G. and 
	{Claudi}, R.~U. and {De Caprio}, V. and {Fantinel}, D. and {Farisato}, G. and 
	{Girard}, J. and {Giro}, E. and {Hagelberg}, J. and {Incorvaia}, S. and 
	{Janson}, M. and {Kral}, Q. and {Lagadec}, E. and {Lagrange}, A.-M. and 
	{Lessio}, L. and {Meyer}, M. and {Peretti}, S. and {Perrot}, C. and 
	{Salasnich}, B. and {Schlieder}, J. and {Schmid}, H.-M. and 
	{Scuderi}, S. and {Sissa}, E. and {Thalmann}, C. and {Turatto}, M.
	},
    title = "{Upper limits for mass and radius of objects around Proxima Cen from SPHERE/VLT}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1611.10362},
 primaryClass = "astro-ph.EP",
     year = 2017,
    month = mar,
   volume = 466,
    pages = {L118-L122},
      doi = {10.1093/mnrasl/slw241},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.466L.118M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Turb16,
   author = {{Turbet}, M. and {Leconte}, J. and {Selsis}, F. and {Bolmont}, E. and 
	{Forget}, F. and {Ribas}, I. and {Raymond}, S.~N. and {Anglada-Escud{\'e}}, G.
	},
    title = "{The habitability of Proxima Centauri b. II. Possible climates and observability}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1608.06827},
 primaryClass = "astro-ph.EP",
 keywords = {stars: individual: Proxima Cen, planets and satellites: individual: Proxima Cen b, planets and satellites: atmospheres, planets and satellites: terrestrial planets, planets and satellites: detection, astrobiology},
     year = 2016,
    month = dec,
   volume = 596,
      eid = {A112},
    pages = {A112},
      doi = {10.1051/0004-6361/201629577},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...596A.112T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sne15,
   author = {{Snellen}, I. and {de Kok}, R. and {Birkby}, J.~L. and {Brandl}, B. and 
	{Brogi}, M. and {Keller}, C. and {Kenworthy}, M. and {Schwarz}, H. and 
	{Stuik}, R.},
    title = "{Combining high-dispersion spectroscopy with high contrast imaging: Probing rocky planets around our nearest neighbors}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1503.01136},
 primaryClass = "astro-ph.EP",
 keywords = {infrared: planetary systems, techniques: imaging spectroscopy, techniques: high angular resolution, methods: data analysis},
     year = 2015,
    month = apr,
   volume = 576,
      eid = {A59},
    pages = {A59},
      doi = {10.1051/0004-6361/201425018},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...576A..59S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Atri17,
   author = {{Atri}, D.},
    title = "{Modelling stellar proton event-induced particle radiation dose on close-in exoplanets}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1606.07027},
 primaryClass = "astro-ph.EP",
     year = 2017,
    month = feb,
   volume = 465,
    pages = {L34-L38},
      doi = {10.1093/mnrasl/slw199},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.465L..34A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaid04,
   author = {{Gaidos}, E. and {Williams}, D.~M.},
    title = "{Seasonality on terrestrial extrasolar planets: inferring obliquity and surface conditions from infrared light curves}",
  journal = {\na},
     year = 2004,
    month = nov,
   volume = 10,
    pages = {67-77},
      doi = {10.1016/j.newast.2004.04.009},
   adsurl = {http://adsabs.harvard.edu/abs/2004NewA...10...67G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Seag09,
   author = {{Seager}, S. and {Deming}, D.},
    title = "{On the Method to Infer an Atmosphere on a Tidally Locked Super Earth Exoplanet and Upper Limits to GJ 876d}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0910.1505},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems, stars: individual: GJ 876, techniques: photometric},
     year = 2009,
    month = oct,
   volume = 703,
    pages = {1884-1889},
      doi = {10.1088/0004-637X/703/2/1884},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...703.1884S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sels11,
   author = {{Selsis}, F. and {Wordsworth}, R.~D. and {Forget}, F.},
    title = "{Thermal phase curves of nontransiting terrestrial exoplanets. I. Characterizing atmospheres}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1104.4763},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: atmospheres, planetary systems, standards},
     year = 2011,
    month = aug,
   volume = 532,
      eid = {A1},
    pages = {A1},
      doi = {10.1051/0004-6361/201116654},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...532A...1S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sels13,
   author = {{Selsis}, F. and {Maurin}, A.-S. and {Hersant}, F. and {Leconte}, J. and 
	{Bolmont}, E. and {Raymond}, S.~N. and {Delbo'}, M.},
    title = "{The effect of rotation and tidal heating on the thermal lightcurves of super Mercuries}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1305.3858},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: photometric, planetary systems},
     year = 2013,
    month = jul,
   volume = 555,
      eid = {A51},
    pages = {A51},
      doi = {10.1051/0004-6361/201321661},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...555A..51S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maur12,
   author = {{Maurin}, A.~S. and {Selsis}, F. and {Hersant}, F. and {Belu}, A.
	},
    title = "{Thermal phase curves of nontransiting terrestrial exoplanets. II. Characterizing airless planets}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.3087},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: spectroscopic, methods: numerical, infrared: planetary, systems, methods: statistical},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A95},
    pages = {A95},
      doi = {10.1051/0004-6361/201117054},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538A..95M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Riau07,
   author = {{Riaud}, P. and {Schneider}, J.},
    title = "{Improving Earth-like planets' detection with an ELT: the differential radial velocity experiment}",
  journal = {\aap},
 keywords = {stars: planetary systems, techniques: spectroscopic, techniques: radial velocities, astrobiology},
     year = 2007,
    month = jul,
   volume = 469,
    pages = {355-361},
      doi = {10.1051/0004-6361:20077085},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..355R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dave16,
   author = {{Davenport}, J.~R.~A. and {Kipping}, D.~M. and {Sasselov}, D. and 
	{Matthews}, J.~M. and {Cameron}, C.},
    title = "{MOST Observations of Our Nearest Neighbor: Flares on Proxima Centauri}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1608.06672},
 primaryClass = "astro-ph.SR",
 keywords = {stars: flare, stars: individual: Proxima Cen, stars: low-mass },
     year = 2016,
    month = oct,
   volume = 829,
      eid = {L31},
    pages = {L31},
      doi = {10.3847/2041-8205/829/2/L31},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...829L..31D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Rick10,
   author = {{Ricker}, G.~R. and {Winn}, J.~N. and {Vanderspek}, R. and {Latham}, D.~W. and 
	{Bakos}, G.~{\'A}. and {Bean}, J.~L. and {Berta-Thompson}, Z.~K. and 
	{Brown}, T.~M. and {Buchhave}, L. and {Butler}, N.~R. and {Butler}, R.~P. and 
	{Chaplin}, W.~J. and {Charbonneau}, D. and {Christensen-Dalsgaard}, J. and 
	{Clampin}, M. and {Deming}, D. and {Doty}, J. and {De Lee}, N. and 
	{Dressing}, C. and {Dunham}, E.~W. and {Endl}, M. and {Fressin}, F. and 
	{Ge}, J. and {Henning}, T. and {Holman}, M.~J. and {Howard}, A.~W. and 
	{Ida}, S. and {Jenkins}, J. and {Jernigan}, G. and {Johnson}, J.~A. and 
	{Kaltenegger}, L. and {Kawai}, N. and {Kjeldsen}, H. and {Laughlin}, G. and 
	{Levine}, A.~M. and {Lin}, D. and {Lissauer}, J.~J. and {MacQueen}, P. and 
	{Marcy}, G. and {McCullough}, P.~R. and {Morton}, T.~D. and 
	{Narita}, N. and {Paegert}, M. and {Palle}, E. and {Pepe}, F. and 
	{Pepper}, J. and {Quirrenbach}, A. and {Rinehart}, S.~A. and 
	{Sasselov}, D. and {Sato}, B. and {Seager}, S. and {Sozzetti}, A. and 
	{Stassun}, K.~G. and {Sullivan}, P. and {Szentgyorgyi}, A. and 
	{Torres}, G. and {Udry}, S. and {Villasenor}, J.},
    title = "{Transiting Exoplanet Survey Satellite (TESS)}",
booktitle = {Space Telescopes and Instrumentation 2014: Optical, Infrared, and Millimeter Wave},
     year = 2014,
   series = {\procspie},
   volume = 9143,
archivePrefix = "arXiv",
   eprint = {1406.0151},
 primaryClass = "astro-ph.EP",
    month = aug,
      eid = {914320},
    pages = {914320},
      doi = {10.1117/12.2063489},
   adsurl = {http://adsabs.harvard.edu/abs/2014SPIE.9143E..20R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sull15,
   author = {{Sullivan}, P.~W. and {Winn}, J.~N. and {Berta-Thompson}, Z.~K. and 
	{Charbonneau}, D. and {Deming}, D. and {Dressing}, C.~D. and 
	{Latham}, D.~W. and {Levine}, A.~M. and {McCullough}, P.~R. and 
	{Morton}, T. and {Ricker}, G.~R. and {Vanderspek}, R. and {Woods}, D.
	},
    title = "{The Transiting Exoplanet Survey Satellite: Simulations of Planet Detections and Astrophysical False Positives}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1506.03845},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: detection, space vehicles: instruments, surveys},
     year = 2015,
    month = aug,
   volume = 809,
      eid = {77},
    pages = {77},
      doi = {10.1088/0004-637X/809/1/77},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...809...77S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Doma14,
   author = {{Domagal-Goldman}, S.~D. and {Segura}, A. and {Claire}, M.~W. and 
	{Robinson}, T.~D. and {Meadows}, V.~S.},
    title = "{Abiotic Ozone and Oxygen in Atmospheres Similar to Prebiotic Earth}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1407.2622},
 primaryClass = "astro-ph.EP",
 keywords = {Earth, infrared: planetary systems, planets and satellites: atmospheres, planets and satellites: terrestrial planets, planet-star interactions, ultraviolet: planetary systems },
     year = 2014,
    month = sep,
   volume = 792,
      eid = {90},
    pages = {90},
      doi = {10.1088/0004-637X/792/2/90},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...792...90D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Luga15,
   author = {{Luger}, R. and {Barnes}, R.},
    title = "{Extreme Water Loss and Abiotic O2Buildup on Planets Throughout the Habitable Zones of M Dwarfs}",
  journal = {Astrobiology},
archivePrefix = "arXiv",
   eprint = {1411.7412},
 primaryClass = "astro-ph.EP",
     year = 2015,
    month = feb,
   volume = 15,
    pages = {119-143},
      doi = {10.1089/ast.2014.1231},
   adsurl = {http://adsabs.harvard.edu/abs/2015AsBio..15..119L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Harm15,
   author = {{Harman}, C.~E. and {Schwieterman}, E.~W. and {Schottelkotte}, J.~C. and 
	{Kasting}, J.~F.},
    title = "{Abiotic O$_{2}$ Levels on Planets around F, G, K, and M Stars: Possible False Positives for Life?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1509.07863},
 primaryClass = "astro-ph.EP",
 keywords = {planet{\ndash}star interactions, planets and satellites: atmospheres, planets and satellites: terrestrial planets, ultraviolet: planetary systems},
     year = 2015,
    month = oct,
   volume = 812,
      eid = {137},
    pages = {137},
      doi = {10.1088/0004-637X/812/2/137},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...812..137H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kane16,
   author = {{Kane}, S.~R. and {Hill}, M.~L. and {Kasting}, J.~F. and {Kopparapu}, R.~K. and 
	{Quintana}, E.~V. and {Barclay}, T. and {Batalha}, N.~M. and 
	{Borucki}, W.~J. and {Ciardi}, D.~R. and {Haghighipour}, N. and 
	{Hinkel}, N.~R. and {Kaltenegger}, L. and {Selsis}, F. and {Torres}, G.
	},
    title = "{A Catalog of Kepler Habitable Zone Exoplanet Candidates}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1608.00620},
 primaryClass = "astro-ph.EP",
 keywords = {astrobiology, astronomical databases: miscellaneous, planetary systems, techniques: photometric},
     year = 2016,
    month = oct,
   volume = 830,
      eid = {1},
    pages = {1},
      doi = {10.3847/0004-637X/830/1/1},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...830....1K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cro13,
   author = {{Crossfield}, I.~J.~M.},
    title = "{On high-contrast characterization of nearby, short-period exoplanets with giant segmented-mirror telescopes}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1301.5884},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: general, planets and satellites: detection, instrumentation: adaptive optics, methods: numerical, techniques: high angular resolution},
     year = 2013,
    month = mar,
   volume = 551,
      eid = {A99},
    pages = {A99},
      doi = {10.1051/0004-6361/201220914},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...551A..99C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Laws12,
   author = {{Lawson}, P.~R. and {Poyneer}, L. and {Barrett}, H. and {Frazin}, R. and 
	{Caucci}, L. and {Devaney}, N. and {Furenlid}, L. and {G{\l}adysz}, S. and 
	{Guyon}, O. and {Krist}, J. and {Maire}, J. and {Marois}, C. and 
	{Mawet}, D. and {Mouillet}, D. and {Mugnier}, L. and {Pearson}, I. and 
	{Perrin}, M. and {Pueyo}, L. and {Savransky}, D.},
    title = "{On advanced estimation techniques for exoplanet detection and characterization using ground-based coronagraphs}",
booktitle = {Adaptive Optics Systems III},
     year = 2012,
   series = {\procspie},
   volume = 8447,
    month = jul,
      eid = {844722},
    pages = {844722},
      doi = {10.1117/12.925099},
   adsurl = {http://adsabs.harvard.edu/abs/2012SPIE.8447E..22L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Mawe12,
   author = {{Mawet}, D. and {Pueyo}, L. and {Lawson}, P. and {Mugnier}, L. and 
	{Traub}, W. and {Boccaletti}, A. and {Trauger}, J.~T. and {Gladysz}, S. and 
	{Serabyn}, E. and {Milli}, J. and {Belikov}, R. and {Kasper}, M. and 
	{Baudoz}, P. and {Macintosh}, B. and {Marois}, C. and {Oppenheimer}, B. and 
	{Barrett}, H. and {Beuzit}, J.-L. and {Devaney}, N. and {Girard}, J. and 
	{Guyon}, O. and {Krist}, J. and {Mennesson}, B. and {Mouillet}, D. and 
	{Murakami}, N. and {Poyneer}, L. and {Savransky}, D. and {V{\'e}rinaud}, C. and 
	{Wallace}, J.~K.},
    title = "{Review of small-angle coronagraphic techniques in the wake of ground-based second-generation adaptive optics systems}",
booktitle = {Space Telescopes and Instrumentation 2012: Optical, Infrared, and Millimeter Wave},
     year = 2012,
   series = {\procspie},
   volume = 8442,
archivePrefix = "arXiv",
   eprint = {1207.5481},
 primaryClass = "astro-ph.IM",
    month = sep,
      eid = {844204},
    pages = {844204},
      doi = {10.1117/12.927245},
   adsurl = {http://adsabs.harvard.edu/abs/2012SPIE.8442E..04M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Quan15,
   author = {{Quanz}, S.~P. and {Crossfield}, I. and {Meyer}, M.~R. and {Schmalzl}, E. and 
	{Held}, J.},
    title = "{Direct detection of exoplanets in the 3-10 {$\mu$}m range with E-ELT/METIS}",
  journal = {International Journal of Astrobiology},
archivePrefix = "arXiv",
   eprint = {1404.0831},
 primaryClass = "astro-ph.IM",
 keywords = {high angular resolution, infrared, instrumentation, planetary systems,},
     year = 2015,
    month = apr,
   volume = 14,
    pages = {279-289},
      doi = {10.1017/S1473550414000135},
   adsurl = {http://adsabs.harvard.edu/abs/2015IJAsB..14..279Q},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krei14,
   author = {{Kreidberg}, L. and {Bean}, J.~L. and {D{\'e}sert}, J.-M. and 
	{Benneke}, B. and {Deming}, D. and {Stevenson}, K.~B. and {Seager}, S. and 
	{Berta-Thompson}, Z. and {Seifahrt}, A. and {Homeier}, D.},
    title = "{Clouds in the atmosphere of the super-Earth exoplanet GJ1214b}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1401.0022},
 primaryClass = "astro-ph.EP",
     year = 2014,
    month = jan,
   volume = 505,
    pages = {69-72},
      doi = {10.1038/nature12888},
   adsurl = {http://adsabs.harvard.edu/abs/2014Natur.505...69K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sing16,
   author = {{Sing}, D.~K. and {Fortney}, J.~J. and {Nikolov}, N. and {Wakeford}, H.~R. and 
	{Kataria}, T. and {Evans}, T.~M. and {Aigrain}, S. and {Ballester}, G.~E. and 
	{Burrows}, A.~S. and {Deming}, D. and {D{\'e}sert}, J.-M. and 
	{Gibson}, N.~P. and {Henry}, G.~W. and {Huitson}, C.~M. and 
	{Knutson}, H.~A. and {Lecavelier Des Etangs}, A. and {Pont}, F. and 
	{Showman}, A.~P. and {Vidal-Madjar}, A. and {Williamson}, M.~H. and 
	{Wilson}, P.~A.},
    title = "{A continuum from clear to cloudy hot-Jupiter exoplanets without primordial water depletion}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1512.04341},
 primaryClass = "astro-ph.EP",
     year = 2016,
    month = jan,
   volume = 529,
    pages = {59-62},
      doi = {10.1038/nature16068},
   adsurl = {http://adsabs.harvard.edu/abs/2016Natur.529...59S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Morl15,
   author = {{Morley}, C.~V. and {Fortney}, J.~J. and {Marley}, M.~S. and 
	{Zahnle}, K. and {Line}, M. and {Kempton}, E. and {Lewis}, N. and 
	{Cahoy}, K.},
    title = "{Thermal Emission and Reflected Light Spectra of Super Earths with Flat Transmission Spectra}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1511.01492},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: atmospheres, planets and satellites: individual: GJ 1214b},
     year = 2015,
    month = dec,
   volume = 815,
      eid = {110},
    pages = {110},
      doi = {10.1088/0004-637X/815/2/110},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...815..110M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Seag15,
   author = {{Seager}, S. and {Turnbull}, M. and {Sparks}, W. and {Thomson}, M. and 
	{Shaklan}, S.~B. and {Roberge}, A. and {Kuchner}, M. and {Kasdin}, N.~J. and 
	{Domagal-Goldman}, S. and {Cash}, W. and {Warfield}, K. and 
	{Lisman}, D. and {Scharf}, D. and {Webb}, D. and {Trabert}, R. and 
	{Martin}, S. and {Cady}, E. and {Heneghan}, C.},
    title = "{The Exo-S probe class starshade mission}",
booktitle = {Techniques and Instrumentation for Detection of Exoplanets VII},
     year = 2015,
   series = {\procspie},
   volume = 9605,
    month = sep,
      eid = {96050W},
    pages = {96050W},
      doi = {10.1117/12.2190378},
   adsurl = {http://adsabs.harvard.edu/abs/2015SPIE.9605E..0WS},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dalc15,
   author = {{Dalcanton}, J. and {Seager}, S. and {Aigrain}, S. and {Battel}, S. and 
	{Brandt}, N. and {Conroy}, C. and {Feinberg}, L. and {Gezari}, S. and 
	{Guyon}, O. and {Harris}, W. and {Hirata}, C. and {Mather}, J. and 
	{Postman}, M. and {Redding}, D. and {Schiminovich}, D. and {Stahl}, H.~P. and 
	{Tumlinson}, J.},
    title = "{From Cosmic Birth to Living Earths: The Future of UVOIR Space Astronomy}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1507.04779},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
     year = 2015,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150704779D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Robi16,
   author = {{Robinson}, T.~D. and {Stapelfeldt}, K.~R. and {Marley}, M.~S.
	},
    title = "{Characterizing Rocky and Gaseous Exoplanets with 2 m Class Space-based Coronagraphs}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1507.00777},
 primaryClass = "astro-ph.EP",
     year = 2016,
    month = feb,
   volume = 128,
   number = 2,
    pages = {025003},
      doi = {10.1088/1538-3873/128/960/025003},
   adsurl = {http://adsabs.harvard.edu/abs/2016PASP..128b5003R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Noec16,
   author = {{Noecker}, M.~C. and {Zhao}, F. and {Demers}, R. and {Trauger}, J. and 
	{Guyon}, O. and {Jeremy Kasdin}, N.},
    title = "{Coronagraph instrument for WFIRST-AFTA}",
  journal = {Journal of Astronomical Telescopes, Instruments, and Systems},
     year = 2016,
    month = jan,
   volume = 2,
   number = 1,
      eid = {011001},
    pages = {011001},
      doi = {10.1117/1.JATIS.2.1.011001},
   adsurl = {http://adsabs.harvard.edu/abs/2016JATIS...2a1001N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Maci06,
   author = {{Macintosh}, B. and {Troy}, M. and {Doyon}, R. and {Graham}, J. and 
	{Baker}, K. and {Bauman}, B. and {Marois}, C. and {Palmer}, D. and 
	{Phillion}, D. and {Poyneer}, L. and {Crossfield}, I. and {Dumont}, P. and 
	{Levine}, B.~M. and {Shao}, M. and {Serabyn}, G. and {Shelton}, C. and 
	{Vasisht}, G. and {Wallace}, J.~K. and {Lavigne}, J.-F. and 
	{Valee}, P. and {Rowlands}, N. and {Tam}, K. and {Hackett}, D.
	},
    title = "{Extreme adaptive optics for the Thirty Meter Telescope}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2006,
   series = {\procspie},
   volume = 6272,
    month = jun,
      eid = {62720N},
    pages = {62720N},
      doi = {10.1117/12.672032},
   adsurl = {http://adsabs.harvard.edu/abs/2006SPIE.6272E..0NM},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Kasp10,
   author = {{Kasper}, M. and {Beuzit}, J.-L. and {Verinaud}, C. and {Gratton}, R.~G. and 
	{Kerber}, F. and {Yaitskova}, N. and {Boccaletti}, A. and {Thatte}, N. and 
	{Schmid}, H.~M. and {Keller}, C. and {Baudoz}, P. and {Abe}, L. and 
	{Aller-Carpentier}, E. and {Antichi}, J. and {Bonavita}, M. and 
	{Dohlen}, K. and {Fedrigo}, E. and {Hanenburg}, H. and {Hubin}, N. and 
	{Jager}, R. and {Korkiakoski}, V. and {Martinez}, P. and {Mesa}, D. and 
	{Preis}, O. and {Rabou}, P. and {Roelfsema}, R. and {Salter}, G. and 
	{Tecza}, M. and {Venema}, L.},
    title = "{EPICS: direct imaging of exoplanets with the E-ELT}",
booktitle = {Ground-based and Airborne Instrumentation for Astronomy III},
     year = 2010,
   series = {\procspie},
   volume = 7735,
    month = jul,
      eid = {77352E-77352E-9},
    pages = {77352E-77352E-9},
      doi = {10.1117/12.856850},
   adsurl = {http://adsabs.harvard.edu/abs/2010SPIE.7735E..2EK},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Davi16,
   author = {{Davies}, R. and {Schubert}, J. and {Hartl}, M. and {Alves}, J. and 
	{Cl{\'e}net}, Y. and {Lang-Bardl}, F. and {Nicklas}, H. and 
	{Pott}, J.-U. and {Ragazzoni}, R. and {Tolstoy}, E. and {Agocs}, T. and 
	{Anwand-Heerwart}, H. and {Barboza}, S. and {Baudoz}, P. and 
	{Bender}, R. and {Bizenberger}, P. and {Boccaletti}, A. and 
	{Boland}, W. and {Bonifacio}, P. and {Briegel}, F. and {Buey}, T. and 
	{Chapron}, F. and {Cohen}, M. and {Czoske}, O. and {Dreizler}, S. and 
	{Falomo}, R. and {Feautrier}, P. and {F{\"o}rster Schreiber}, N. and 
	{Gendron}, E. and {Genzel}, R. and {Gl{\"u}ck}, M. and {Gratadour}, D. and 
	{Greimel}, R. and {Grupp}, F. and {H{\"a}user}, M. and {Haug}, M. and 
	{Hennawi}, J. and {Hess}, H.~J. and {H{\"o}rmann}, V. and {Hofferbert}, R. and 
	{Hopp}, U. and {Hubert}, Z. and {Ives}, D. and {Kausch}, W. and 
	{Kerber}, F. and {Kravcar}, H. and {Kuijken}, K. and {Lang-Bardl}, F. and 
	{Leitzinger}, M. and {Leschinski}, K. and {Massari}, D. and 
	{Mei}, S. and {Merlin}, F. and {Mohr}, L. and {Monna}, A. and 
	{M{\"u}ller}, F. and {Navarro}, R. and {Plattner}, M. and {Przybilla}, N. and 
	{Ramlau}, R. and {Ramsay}, S. and {Ratzka}, T. and {Rhode}, P. and 
	{Richter}, J. and {Rix}, H.-W. and {Rodeghiero}, G. and {Rohloff}, R.-R. and 
	{Rousset}, G. and {Ruddenklau}, R. and {Schaffenroth}, V. and 
	{Schlichter}, J. and {Sevin}, A. and {Stuik}, R. and {Sturm}, E. and 
	{Thomas}, J. and {Tromp}, N. and {Turatto}, M. and {Verdoes-Kleijn}, G. and 
	{Vidal}, F. and {Wagner}, R. and {Wegner}, M. and {Zeilinger}, W. and 
	{Ziegler}, B. and {Zins}, G.},
    title = "{MICADO: first light imager for the E-ELT}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2016,
   series = {\procspie},
   volume = 9908,
archivePrefix = "arXiv",
   eprint = {1607.01954},
 primaryClass = "astro-ph.IM",
    month = aug,
      eid = {99081Z},
    pages = {99081Z},
      doi = {10.1117/12.2233047},
   adsurl = {http://adsabs.harvard.edu/abs/2016SPIE.9908E..1ZD},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Beli15,
   author = {{Belikov}, R. and {Bendek}, E. and {Thomas}, S. and {Males}, J. and 
	{Lozi}, J.},
    title = "{How to directly image a habitable planet around Alpha Centauri with a \~{}30-45cm space telescope}",
booktitle = {Techniques and Instrumentation for Detection of Exoplanets VII},
     year = 2015,
   series = {\procspie},
   volume = 9605,
archivePrefix = "arXiv",
   eprint = {1510.02479},
 primaryClass = "astro-ph.IM",
    month = sep,
      eid = {960517},
    pages = {960517},
      doi = {10.1117/12.2188732},
   adsurl = {http://adsabs.harvard.edu/abs/2015SPIE.9605E..17B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Grof16,
   author = {{Groff}, T.~D. and {Chilcote}, J. and {Kasdin}, N.~J. and {Galvin}, M. and 
	{Loomis}, C. and {Carr}, M.~A. and {Brandt}, T. and {Knapp}, G. and 
	{Limbach}, M.~A. and {Guyon}, O. and {Jovanovic}, N. and {McElwain}, M.~W. and 
	{Takato}, N. and {Hayashi}, M.},
    title = "{Laboratory testing and performance verification of the CHARIS integral field spectrograph}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2016,
   series = {\procspie},
   volume = 9908,
    month = aug,
      eid = {99080O},
    pages = {99080O},
      doi = {10.1117/12.2233447},
   adsurl = {http://adsabs.harvard.edu/abs/2016SPIE.9908E..0OG},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mair15,
   author = {{Maire}, A.-L. and {Bonnefoy}, M. and {Ginski}, C. and {Vigan}, A. and 
	{Messina}, S. and {Mesa}, D. and {Galicher}, R. and {Gratton}, R. and 
	{Desidera}, S. and {Kopytova}, T.~G. and {Millward}, M. and 
	{Thalmann}, C. and {Claudi}, R.~U. and {Ehrenreich}, D. and 
	{Zurlo}, A. and {Chauvin}, G. and {Antichi}, J. and {Baruffolo}, A. and 
	{Bazzon}, A. and {Beuzit}, J.-L. and {Blanchard}, P. and {Boccaletti}, A. and 
	{de Boer}, J. and {Carle}, M. and {Cascone}, E. and {Costille}, A. and 
	{De Caprio}, V. and {Delboulb{\'e}}, A. and {Dohlen}, K. and 
	{Dominik}, C. and {Feldt}, M. and {Fusco}, T. and {Girard}, J.~H. and 
	{Giro}, E. and {Gisler}, D. and {Gluck}, L. and {Gry}, C. and 
	{Henning}, T. and {Hubin}, N. and {Hugot}, E. and {Jaquet}, M. and 
	{Kasper}, M. and {Lagrange}, A.-M. and {Langlois}, M. and {Le Mignant}, D. and 
	{Llored}, M. and {Madec}, F. and {Martinez}, P. and {Mawet}, D. and 
	{Milli}, J. and {M{\"o}ller-Nilsson}, O. and {Mouillet}, D. and 
	{Moulin}, T. and {Moutou}, C. and {Orign{\'e}}, A. and {Pavlov}, A. and 
	{Petit}, C. and {Pragt}, J. and {Puget}, P. and {Ramos}, J. and 
	{Rochat}, S. and {Roelfsema}, R. and {Salasnich}, B. and {Sauvage}, J.-F. and 
	{Schmid}, H.~M. and {Turatto}, M. and {Udry}, S. and {Vakili}, F. and 
	{Wahhaj}, Z. and {Weber}, L. and {Wildi}, F.},
    title = "{First light of the VLT planet finder SPHERE. II. The physical properties and the architecture of the young systems PZ Telescopii and HD 1160 revisited}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1511.04072},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, stars: individual: PZ Telescopii, stars: individual: HD 1160, techniques: high angular resolution, techniques: image processing, techniques: spectroscopic},
     year = 2016,
    month = mar,
   volume = 587,
      eid = {A56},
    pages = {A56},
      doi = {10.1051/0004-6361/201526594},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...587A..56M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Morz15,
   author = {{Morzinski}, K.~M. and {Males}, J.~R. and {Skemer}, A.~J. and 
	{Close}, L.~M. and {Hinz}, P.~M. and {Rodigas}, T.~J. and {Puglisi}, A. and 
	{Esposito}, S. and {Riccardi}, A. and {Pinna}, E. and {Xompero}, M. and 
	{Briguglio}, R. and {Bailey}, V.~P. and {Follette}, K.~B. and 
	{Kopon}, D. and {Weinberger}, A.~J. and {Wu}, Y.-L.},
    title = "{Magellan Adaptive Optics First-light Observations of the Exoplanet {$\beta$} Pic b. II. 3-5 {$\mu$}m Direct Imaging with MagAO+Clio, and the Empirical Bolometric Luminosity of a Self-luminous Giant Planet}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1511.02894},
 primaryClass = "astro-ph.EP",
 keywords = {instrumentation: adaptive optics, planetary systems, planets and satellites: individual: Beta Pictoris b, stars: individual: Beta Pictoris},
     year = 2015,
    month = dec,
   volume = 815,
      eid = {108},
    pages = {108},
      doi = {10.1088/0004-637X/815/2/108},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...815..108M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Wu17,
   author = {{Wu}, Y.-L. and {Sheehan}, P.~D. and {Males}, J.~R. and {Close}, L.~M. and 
	{Morzinski}, K.~M. and {Teske}, J.~K. and {Haug-Baltzell}, A. and 
	{Merchant}, N. and {Lyons}, E.},
    title = "{An ALMA and MagAO Study of the Substellar Companion GQ Lup B}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1701.07541},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
     year = 2017,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170107541W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Quil98,
   author = {{Quillen}, A.~C. and {Trilling}, D.~E.},
    title = "{Do Proto-jovian Planets Drive Outflows?}",
  journal = {\apj},
   eprint = {astro-ph/9712033},
 keywords = {ISM: JETS AND OUTFLOWS, MAGNETOHYDRODYNAMICS: MHD, STARS: PLANETARY SYSTEMS, STARS: MASS LOSS, STARS: PRE-MAIN-SEQUENCE, ISM: Jets and Outflows, Magnetohydrodynamics: MHD, Stars: Planetary Systems, Stars: Mass Loss, Stars: Pre-Main-Sequence},
     year = 1998,
    month = dec,
   volume = 508,
    pages = {707-713},
      doi = {10.1086/306421},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...508..707Q},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Seif07,
   author = {{Seifahrt}, A. and {Neuh{\"a}user}, R. and {Hauschildt}, P.~H.
	},
    title = "{Near-infrared integral-field spectroscopy of the companion to GQ Lupi}",
  journal = {\aap},
   eprint = {astro-ph/0612250},
 keywords = {stars: low-mass, brown dwarfs, planetary systems, techniques: spectroscopic},
     year = 2007,
    month = feb,
   volume = 463,
    pages = {309-313},
      doi = {10.1051/0004-6361:20066463},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...463..309S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schm08,
   author = {{Schmidt}, T.~O.~B. and {Neuh{\"a}user}, R. and {Seifahrt}, A. and 
	{Vogt}, N. and {Bedalov}, A. and {Helling}, C. and {Witte}, S. and 
	{Hauschildt}, P.~H.},
    title = "{Direct evidence of a sub-stellar companion around CT Chamaeleontis}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0809.2812},
 keywords = {stars: pre-main sequence, stars: planetary systems: formation, stars: individual: CT Cha},
     year = 2008,
    month = nov,
   volume = 491,
    pages = {311-320},
      doi = {10.1051/0004-6361:20078840},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...491..311S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bowl16,
   author = {{Bowler}, B.~P.},
    title = "{Imaging Extrasolar Giant Planets}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1605.02731},
 primaryClass = "astro-ph.EP",
     year = 2016,
    month = oct,
   volume = 128,
   number = 10,
    pages = {102001},
      doi = {10.1088/1538-3873/128/968/102001},
   adsurl = {http://adsabs.harvard.edu/abs/2016PASP..128j2001B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bowl11,
   author = {{Bowler}, B.~P. and {Liu}, M.~C. and {Kraus}, A.~L. and {Mann}, A.~W. and 
	{Ireland}, M.~J.},
    title = "{A Disk around the Planetary-mass Companion GSC 06214-00210 b: Clues about the Formation of Gas Giants on Wide Orbits}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1109.5693},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: formation, stars: individual: GSC 06214-00210, stars: pre-main sequence},
     year = 2011,
    month = dec,
   volume = 743,
      eid = {148},
    pages = {148},
      doi = {10.1088/0004-637X/743/2/148},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743..148B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bowl14,
   author = {{Bowler}, B.~P. and {Liu}, M.~C. and {Kraus}, A.~L. and {Mann}, A.~W.
	},
    title = "{Spectroscopic Confirmation of Young Planetary-mass Companions on Wide Orbits}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1401.7668},
 primaryClass = "astro-ph.EP",
 keywords = {brown dwarfs, planetary systems, stars: individual: ROXs 42B FW Tau GSC 6214-210 SR 12, stars: low-mass},
     year = 2014,
    month = mar,
   volume = 784,
      eid = {65},
    pages = {65},
      doi = {10.1088/0004-637X/784/1/65},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...784...65B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonn14,
   author = {{Bonnefoy}, M. and {Chauvin}, G. and {Lagrange}, A.-M. and {Rojo}, P. and 
	{Allard}, F. and {Pinte}, C. and {Dumas}, C. and {Homeier}, D.
	},
    title = "{A library of near-infrared integral field spectra of young M-L dwarfs}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1306.3709},
 primaryClass = "astro-ph.SR",
 keywords = {stars: low-mass, brown dwarfs, planetary systems, techniques: spectroscopic},
     year = 2014,
    month = feb,
   volume = 562,
      eid = {A127},
    pages = {A127},
      doi = {10.1051/0004-6361/201118270},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...562A.127B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Natt14,
   author = {{Natta}, A. and {Testi}, L. and {Muzerolle}, J. and {Randich}, S. and 
	{Comer{\'o}n}, F. and {Persi}, P.},
    title = "{Accretion in brown dwarfs: An infrared view}",
  journal = {\aap},
   eprint = {astro-ph/0406106},
 keywords = {stars: low-mass, brown dwarfs, stars: formation, stars: activity, line: profiles, accretion, accretion disks},
     year = 2004,
    month = sep,
   volume = 424,
    pages = {603-612},
      doi = {10.1051/0004-6361:20040356},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...424..603N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Joer13,
   author = {{Joergens}, V. and {Bonnefoy}, M. and {Liu}, Y. and {Bayo}, A. and 
	{Wolf}, S. and {Chauvin}, G. and {Rojo}, P.},
    title = "{OTS 44: Disk and accretion at the planetary border}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1310.1936},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: pre-main sequence, circumstellar matter, accretion, accretion disks, stars: formation, stars: individual: OTS 44},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {L7},
    pages = {L7},
      doi = {10.1051/0004-6361/201322432},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...558L...7J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lavi09,
   author = {{Lavigne}, J.-F. and {Doyon}, R. and {Lafreni{\`e}re}, D. and 
	{Marois}, C. and {Barman}, T.},
    title = "{Near-Infrared Observations of GQ Lup b Using the Gemini Integral Field Spectrograph NIFS}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0908.3723},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems, stars: individual: GQ Lup, stars: low-mass, brown dwarfs, stars: pre-main sequence, techniques: high angular resolution, techniques: spectroscopic},
     year = 2009,
    month = oct,
   volume = 704,
    pages = {1098-1106},
      doi = {10.1088/0004-637X/704/2/1098},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...704.1098L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lach15,
   author = {{Lachapelle}, F.-R. and {Lafreni{\`e}re}, D. and {Gagn{\'e}}, J. and 
	{Jayawardhana}, R. and {Janson}, M. and {Helling}, C. and {Witte}, S.
	},
    title = "{Characterization of Low-mass, Wide-separation Substellar Companions to Stars in Upper Scorpius: Near-infrared Photometry and Spectroscopy}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1503.07586},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, infrared: planetary systems, stars: atmospheres, stars: imaging, stars: low-mass, stars: pre-main sequence},
     year = 2015,
    month = mar,
   volume = 802,
      eid = {61},
    pages = {61},
      doi = {10.1088/0004-637X/802/1/61},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...802...61L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marl07,
   author = {{Marley}, M.~S. and {Fortney}, J.~J. and {Hubickyj}, O. and 
	{Bodenheimer}, P. and {Lissauer}, J.~J.},
    title = "{On the Luminosity of Young Jupiters}",
  journal = {\apj},
   eprint = {astro-ph/0609739},
 keywords = {Stars: Planetary Systems: Formation, Planets and Satellites: Formation},
     year = 2007,
    month = jan,
   volume = 655,
    pages = {541-549},
      doi = {10.1086/509759},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...655..541M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bara09,
   author = {{Baraffe}, I. and {Chabrier}, G. and {Gallardo}, J.},
    title = "{Episodic Accretion at Early Stages of Evolution of Low-Mass Stars and Brown Dwarfs: A Solution for the Observed Luminosity Spread in H-R Diagrams?}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0907.3886},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, stars: formation, stars: low-mass, brown dwarfs},
     year = 2009,
    month = sep,
   volume = 702,
    pages = {L27-L31},
      doi = {10.1088/0004-637X/702/1/L27},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...702L..27B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cace15,
   author = {{Caceres}, C. and {Hardy}, A. and {Schreiber}, M.~R. and {C{\'a}novas}, H. and 
	{Cieza}, L.~A. and {Williams}, J.~P. and {Hales}, A. and {Pinte}, C. and 
	{M{\'e}nard}, F. and {Wahhaj}, Z.},
    title = "{On the Nature of the Tertiary Companion to FW Tau: ALMA CO Observations and SED Modeling}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1504.05644},
 primaryClass = "astro-ph.EP",
 keywords = {circumstellar matter, planetary systems, protoplanetary disks, stars: individual: FW Tau, techniques: interferometric},
     year = 2015,
    month = jun,
   volume = 806,
      eid = {L22},
    pages = {L22},
      doi = {10.1088/2041-8205/806/2/L22},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...806L..22C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bowl15,
   author = {{Bowler}, B.~P. and {Andrews}, S.~M. and {Kraus}, A.~L. and 
	{Ireland}, M.~J. and {Herczeg}, G. and {Ricci}, L. and {Carpenter}, J. and 
	{Brown}, M.~E.},
    title = "{An ALMA Constraint on the GSC 6214-210 B Circum-Substellar Accretion Disk Mass}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1505.01483},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion disks, brown dwarfs, stars: individual: GSC 6214-210},
     year = 2015,
    month = jun,
   volume = 805,
      eid = {L17},
    pages = {L17},
      doi = {10.1088/2041-8205/805/2/L17},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...805L..17B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krau15,
   author = {{Kraus}, A.~L. and {Andrews}, S.~M. and {Bowler}, B.~P. and 
	{Herczeg}, G. and {Ireland}, M.~J. and {Liu}, M.~C. and {Metchev}, S. and 
	{Cruz}, K.~L.},
    title = "{An ALMA Disk Mass for the Candidate Protoplanetary Companion to FW Tau}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1412.2175},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: formation, planets and satellites: general, protoplanetary disks },
     year = 2015,
    month = jan,
   volume = 798,
      eid = {L23},
    pages = {L23},
      doi = {10.1088/2041-8205/798/1/L23},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798L..23K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Macg17,
   author = {{MacGregor}, M.~A. and {Wilner}, D.~J. and {Czekala}, I. and 
	{Andrews}, S.~M. and {Dai}, Y.~S. and {Herczeg}, G.~J. and {Kratter}, K.~M. and 
	{Kraus}, A.~L. and {Ricci}, L. and {Testi}, L.},
    title = "{ALMA Measurements of Circumstellar Material in the GQ Lup System}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1611.06229},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: individual: GQ Lup, submillimeter: planetary systems},
     year = 2017,
    month = jan,
   volume = 835,
      eid = {17},
    pages = {17},
      doi = {10.3847/1538-4357/835/1/17},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...835...17M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Clos14,
   author = {{Close}, L.~M. and {Follette}, K.~B. and {Males}, J.~R. and 
	{Puglisi}, A. and {Xompero}, M. and {Apai}, D. and {Najita}, J. and 
	{Weinberger}, A.~J. and {Morzinski}, K. and {Rodigas}, T.~J. and 
	{Hinz}, P. and {Bailey}, V. and {Briguglio}, R.},
    title = "{Discovery of H{$\alpha$} Emission from the Close Companion inside the Gap of Transitional Disk HD 142527}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1401.1273},
 primaryClass = "astro-ph.EP",
 keywords = {instrumentation: adaptive optics, open clusters and associations: individual: Sco OB-2 association, planetary systems, planet-disk interactions, stars: individual: HD 142527},
     year = 2014,
    month = feb,
   volume = 781,
      eid = {L30},
    pages = {L30},
      doi = {10.1088/2041-8205/781/2/L30},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...781L..30C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Clos13,
   author = {{Close}, L.~M. and {Males}, J.~R. and {Morzinski}, K. and {Kopon}, D. and 
	{Follette}, K. and {Rodigas}, T.~J. and {Hinz}, P. and {Wu}, Y.-L. and 
	{Puglisi}, A. and {Esposito}, S. and {Riccardi}, A. and {Pinna}, E. and 
	{Xompero}, M. and {Briguglio}, R. and {Uomoto}, A. and {Hare}, T.
	},
    title = "{Diffraction-limited Visible Light Images of Orion Trapezium Cluster with the Magellan Adaptive Secondary Adaptive Optics System (MagAO)}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1308.4155},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: general, brown dwarfs, instrumentation: adaptive optics, stars: evolution, stars: formation, stars: low-mass},
     year = 2013,
    month = sep,
   volume = 774,
      eid = {94},
    pages = {94},
      doi = {10.1088/0004-637X/774/2/94},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...774...94C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sall15,
   author = {{Sallum}, S. and {Follette}, K.~B. and {Eisner}, J.~A. and {Close}, L.~M. and 
	{Hinz}, P. and {Kratter}, K. and {Males}, J. and {Skemer}, A. and 
	{Macintosh}, B. and {Tuthill}, P. and {Bailey}, V. and {Defr{\`e}re}, D. and 
	{Morzinski}, K. and {Rodigas}, T. and {Spalding}, E. and {Vaz}, A. and 
	{Weinberger}, A.~J.},
    title = "{Accreting protoplanets in the LkCa 15 transition disk}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1511.07456},
 primaryClass = "astro-ph.EP",
     year = 2015,
    month = nov,
   volume = 527,
    pages = {342-344},
      doi = {10.1038/nature15761},
   adsurl = {http://adsabs.harvard.edu/abs/2015Natur.527..342S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bocc15,
   author = {{Boccaletti}, A. and {Lagage}, P.-O. and {Baudoz}, P. and {Beichman}, C. and 
	{Bouchet}, P. and {Cavarroc}, C. and {Dubreuil}, D. and {Glasse}, A. and 
	{Glauser}, A.~M. and {Hines}, D.~C. and {Lajoie}, C.-P. and 
	{Lebreton}, J. and {Perrin}, M.~D. and {Pueyo}, L. and {Reess}, J.~M. and 
	{Rieke}, G.~H. and {Ronayette}, S. and {Rouan}, D. and {Soummer}, R. and 
	{Wright}, G.~S.},
    title = "{The Mid-Infrared Instrument for the James Webb Space Telescope, V: Predicted Performance of the MIRI Coronagraphs}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1508.02352},
 primaryClass = "astro-ph.IM",
     year = 2015,
    month = jul,
   volume = 127,
    pages = {633},
      doi = {10.1086/682256},
   adsurl = {http://adsabs.harvard.edu/abs/2015PASP..127..633B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Line14,
   author = {{Line}, M.~R. and {Fortney}, J.~J. and {Marley}, M.~S. and {Sorahana}, S.
	},
    title = "{A Data-driven Approach for Retrieving Temperatures and Abundances in Brown Dwarf Atmospheres}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1403.6412},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, methods: statistical, radiative transfer, stars: atmospheres, stars: individual: Gl 570D},
     year = 2014,
    month = sep,
   volume = 793,
      eid = {33},
    pages = {33},
      doi = {10.1088/0004-637X/793/1/33},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...793...33L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Line15,
   author = {{Line}, M.~R. and {Teske}, J. and {Burningham}, B. and {Fortney}, J.~J. and 
	{Marley}, M.~S.},
    title = "{Uniform Atmospheric Retrieval Analysis of Ultracool Dwarfs. I. Characterizing Benchmarks, Gl 570D and HD 3651B}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1504.06670},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, radiative transfer, stars: abundances, stars: atmospheres, stars: individual: Gl 570, HD 3651},
     year = 2015,
    month = jul,
   volume = 807,
      eid = {183},
    pages = {183},
      doi = {10.1088/0004-637X/807/2/183},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...807..183L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burn17,
   author = {{Burningham}, B. and {Marley}, M.~S. and {Line}, M.~R. and {Visscher}, C. and 
	{Morley}, C.~V. and {Saumon}, D. and {Lupu}, R. and {Freedman}, R.
	},
    title = "{Retrieval of atmospheric properties of cloudy L dwarfs}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1701.01257},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
     year = 2017,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170101257B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krei14b,
   author = {{Kreidberg}, L. and {Bean}, J.~L. and {D{\'e}sert}, J.-M. and 
	{Line}, M.~R. and {Fortney}, J.~J. and {Madhusudhan}, N. and 
	{Stevenson}, K.~B. and {Showman}, A.~P. and {Charbonneau}, D. and 
	{McCullough}, P.~R. and {Seager}, S. and {Burrows}, A. and {Henry}, G.~W. and 
	{Williamson}, M. and {Kataria}, T. and {Homeier}, D.},
    title = "{A Precise Water Abundance Measurement for the Hot Jupiter WASP-43b}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1410.2255},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: individual: WASP-43b },
     year = 2014,
    month = oct,
   volume = 793,
      eid = {L27},
    pages = {L27},
      doi = {10.1088/2041-8205/793/2/L27},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...793L..27K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Benn16,
   author = {{Benneke}, B.},
    title = "{Strict Upper Limits on the Carbon-to-Oxygen Ratios of Eight Hot Jupiters from Self-Consistent Atmospheric Retrieval}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1504.07655},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2015,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150407655B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lavi16,
   author = {{Lavie}, B. and {Mendon{\c c}a}, J.~M. and {Mordasini}, C. and 
	{Malik}, M. and {Bonnefoy}, M. and {Demory}, B.-O. and {Oreshenko}, M. and 
	{Grimm}, S.~L. and {Ehrenreich}, D. and {Heng}, K.},
    title = "{HELIOS-Retrieval: An Open-source, Nested Sampling Atmospheric Retrieval Code, Application to the HR 8799 Exoplanets and Inferred Constraints for Planet Formation}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1610.03216},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics, Physics - Atmospheric and Oceanic Physics},
     year = 2016,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161003216L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hell14,
   author = {{Helling}, C. and {Woitke}, P. and {Rimmer}, P.~B. and {Kamp}, I. and 
	{Thi}, W.-F. and {Meijerink}, R.},
    title = "{Disk Evolution, Element Abundances and Cloud Properties of Young Gas Giant Planets}",
  journal = {Life},
archivePrefix = "arXiv",
   eprint = {1403.4420},
 primaryClass = "astro-ph.EP",
 keywords = {astrochemistry, element abundances, extra-solar planets, gas giants, planet formation, cloud formation },
     year = 2014,
    month = apr,
   volume = 4,
      doi = {10.3390/life4020142},
   adsurl = {http://adsabs.harvard.edu/abs/2014Life....4..142H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hell09,
   author = {{Helled}, R. and {Schubert}, G.},
    title = "{Heavy-element Enrichment of a Jupiter-mass Protoplanet as a Function of Orbital Location}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0903.1997},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems: protoplanetary disks, planets and satellites: formation, solar system: formation},
     year = 2009,
    month = jun,
   volume = 697,
    pages = {1256-1262},
      doi = {10.1088/0004-637X/697/2/1256},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...697.1256H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ober16,
   author = {{{\"O}berg}, K.~I. and {Bergin}, E.~A.},
    title = "{Excess C/O and C/H in Outer Protoplanetary Disk Gas}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1610.07859},
 keywords = {astrochemistry, molecular processes, planet{\ndash}disk interactions, planets and satellites: atmospheres, planets and satellites: formation, protoplanetary disks},
     year = 2016,
    month = nov,
   volume = 831,
      eid = {L19},
    pages = {L19},
      doi = {10.3847/2041-8205/831/2/L19},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...831L..19O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ober11,
   author = {{{\"O}berg}, K.~I. and {Murray-Clay}, R. and {Bergin}, E.~A.
	},
    title = "{The Effects of Snowlines on C/O in Planetary Atmospheres}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1110.5567},
 keywords = {astrochemistry, circumstellar matter, molecular processes, planetary systems, planet-disk interactions, planets and satellites: atmospheres},
     year = 2011,
    month = dec,
   volume = 743,
      eid = {L16},
    pages = {L16},
      doi = {10.1088/2041-8205/743/1/L16},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743L..16O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mord09,
   author = {{Mordasini}, C. and {Alibert}, Y. and {Benz}, W.},
    title = "{Extrasolar planet population synthesis. I. Method, formation tracks, and mass-distance distribution}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0904.2524},
 primaryClass = "astro-ph.EP",
 keywords = {stars: planetary systems, stars: planetary systems: formation, stars: planetary systems: protoplanetary disks, planets and satellites: formation, solar system: formation, methods: numerical},
     year = 2009,
    month = jul,
   volume = 501,
    pages = {1139-1160},
      doi = {10.1051/0004-6361/200810301},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...501.1139M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Dorn16,
   author = {{Dorn}, R.~J. and {Follert}, R. and {Bristow}, P. and {Cumani}, C. and 
	{Eschbaumer}, S. and {Grunhut}, J. and {Haimerl}, A. and {Hatzes}, A. and 
	{Heiter}, U. and {Hinterschuster}, R. and {Ives}, D.~J. and 
	{Jung}, Y. and {Kerber}, F. and {Klein}, B. and {Lavaila}, A. and 
	{Lizon}, J.~L. and {L{\"o}winger}, T. and {Molina-Conde}, I. and 
	{Nicholson}, B. and {Marquart}, T. and {Oliva}, E. and {Origlia}, L. and 
	{Pasquini}, L. and {Paufique}, J. and {Piskunov}, N. and {Reiners}, A. and 
	{Seemann}, U. and {Stegmeier}, J. and {Stempels}, E. and {Tordo}, S.
	},
    title = "{The ``+'' for CRIRES: enabling better science at infrared wavelength and high spectral resolution at the ESO VLT}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2016,
   series = {\procspie},
   volume = 9908,
    month = aug,
      eid = {99080I},
    pages = {99080I},
      doi = {10.1117/12.2232837},
   adsurl = {http://adsabs.harvard.edu/abs/2016SPIE.9908E..0ID},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Quir16,
   author = {{Quirrenbach}, A. and {Amado}, P.~J. and {Caballero}, J.~A. and 
	{Mundt}, R. and {Reiners}, A. and {Ribas}, I. and {Seifert}, W. and 
	{Abril}, M. and {Aceituno}, J. and {Alonso-Floriano}, F.~J. and 
	{Anwand-Heerwart}, H. and {Azzaro}, M. and {Bauer}, F. and {Barrado}, D. and 
	{Becerril}, S. and {Bejar}, V.~J.~S. and {Benitez}, D. and {Berdinas}, Z.~M. and 
	{Brinkm{\"o}ller}, M. and {Cardenas}, M.~C. and {Casal}, E. and 
	{Claret}, A. and {Colom{\'e}}, J. and {Cortes-Contreras}, M. and 
	{Czesla}, S. and {Doellinger}, M. and {Dreizler}, S. and {Feiz}, C. and 
	{Fernandez}, M. and {Ferro}, I.~M. and {Fuhrmeister}, B. and 
	{Galadi}, D. and {Gallardo}, I. and {G{\'a}lvez-Ortiz}, M.~C. and 
	{Garcia-Piquer}, A. and {Garrido}, R. and {Gesa}, L. and {G{\'o}mez Galera}, V. and 
	{Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and {Gonzalez Peinado}, R. and 
	{Gr{\"o}zinger}, U. and {Gu{\`a}rdia}, J. and {Guenther}, E.~W. and 
	{de Guindos}, E. and {Hagen}, H.-J. and {Hatzes}, A.~P. and 
	{Hauschildt}, P.~H. and {Helmling}, J. and {Henning}, T. and 
	{Hermann}, D. and {Hern{\'a}ndez Arabi}, R. and {Hern{\'a}ndez Casta{\~n}o}, L. and 
	{Hern{\'a}ndez Hernando}, F. and {Herrero}, E. and {Huber}, A. and 
	{Huber}, K.~F. and {Huke}, P. and {Jeffers}, S.~V. and {de Juan}, E. and 
	{Kaminski}, A. and {Kehr}, M. and {Kim}, M. and {Klein}, R. and 
	{Kl{\"u}ter}, J. and {K{\"u}rster}, M. and {Lafarga}, M. and 
	{Lara}, L.~M. and {Lamert}, A. and {Laun}, W. and {Launhardt}, R. and 
	{Lemke}, U. and {Lenzen}, R. and {Llamas}, M. and {Lopez del Fresno}, M. and 
	{L{\'o}pez-Puertas}, M. and {L{\'o}pez-Santiago}, J. and {Lopez Salas}, J.~F. and 
	{Magan Madinabeitia}, H. and {Mall}, U. and {Mandel}, H. and 
	{Mancini}, L. and {Marin Molina}, J.~A. and {Maroto Fern{\'a}ndez}, D. and 
	{Mart{\'{\i}}n}, E.~L. and {Mart{\'{\i}}n-Ruiz}, S. and {Marvin}, C. and 
	{Mathar}, R.~J. and {Mirabet}, E. and {Montes}, D. and {Morales}, J.~C. and 
	{Morales Mu{\~n}oz}, R. and {Nagel}, E. and {Naranjo}, V. and 
	{Nowak}, G. and {Palle}, E. and {Panduro}, J. and {Passegger}, V.~M. and 
	{Pavlov}, A. and {Pedraz}, S. and {Perez}, E. and {P{\'e}rez-Medialdea}, D. and 
	{Perger}, M. and {Pluto}, M. and {Ram{\'o}n}, A. and {Rebolo}, R. and 
	{Redondo}, P. and {Reffert}, S. and {Reinhart}, S. and {Rhode}, P. and 
	{Rix}, H.-W. and {Rodler}, F. and {Rodr{\'{\i}}guez}, E. and 
	{Rodr{\'{\i}}guez L{\'o}pez}, C. and {Rohloff}, R.~R. and {Rosich}, A. and 
	{Sanchez Carrasco}, M.~A. and {Sanz-Forcada}, J. and {Sarkis}, P. and 
	{Sarmiento}, L.~F. and {Sch{\"a}fer}, S. and {Schiller}, J. and 
	{Schmidt}, C. and {Schmitt}, J.~H.~M.~M. and {Sch{\"o}fer}, P. and 
	{Schweitzer}, A. and {Shulyak}, D. and {Solano}, E. and {Stahl}, O. and 
	{Storz}, C. and {Tabernero}, H.~M. and {Tala}, M. and {Tal-Or}, L. and 
	{Ulbrich}, R.-G. and {Veredas}, G. and {Vico Linares}, J.~I. and 
	{Vilardell}, F. and {Wagner}, K. and {Winkler}, J. and {Zapatero Osorio}, M.-R. and 
	{Zechmeister}, M. and {Ammler-von Eiff}, M. and {Anglada-Escud{\'e}}, G. and 
	{del Burgo}, C. and {Garcia-Vargas}, M.~L. and {Klutsch}, A. and 
	{Lizon}, J.-L. and {Lopez-Morales}, M. and {Ofir}, A. and {P{\'e}rez-Calpena}, A. and 
	{Perryman}, M.~A.~C. and {S{\'a}nchez-Blanco}, E. and {Strachan}, J.~B.~P. and 
	{St{\"u}rmer}, J. and {Su{\'a}rez}, J.~C. and {Trifonov}, T. and 
	{Tulloch}, S.~M. and {Xu}, W.},
    title = "{CARMENES: an overview six months after first light}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2016,
   series = {\procspie},
   volume = 9908,
    month = aug,
      eid = {990812},
    pages = {990812},
      doi = {10.1117/12.2231880},
   adsurl = {http://adsabs.harvard.edu/abs/2016SPIE.9908E..12Q},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Arti14,
   author = {{Artigau}, {\'E}. and {Kouach}, D. and {Donati}, J.-F. and {Doyon}, R. and 
	{Delfosse}, X. and {Baratchart}, S. and {Lacombe}, M. and {Moutou}, C. and 
	{Rabou}, P. and {Par{\`e}s}, L.~P. and {Micheau}, Y. and {Thibault}, S. and 
	{Reshetov}, V.~A. and {Dubois}, B. and {Hernandez}, O. and {Vall{\'e}e}, P. and 
	{Wang}, S.-Y. and {Dolon}, F. and {Pepe}, F.~A. and {Bouchy}, F. and 
	{Striebig}, N. and {H{\'e}nault}, F. and {Loop}, D. and {Saddlemyer}, L. and 
	{Barrick}, G. and {Vermeulen}, T. and {Dupieux}, M. and {H{\'e}brard}, G. and 
	{Boisse}, I. and {Martioli}, E. and {Alencar}, S.~H.~P. and 
	{do Nascimento}, J.-D. and {Figueira}, P.},
    title = "{SPIRou: the near-infrared spectropolarimeter/high-precision velocimeter for the Canada-France-Hawaii telescope}",
booktitle = {Ground-based and Airborne Instrumentation for Astronomy V},
     year = 2014,
   series = {\procspie},
   volume = 9147,
archivePrefix = "arXiv",
   eprint = {1406.6992},
 primaryClass = "astro-ph.IM",
    month = jul,
      eid = {914715},
    pages = {914715},
      doi = {10.1117/12.2055663},
   adsurl = {http://adsabs.harvard.edu/abs/2014SPIE.9147E..15A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gagn15,
   author = {{Gagn{\'e}}, J. and {Faherty}, J.~K. and {Cruz}, K.~L. and {Lafreni{\'e}re}, D. and 
	{Doyon}, R. and {Malo}, L. and {Burgasser}, A.~J. and {Naud}, M.-E. and 
	{Artigau}, {\'E}. and {Bouchard}, S. and {Gizis}, J.~E. and 
	{Albert}, L.},
    title = "{BANYAN. VII. A New Population of Young Substellar Candidate Members of Nearby Moving Groups from the BASS Survey}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1506.07712},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, methods: data analysis, proper motions, stars: kinematics and dynamics, stars: low-mass},
     year = 2015,
    month = aug,
   volume = 219,
      eid = {33},
    pages = {33},
      doi = {10.1088/0067-0049/219/2/33},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJS..219...33G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fahe16,
   author = {{Faherty}, J.~K. and {Riedel}, A.~R. and {Cruz}, K.~L. and {Gagne}, J. and 
	{Filippazzo}, J.~C. and {Lambrides}, E. and {Fica}, H. and {Weinberger}, A. and 
	{Thorstensen}, J.~R. and {Tinney}, C.~G. and {Baldassare}, V. and 
	{Lemonier}, E. and {Rice}, E.~L.},
    title = "{Population Properties of Brown Dwarf Analogs to Exoplanets}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1605.07927},
 primaryClass = "astro-ph.SR",
 keywords = {astrometry, brown dwarfs, stars: low-mass},
     year = 2016,
    month = jul,
   volume = 225,
      eid = {10},
    pages = {10},
      doi = {10.3847/0067-0049/225/1/10},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJS..225...10F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zuck04,
   author = {{Zuckerman}, B. and {Song}, I.},
    title = "{Young Stars Near the Sun}",
  journal = {\araa},
     year = 2004,
    month = sep,
   volume = 42,
    pages = {685-721},
      doi = {10.1146/annurev.astro.42.053102.134111},
   adsurl = {http://adsabs.harvard.edu/abs/2004ARA%26A..42..685Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oppo13,
   author = {{Oppenheimer}, B.~R. and {Baranec}, C. and {Beichman}, C. and 
	{Brenner}, D. and {Burruss}, R. and {Cady}, E. and {Crepp}, J.~R. and 
	{Dekany}, R. and {Fergus}, R. and {Hale}, D. and {Hillenbrand}, L. and 
	{Hinkley}, S. and {Hogg}, D.~W. and {King}, D. and {Ligon}, E.~R. and 
	{Lockhart}, T. and {Nilsson}, R. and {Parry}, I.~R. and {Pueyo}, L. and 
	{Rice}, E. and {Roberts}, J.~E. and {Roberts}, Jr., L.~C. and 
	{Shao}, M. and {Sivaramakrishnan}, A. and {Soummer}, R. and 
	{Truong}, T. and {Vasisht}, G. and {Veicht}, A. and {Vescelus}, F. and 
	{Wallace}, J.~K. and {Zhai}, C. and {Zimmerman}, N.},
    title = "{Reconnaissance of the HR 8799 Exosolar System. I. Near-infrared Spectroscopy}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1303.2627},
 primaryClass = "astro-ph.EP",
 keywords = {instrumentation: adaptive optics, instrumentation: spectrographs, methods: data analysis, planetary systems, stars: individual: HR 8799, techniques: spectroscopic},
     year = 2013,
    month = may,
   volume = 768,
      eid = {24},
    pages = {24},
      doi = {10.1088/0004-637X/768/1/24},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...768...24O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






==> spbasicHBexo <==

%% spbasicBHexo: manually modified by HD on 20Apr2016 from spbasic.bst 
%% to cut author lists longer than 5 authors to 3 authors et al. 
%% The only modified part is in FUNCTION {format.names} 
%%
%% This is file `spbasic.bst',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `ay,nat,seq-lab,vonx,nm-rvx,ed-rev,jnrlst,dt-beg,yr-par,yrp-x,yrpp-xsp,note-yr,jxper,jttl-rm,thtit-a,pgsep-c,num-xser,ser-vol,jnm-x,btit-rm,bt-rm,pre-pub,doi,edparxc,blk-tit,in-col,fin-bare,pp,ed,abr,mth-bare,ord,jabr,xand,eprint,url,url-blk,em-x,nfss,')
%% ----------------------------------------
%%
%%********************************************************************************%%
%%                                                                                %%
%% For Springer medical, life sciences, chemistry, geology, engineering and       %%
%%   computer science publications.                                               %%
%% For use with the natbib package (see below). Default is author-year citations. %%
%%   When citations are numbered, please use \usepackage[numbers]{natbib}.        %%
%% A lack of punctuation is the key feature. Springer-Verlag 2004/10/15           %%
%% Report bugs and improvements to: Joylene Vette-Guillaume or Frank Holzwarth    %%
%%                                                                                %%
%%********************************************************************************%%
%%
%% Copyright 1994-2004 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2004/02/09 4.13 (PWD, AO, DPC)]
 %   For use with BibTeX version 0.99a or later
 %-------------------------------------------------------------------
 % This bibliography style file is intended for texts in ENGLISH
 % This is an author-year citation style bibliography. As such, it is
 % non-standard LaTeX, and requires a special package file to function properly.
 % Such a package is    natbib.sty   by Patrick W. Daly
 % The form of the \bibitem entries is
 %   \bibitem[Jones et al.(1990)]{key}...
 %   \bibitem[Jones et al.(1990)Jones, Baker, and Smith]{key}...
 % The essential feature is that the label (the part in brackets) consists
 % of the author names, as they should appear in the citation, with the year
 % in parentheses following. There must be no space before the opening
 % parenthesis!
 % With natbib v5.3, a full list of authors may also follow the year.
 % In natbib.sty, it is possible to define the type of enclosures that is
 % really wanted (brackets or parentheses), but in either case, there must
 % be parentheses in the label.
 % The \cite command functions as follows:
 %   \citet{key} ==>>                Jones et al. (1990)
 %   \citet*{key} ==>>               Jones, Baker, and Smith (1990)
 %   \citep{key} ==>>                (Jones et al., 1990)
 %   \citep*{key} ==>>               (Jones, Baker, and Smith, 1990)
 %   \citep[chap. 2]{key} ==>>       (Jones et al., 1990, chap. 2)
 %   \citep[e.g.][]{key} ==>>        (e.g. Jones et al., 1990)
 %   \citep[e.g.][p. 32]{key} ==>>   (e.g. Jones et al., p. 32)
 %   \citeauthor{key} ==>>           Jones et al.
 %   \citeauthor*{key} ==>>          Jones, Baker, and Smith
 %   \citeyear{key} ==>>             1990
 %---------------------------------------------------------------------

ENTRY
  { address
    archive
    author
    booktitle
    chapter
    doi
    edition
    editor
    eid
    eprint
    howpublished
    institution
    journal
    key
    month
    note
    number
    organization
    pages
    publisher
    school
    series
    title
    type
    url
    volume
    year
  }
  {}
  { label extra.label sort.label short.list }
INTEGERS { output.state before.all mid.sentence after.sentence after.block }
FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}
STRINGS { s t}
FUNCTION {output.nonnull}
{ 's :=
  output.state mid.sentence =
    { ", " * write$ }
    { output.state after.block =
        { add.period$ write$
          newline$
          "\newblock " write$
        }
        { output.state before.all =
            'write$
            { add.period$ " " * write$ }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}
FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}
FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}
FUNCTION {fin.entry}
{ duplicate$ empty$
    'pop$
    'write$
  if$
  newline$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}
FUNCTION {new.sentence}
{ output.state after.block =
    'skip$
    { output.state before.all =
        'skip$
        { after.sentence 'output.state := }
      if$
    }
  if$
}
FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}

FUNCTION {no.blank.or.punct}
{  "\hspace{0pt}" * before.all 'output.state :=
}

FUNCTION {date.block}
{
    add.blank
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}
FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}
FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}
STRINGS {z}
FUNCTION {remove.dots}
{ 'z :=
  ""
  { z empty$ not }
  { z #1 #1 substring$
    z #2 global.max$ substring$ 'z :=
    duplicate$ "." = 'pop$
      { * }
    if$
  }
  while$
}
FUNCTION {new.block.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.block
  if$
}
FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}
FUNCTION {emphasize}
{ skip$ }
FUNCTION {tie.or.space.prefix}
{ duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$
}

FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }
 % Here are the language-specific definitions for explicit words.
 % Each function has a name bbl.xxx where xxx is the English word.
 % The language selected here is ENGLISH
FUNCTION {bbl.and}
{ "and"}

FUNCTION {bbl.etal}
{ "et~al" }

FUNCTION {bbl.editors}
{ "eds" }

FUNCTION {bbl.editor}
{ "ed" }

FUNCTION {bbl.edby}
{ "edited by" }

FUNCTION {bbl.edition}
{ "edn" }

FUNCTION {bbl.volume}
{ "vol" }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "no." }

FUNCTION {bbl.nr}
{ "no." }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "pp" }

FUNCTION {bbl.page}
{ "p" }

FUNCTION {bbl.chapter}
{ "chap" }

FUNCTION {bbl.techrep}
{ "Tech. Rep." }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "PhD thesis" }

FUNCTION {bbl.first}
{ "1st" }

FUNCTION {bbl.second}
{ "2nd" }

FUNCTION {bbl.third}
{ "3rd" }

FUNCTION {bbl.fourth}
{ "4th" }

FUNCTION {bbl.fifth}
{ "5th" }

FUNCTION {bbl.st}
{ "st" }

FUNCTION {bbl.nd}
{ "nd" }

FUNCTION {bbl.rd}
{ "rd" }

FUNCTION {bbl.th}
{ "th" }

MACRO {jan} {"Jan."}

MACRO {feb} {"Feb."}

MACRO {mar} {"Mar."}

MACRO {apr} {"Apr."}

MACRO {may} {"May"}

MACRO {jun} {"Jun."}

MACRO {jul} {"Jul."}

MACRO {aug} {"Aug."}

MACRO {sep} {"Sep."}

MACRO {oct} {"Oct."}

MACRO {nov} {"Nov."}

MACRO {dec} {"Dec."}

FUNCTION {eng.ord}
{ duplicate$ "1" swap$ *
  #-2 #1 substring$ "1" =
     { bbl.th * }
     { duplicate$ #-1 #1 substring$
       duplicate$ "1" =
         { pop$ bbl.st * }
         { duplicate$ "2" =
             { pop$ bbl.nd * }
             { "3" =
                 { bbl.rd * }
                 { bbl.th * }
               if$
             }
           if$
          }
       if$
     }
   if$
}

MACRO {acmcs} {"ACM Comput Surv"}

MACRO {acta} {"Acta Inf"}

MACRO {cacm} {"Commun ACM"}

MACRO {ibmjrd} {"IBM~J~Res Dev"}

MACRO {ibmsj} {"IBM Syst~J"}

MACRO {ieeese} {"IEEE Trans Softw Eng"}

MACRO {ieeetc} {"IEEE Trans Comput"}

MACRO {ieeetcad}
 {"IEEE Trans Comput Aid Des"}

MACRO {ipl} {"Inf Process Lett"}

MACRO {jacm} {"J~ACM"}

MACRO {jcss} {"J~Comput Syst Sci"}

MACRO {scp} {"Sci Comput Program"}

MACRO {sicomp} {"SIAM J~Comput"}

MACRO {tocs} {"ACM Trans Comput Syst"}

MACRO {tods} {"ACM Trans Database Syst"}

MACRO {tog} {"ACM Trans Graphic"}

MACRO {toms} {"ACM Trans Math Softw"}

MACRO {toois} {"ACM Trans Office Inf Syst"}

MACRO {toplas} {"ACM Trans Program Lang Syst"}

MACRO {tcs} {"Theor Comput Sci"}

FUNCTION {bibinfo.check}
{ swap$
  duplicate$ missing$
    {
      pop$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ pop$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
FUNCTION {bibinfo.warn}
{ swap$
  duplicate$ missing$
    {
      swap$ "missing " swap$ * " in " * cite$ * warning$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ "empty " swap$ * " in " * cite$ * warning$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
FUNCTION {format.eprint}
{ eprint duplicate$ empty$
    'skip$
    { "\eprint"
      archive empty$
        'skip$
        { "[" * archive * "]" * }
      if$
      "{" * swap$ * "}" *
    }
  if$
}
FUNCTION {format.url}
{ url empty$
    { "" }
    { "\urlprefix\url{" url * "}" * }
  if$
}

STRINGS  { bibinfo}
INTEGERS { nameptr namesleft numnames }

FUNCTION {format.names}
{ 'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv~}{ll}{ f{}}{ jj}"
      format.name$
      remove.dots
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          nameptr #3
          #1 + =
          numnames #5
          > and
            { "others" 't :=
              #1 'namesleft := }
            'skip$
          if$
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
%%              "," *
              t "others" =
                {
                  " " * bbl.etal *
                }
                { " " * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  } if$
}
FUNCTION {format.names.ed}
{
  format.names
}
FUNCTION {format.key}
{ empty$
    { key field.or.null }
    { "" }
  if$
}

FUNCTION {format.authors}
{ author "author" format.names
}
FUNCTION {get.bbl.editor}
{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }

FUNCTION {format.editors}
{ editor "editor" format.names duplicate$ empty$ 'skip$
    {
      " " *
      get.bbl.editor
   "(" swap$ * ")" *
      *
    }
  if$
}
FUNCTION {format.doi}
{ doi "doi" bibinfo.check
  duplicate$ empty$ 'skip$
    {
      "\doi{" swap$ * "}" *
    }
  if$
}
FUNCTION {format.note}
{
 note empty$
    { "" }
    { note #1 #1 substring$
      duplicate$ "{" =
        'skip$
        { output.state mid.sentence =
          { "l" }
          { "u" }
        if$
        change.case$
        }
      if$
      note #2 global.max$ substring$ * "note" bibinfo.check
    }
  if$
}

FUNCTION {format.title}
{ title
  duplicate$ empty$ 'skip$
    { "t" change.case$ }
  if$
  "title" bibinfo.check
}
FUNCTION {format.full.names}
{'s :=
 "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv~}{ll}" format.name$
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {
                  " " * bbl.etal *
                }
                {
                  numnames #2 >
                    { "," * }
                    'skip$
                  if$
                  bbl.and
                  space.word * t *
                }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {author.editor.key.full}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { editor format.full.names }
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {author.key.full}
{ author empty$
    { key empty$
         { cite$ #1 #3 substring$ }
          'key
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {editor.key.full}
{ editor empty$
    { key empty$
         { cite$ #1 #3 substring$ }
          'key
      if$
    }
    { editor format.full.names }
  if$
}

FUNCTION {make.full.names}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.key.full
    { type$ "proceedings" =
        'editor.key.full
        'author.key.full
      if$
    }
  if$
}

FUNCTION {output.bibitem}
{ newline$
  "\bibitem[{" write$
  label write$
  ")" make.full.names duplicate$ short.list =
     { pop$ }
     { * }
   if$
  "}]{" * write$
  cite$ write$
  "}" write$
  newline$
  ""
  before.all 'output.state :=
}

FUNCTION {add.period}
{ duplicate$ empty$
    'skip$
    { "." * add.blank }
  if$
}

FUNCTION {if.digit}
{ duplicate$ "0" =
  swap$ duplicate$ "1" =
  swap$ duplicate$ "2" =
  swap$ duplicate$ "3" =
  swap$ duplicate$ "4" =
  swap$ duplicate$ "5" =
  swap$ duplicate$ "6" =
  swap$ duplicate$ "7" =
  swap$ duplicate$ "8" =
  swap$ "9" = or or or or or or or or or
}
FUNCTION {n.separate}
{ 't :=
  ""
  #0 'numnames :=
  { t empty$ not }
  { t #-1 #1 substring$ if.digit
      { numnames #1 + 'numnames := }
      { #0 'numnames := }
    if$
    t #-1 #1 substring$ swap$ *
    t #-2 global.max$ substring$ 't :=
    numnames #5 =
      { duplicate$ #1 #2 substring$ swap$
        #3 global.max$ substring$
        "," swap$ * *
      }
      'skip$
    if$
  }
  while$
}
FUNCTION {n.dashify}
{
  n.separate
  't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
        { t #1 #2 substring$ "--" = not
            { "--" *
              t #2 global.max$ substring$ 't :=
            }
            {   { t #1 #1 substring$ "-" = }
                { "-" *
                  t #2 global.max$ substring$ 't :=
                }
              while$
            }
          if$
        }
        { t #1 #1 substring$ *
          t #2 global.max$ substring$ 't :=
        }
      if$
    }
  while$
}

FUNCTION {word.in}
{ bbl.in capitalize
  ":" *
  " " * }

FUNCTION {format.date}
{ year "year" bibinfo.check duplicate$ empty$
    {
      "empty year in " cite$ * "; set to ????" * warning$
       pop$ "????"
    }
    'skip$
  if$
  extra.label *
  before.all 'output.state :=
  " (" swap$ * ")" *
}
FUNCTION {format.btitle}
{ title "title" bibinfo.check
  duplicate$ empty$ 'skip$
    {
    }
  if$
}
FUNCTION {either.or.check}
{ empty$
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}
FUNCTION {format.bvolume}
{ volume empty$
    { "" }
    { bbl.volume volume tie.or.space.prefix
      "volume" bibinfo.check * *
      series "series" bibinfo.check
      duplicate$ empty$ 'pop$
        { emphasize ", " * swap$ * }
      if$
      "volume and number" number either.or.check
    }
  if$
}
FUNCTION {format.number.series}
{ volume empty$
    { number empty$
        { series field.or.null }
        { series empty$
            { number "number" bibinfo.check }
            { output.state mid.sentence =
                { bbl.number }
                { bbl.number capitalize }
              if$
              number tie.or.space.prefix "number" bibinfo.check * *
              bbl.in space.word *
              series "series" bibinfo.check *
            }
          if$
        }
      if$
    }
    { "" }
  if$
}
FUNCTION {is.num}
{ chr.to.int$
  duplicate$ "0" chr.to.int$ < not
  swap$ "9" chr.to.int$ > not and
}

FUNCTION {extract.num}
{ duplicate$ 't :=
  "" 's :=
  { t empty$ not }
  { t #1 #1 substring$
    t #2 global.max$ substring$ 't :=
    duplicate$ is.num
      { s swap$ * 's := }
      { pop$ "" 't := }
    if$
  }
  while$
  s empty$
    'skip$
    { pop$ s }
  if$
}

FUNCTION {convert.edition}
{ extract.num "l" change.case$ 's :=
  s "first" = s "1" = or
    { bbl.first 't := }
    { s "second" = s "2" = or
        { bbl.second 't := }
        { s "third" = s "3" = or
            { bbl.third 't := }
            { s "fourth" = s "4" = or
                { bbl.fourth 't := }
                { s "fifth" = s "5" = or
                    { bbl.fifth 't := }
                    { s #1 #1 substring$ is.num
                        { s eng.ord 't := }
                        { edition 't := }
                      if$
                    }
                  if$
                }
              if$
            }
          if$
        }
      if$
    }
  if$
  t
}

FUNCTION {format.edition}
{ edition duplicate$ empty$ 'skip$
    {
      convert.edition
      output.state mid.sentence =
        { "l" }
        { "t" }
      if$ change.case$
      "edition" bibinfo.check
      " " * bbl.edition *
    }
  if$
}
INTEGERS { multiresult }
FUNCTION {multi.page.check}
{ 't :=
  #0 'multiresult :=
    { multiresult not
      t empty$ not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
        { #1 'multiresult := }
        { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}
FUNCTION {format.pages}
{ pages duplicate$ empty$ 'skip$
    { duplicate$ multi.page.check
        {
          bbl.pages swap$
          n.dashify
        }
        {
          bbl.page swap$
        }
      if$
      tie.or.space.prefix
      "pages" bibinfo.check
      * *
    }
  if$
}
FUNCTION {format.journal.pages}
{ pages duplicate$ empty$ 'pop$
    { swap$ duplicate$ empty$
        { pop$ pop$ format.pages }
        {
          ":" *
          swap$
          n.dashify
          "pages" bibinfo.check
          *
        }
      if$
    }
  if$
}
FUNCTION {format.journal.eid}
{ eid "eid" bibinfo.check
  duplicate$ empty$ 'pop$
    { swap$ duplicate$ empty$ 'skip$
      {
          ":" *
      }
      if$
      swap$ *
    }
  if$
}
FUNCTION {format.vol.num.pages}
{ volume field.or.null
  duplicate$ empty$ 'skip$
    {
      "volume" bibinfo.check
    }
  if$
  number "number" bibinfo.check duplicate$ empty$ 'skip$
    {
      swap$ duplicate$ empty$
        { "there's a number but no volume in " cite$ * warning$ }
        'skip$
      if$
      swap$
      "(" swap$ * ")" *
    }
  if$ *
  eid empty$
    { format.journal.pages }
    { format.journal.eid }
  if$
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    'format.pages
    { type empty$
        { bbl.chapter }
        { type "l" change.case$
          "type" bibinfo.check
        }
      if$
      chapter tie.or.space.prefix
      "chapter" bibinfo.check
      * *
      pages empty$
        'skip$
        { ", " * format.pages * }
      if$
    }
  if$
}

FUNCTION {format.booktitle}
{
  booktitle "booktitle" bibinfo.check
}
FUNCTION {format.in.ed.booktitle}
{ format.booktitle duplicate$ empty$ 'skip$
    {
      editor "editor" format.names.ed duplicate$ empty$ 'pop$
        {
          " " *
          get.bbl.editor
          "(" swap$ * ") " *
          * swap$
          * }
      if$
      word.in swap$ *
    }
  if$
}
FUNCTION {format.thesis.type}
{ type duplicate$ empty$
    'pop$
    { swap$ pop$
      "t" change.case$ "type" bibinfo.check
    }
  if$
}
FUNCTION {format.tr.number}
{ number "number" bibinfo.check
  type duplicate$ empty$
    { pop$ bbl.techrep }
    'skip$
  if$
  "type" bibinfo.check
  swap$ duplicate$ empty$
    { pop$ "t" change.case$ }
    { tie.or.space.prefix * * }
  if$
}
FUNCTION {format.article.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}
FUNCTION {format.book.crossref}
{ volume duplicate$ empty$
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      pop$ word.in
    }
    { bbl.volume
      capitalize
      swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *
    }
  if$
  " \cite{" * crossref * "}" *
}
FUNCTION {format.incoll.inproc.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}
FUNCTION {format.org.or.pub}
{ 't :=
  ""
  address empty$ t empty$ and
    'skip$
    {
      t empty$
        { address "address" bibinfo.check *
        }
        { t *
          address empty$
            'skip$
            { ", " * address "address" bibinfo.check * }
          if$
        }
      if$
    }
  if$
}
FUNCTION {format.publisher.address}
{ publisher "publisher" bibinfo.warn format.org.or.pub
}

FUNCTION {format.organization.address}
{ organization "organization" bibinfo.check format.org.or.pub
}

FUNCTION {article}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.sentence
  crossref missing$
    {
      journal
      remove.dots
      "journal" bibinfo.check
      "journal" output.check
      add.blank
      format.vol.num.pages output
    }
    { format.article.crossref output.nonnull
      format.pages output
    }
  if$
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}
FUNCTION {book}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      editor format.key output
      add.blank
    }
    { format.authors output.nonnull
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      format.edition output
  new.sentence
      format.number.series output
      format.publisher.address output
    }
    {
  new.sentence
      format.book.crossref output.nonnull
    }
  if$
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}
FUNCTION {booklet}
{ output.bibitem
  format.authors output
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.sentence
  howpublished "howpublished" bibinfo.check output
  address "address" bibinfo.check output
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}

FUNCTION {inbook}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      editor format.key output
    }
    { format.authors output.nonnull
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  crossref missing$
    {
      format.bvolume output
      format.edition output
      format.publisher.address output
      format.chapter.pages "chapter and pages" output.check
  new.sentence
      format.number.series output
    }
    {
      format.chapter.pages "chapter and pages" output.check
  new.sentence
      format.book.crossref output.nonnull
    }
  if$
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}

FUNCTION {incollection}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.sentence
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.bvolume output
      format.edition output
      format.number.series output
      format.publisher.address output
      format.chapter.pages output
    }
    { format.incoll.inproc.crossref output.nonnull
      format.chapter.pages output
    }
  if$
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}
FUNCTION {inproceedings}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  new.sentence
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      publisher empty$
        { format.organization.address output }
        { organization "organization" bibinfo.check output
          format.publisher.address output
        }
      if$
      format.bvolume output
      format.number.series output
      format.pages output
    }
    { format.incoll.inproc.crossref output.nonnull
      format.pages output
    }
  if$
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}
FUNCTION {conference} { inproceedings }
FUNCTION {manual}
{ output.bibitem
  format.authors output
  author format.key output
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  new.sentence
  organization "organization" bibinfo.check output
  address "address" bibinfo.check output
  format.edition output
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}

FUNCTION {mastersthesis}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title
  "title" output.check
  new.sentence
  bbl.mthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}

FUNCTION {misc}
{ output.bibitem
  format.authors output
  author format.key output
  format.date "year" output.check
  date.block
  format.title output
  new.sentence
  howpublished "howpublished" bibinfo.check output
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}
FUNCTION {phdthesis}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title
  "title" output.check
  new.sentence
  bbl.phdthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
  format.editors output
  editor format.key output
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  format.bvolume output
  format.number.series output
  publisher empty$
    { format.organization.address output }
    { organization "organization" bibinfo.check output
      format.publisher.address output
    }
  if$
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}

FUNCTION {techreport}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title
  "title" output.check
  new.sentence
  format.tr.number output.nonnull
  institution "institution" bibinfo.warn output
  address "address" bibinfo.check output
  format.doi output
  format.url output
  format.note output
  format.eprint output
  fin.entry
}

FUNCTION {unpublished}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  format.date "year" output.check
  date.block
  format.title "title" output.check
  format.doi output
  format.url output
  format.note "note" output.check
  format.eprint output
  fin.entry
}

FUNCTION {default.type} { misc }
READ
FUNCTION {sortify}
{ purify$
  "l" change.case$
}
INTEGERS { len }
FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}
FUNCTION {format.lab.names}
{ 's :=
  "" 't :=
  s #1 "{vv~}{ll}" format.name$
  s num.names$ duplicate$
  #2 >
    { pop$
      " " * bbl.etal *
    }
    { #2 <
        'skip$
        { s #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            {
              " " * bbl.etal *
            }
            { bbl.and space.word * s #2 "{vv~}{ll}" format.name$
              * }
          if$
        }
      if$
    }
  if$
}

FUNCTION {author.key.label}
{ author empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {author.editor.key.label}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { editor format.lab.names }
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {editor.key.label}
{ editor empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { editor format.lab.names }
  if$
}

FUNCTION {calc.short.authors}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.key.label
    { type$ "proceedings" =
        'editor.key.label
        'author.key.label
      if$
    }
  if$
  'short.list :=
}

FUNCTION {calc.label}
{ calc.short.authors
  short.list
  "("
  *
  year duplicate$ empty$
     { pop$ "????" }
     'skip$
  if$
  *
  'label :=
}

FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{ll{ }}{  f{ }}{  jj{ }}"
      format.name$ 't :=
      nameptr #1 >
        {
          "   "  *
          namesleft #1 = t "others" = and
            { "zzzzz" * }
            { numnames #2 > nameptr #2 = and
                { "zz" * year field.or.null * "   " * }
                'skip$
              if$
              t sortify *
            }
          if$
        }
        { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}
FUNCTION {author.sort}
{ author empty$
    { key empty$
        { "to sort, need author or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
        { key empty$
            { "to sort, need author, editor, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {editor.sort}
{ editor empty$
    { key empty$
        { "to sort, need editor or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { editor sort.format.names }
  if$
}
FUNCTION {presort}
{ calc.label
  label sortify
  "    "
  *
  type$ "book" =
  type$ "inbook" =
  or
    'author.editor.sort
    { type$ "proceedings" =
        'editor.sort
        'author.sort
      if$
    }
  if$
  #1 entry.max$ substring$
  'sort.label :=
  sort.label
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {presort}
SORT
STRINGS { last.label next.extra }
INTEGERS { last.extra.num number.label }
FUNCTION {initialize.extra.label.stuff}
{ #0 int.to.chr$ 'last.label :=
  "" 'next.extra :=
  #0 'last.extra.num :=
  #0 'number.label :=
}
FUNCTION {forward.pass}
{ last.label label =
    { last.extra.num #1 + 'last.extra.num :=
      last.extra.num int.to.chr$ 'extra.label :=
    }
    { "a" chr.to.int$ 'last.extra.num :=
      "" 'extra.label :=
      label 'last.label :=
    }
  if$
  number.label #1 + 'number.label :=
}
FUNCTION {reverse.pass}
{ next.extra "b" =
    { "a" 'extra.label := }
    'skip$
  if$
  extra.label 'next.extra :=
  extra.label
  duplicate$ empty$
    'skip$
    { "{\natexlab{" swap$ * "}}" * }
  if$
  'extra.label :=
  label extra.label * 'label :=
}
EXECUTE {initialize.extra.label.stuff}
ITERATE {forward.pass}
REVERSE {reverse.pass}
FUNCTION {bib.sort.order}
{ sort.label
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}
ITERATE {bib.sort.order}
SORT
FUNCTION {begin.bib}
{ preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{" number.label int.to.str$ * "}" *
  write$ newline$
  "\providecommand{\natexlab}[1]{#1}"
  write$ newline$
  "\providecommand{\url}[1]{{#1}}"
  write$ newline$
  "\providecommand{\urlprefix}{URL }"
  write$ newline$
  "\expandafter\ifx\csname urlstyle\endcsname\relax"
  write$ newline$
  "  \providecommand{\doi}[1]{DOI~\discretionary{}{}{}#1}\else"
  write$ newline$
  "  \providecommand{\doi}{DOI~\discretionary{}{}{}\begingroup \urlstyle{rm}\Url}\fi"
  write$ newline$
  "\providecommand{\eprint}[2][]{\url{#2}}"
  write$ newline$
}
EXECUTE {begin.bib}
EXECUTE {init.state.consts}
ITERATE {call.type$}
FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}
EXECUTE {end.bib}
%% End of customized bst file
%%
%% End of file `spbasic.bst'.


